Particle Filtering for Large Dimensional State Spaces with Multimodal Observation Likelihoods

We study efficient importance sampling techniques for particle filtering (PF) when either (a) the observation likelihood (OL) is frequently multimodal or heavy-tailed, or (b) the state space dimension is large or both. When the OL is multimodal, but the state transition pdf (STP) is narrow enough, the optimal importance density is usually unimodal. Under this assumption, many techniques have been proposed. But when the STP is broad, this assumption does not hold. We study how existing techniques can be generalized to situations where the optimal importance density is multimodal, but is unimodal conditioned on a part of the state vector. Sufficient conditions to test for the unimodality of this conditional posterior are derived. The number of particles, N, to accurately track using a PF increases with state space dimension, thus making any regular PF impractical for large dimensional tracking problems. We propose a solution that partially addresses this problem. An important class of large dimensional problems with multimodal OL is tracking spatially varying physical quantities such as temperature or pressure in a large area using a network of sensors which may be nonlinear and/or may have non-negligible failure probabilities.

==> abstract.tex <==
\begin{abstract}
We consider the problem of tracking the boundary contour of a moving and deforming object from a sequence of images. If the motion of the ``object" or region of interest is constrained (e.g. rigid or approximately rigid), the contour motion can be efficiently represented by a small number of parameters, e.g. the affine group. But if the ``object"  is arbitrarily deforming, each contour point can move independently. Contour deformation then forms an infinite (in practice, very large), dimensional space. Direct application of particle filters for large dimensional problems is impractical, due to the reduction in effective particle size as dimension increases. But in most real problems, at any given time, ``most of the contour deformation" occurs in a small number of dimensions (``effective basis") while the residual deformation in the rest of the state space (``residual space") is ``small". The effective basis may be fixed or time varying. Based on this assumption, we modify the particle filtering method to  perform sequential importance sampling only on the effective basis dimensions, while replacing it with deterministic mode tracking  in residual space (PF-MT). We develop the PF-MT idea for contour tracking.  Techniques for detecting effective basis dimension change and estimating the new effective basis are presented. Tracking results on simulated and real sequences are shown and compared with past work.
% using  using global translation and deformation velocity at subsampled contour locations interpolated using a B-spline basis as the effective basis.
%We show how to approximate the contour deformation in a time varying  small dimensional basis.
% Given a sequence of images as  observations, the goal is to  causally estimate the posterior probability distribution of the contour  and of the global motion and local deformation velocity using a particle filter.
\end{abstract}


==> algor1.tex <==
\begin{algorithm}[b!]   %\begin{algorithmic} [1]
\caption{{\small \bf PF-MT. Going from $\pi_{t-1}^N$ to $\pi_t^N(X_t) = \sum_{i=1}^N \wi \delta(X_{t} - X_{t}^{i})$, \ $X_{t}^{i} = [C_t^{i}, v_{t,s}^{i},v_{t,r}^{i}]$  }}
\label{pfmt}
\ben
\item  \vspace{-0.05in}
{\em IS on effective basis: } $\forall i$, sample $v_{t,s}^{i} \sim \n(f_s(v_{t-1,s}^{i}), \Sigma_s)$ and compute $\chati$ using (\ref{defhatct}).
\item  \vspace{-0.05in}
{\em Mode Tracking (MT) in residual space: } $\forall i$,
\ben
 \item  \vspace{-0.05in}
 Compute $m_t^{i} =  \arg \min_{v_{t,r}} L^i(v_{t,r})$ and $\Sigma_{IS}^{i}\defn (\nabla^2 L(m_t^{i}))^{-1}$.
  \label{modeval}
 \item  \vspace{-0.05in}
 Set $v_{t,r}^{i} = m_t^{i}$. ~~~~~~~~~~~~{\small \bf [instead of IS  from $\n(m_t^{i}, \ \Sigma_{IS}^{i})$ as in PF-EIS]}
 \item  \vspace{-0.05in}
 Compute $C_t^{i}$ using (\ref{defct}). %and set $X_{t}^{i} = [C_t^{i}, v_{t,s}^{i},v_{t,r}^{i}]$.
  \vspace{-0.05in}
\een
\item  \vspace{-0.05in}
{\em Weight \& Resample: } Compute $w_t^{i} \propto w_{t-1}^{i} \frac{p(Y_t|C_t^{i}) \ \n(v_{t,r}^{i}; \ f_r(v_{t-1,r}^{i}), \ \Sigma_r)}{\n(v_{t,r}^{i}; \ m_t^{i}, \ \Sigma_{IS}^{i})}$ and resample.
%w_t^i = \frac{p(Y_t|C_t^i) p(X_t^i|X_{t-1}^i)}{q
 %$q(X_{t}^{i}) = \n(v_{t,s}^{i}; \ f_s(v_{t-1,s}^{i}), \ \Sigma_s)  \ \n(v_{t,r}^{i}; \ m_t^{i}, \ \Sigma_{IS}^{i})$.
%Since $\E_{Y_t}[\Sigma_{IS}^{(i)}] \le \Sigma_r$, when $\Sigma_r$ is small, one can replace $\Sigma_{IS}^{(i)}$ by $\Sigma_r$. With this approximation, the denominator in step \ref{weight} of Algorithm \ref{pfeis} becomes a constant and can be removed.
\label{weight}
\vspace{-0.2in}
\een
\end{algorithm}



==> change.tex <==
\section{State Space Model}
\label{ssmodel}
%Our state space model  is based on the model introduced in \cite{pap2}. %We use $L$ to denote the length of the contour.
The observation at time $t$ (image and edge map at $t$) is denoted by $Y_t$ and the state at $t$ (contour, contour velocity) is denoted by $X_t$. A block diagram is shown in Fig. \ref{modelfig}.  The contour at $t$ can be represented as $C_t=C_t(p) = [C_t^x(p), C_t^y(p)]$, $p \in [0,1]$. The parametrization is not unique, i.e. all re-parameterizations  of the parameter $p$ of the form $\tilde{p}=f(p)$, where $f: [0,1] \rightarrow [0,1]$ is continuous and strictly monotonic, yield the same contour \cite{sapiro}. The  outward normal to contour $C_t$ at $p$ is denoted by $\N(C_t(p))$ or by $\N_t(p)$.
Denote the space of contours~\cite{conformalmetric} by $\spc$. Then the tangent space to $\spc$ at $C_t$ will be \cite{conformalmetric} the space of all non-tangential velocities (velocities along the normal to $C_t$ at each point), since tangential velocity only re-parameterizes the contour~\cite{sapiro}. We use $v_t$ to denote the vector of normal velocities.%, denoted $\tspc_{C_t}$, \in \tspc_{C_t}

We use the notation $\n(x;\mu, \Sigma) \defn \frac{1}{\sqrt{2\pi}|\Sigma|} e^{-x^T \Sigma^{-1} x}$.
%(1/(\sqrt{2\pi}|\Sigma|) ) \exp[-x^T \Sigma^{-1} x]$.

Note that the contour is a geometric entity \cite{sapiro}, i.e. it is a function of its own arclength. Any deformation of the contour deforms the arclength. In implementation using a level set method \cite{sethian1999,osher2003}, this results in  change in contour dimension, $M_t$, and also change in distance between neighboring points, i.e. $p_j, j=1,2,..M_t$ are not uniformly spaced.

%Also, note that $\n(x;\mu,\Sigma)$ denotes a Gaussian probability density function.
\subsection{System Model}
The state at any time $t$, consists of the contour, its normal deformation velocity, and the global translational velocity. %By separating translation, we can assume the deformation velocity to be zero mean.
%\footnote{We treat the translation of the contour separately, for simplicity.}, $\rho_t  \in \re^2$.
Because of the LDSS property (described in Section \ref{mainidea}), ``most of the contour deformation"  occurs in a smaller number of dimensions, $K$, which form the ``effective basis". Thus, we split $v_t$ as $v_t(p) = B_s(p) v_{t,s} + B_r(p) v_{t,r} + \N_t(p)^T \rho_t$ where $B_s$ denotes the effective basis directions for contour deformation (with translation removed) while $B_r$ denotes the basis spanning the residual space. $v_{t,s}$, $v_{t,r}$ denote the corresponding coefficients. $\rho_t \in \re^2$ denotes the global x-y translation vector. We use velocity at $K$ subsampled locations interpolated onto the entire contour using B-spline interpolation functions as the effective basis. This is explained in Section \ref{basischoice}.
We assume that $\rho_t$, $v_{t,s}$ follow a first order autoregressive (AR) model, while $v_{t,r}$ is assumed temporally independent. Thus, the system dynamics of $X_t = [C_t, v_{t,s}, v_{t,r}, \rho_t]$ is:
\setlength{\arraycolsep}{0.05cm}
\bea
\partial{C_t(p)} \se [B_s(p) dv_{t,s} + B_r(p) dv_{t,r} + \N_t(p)^T  d \rho_t ] \ \N_t(p)    \nn \\
dv_{t,s} \se -A_s' v_{t,s} dt + dW_{t,s}, \ \ dW_{t,s} \sim \n(0, \Sigma_s')     \nn \\
dv_{t,r} \se dW_{t,r}, \ \ dW_{t,r} \sim \n(0, \Sigma_r')     \nn \\
d\rho_{t} \se -A_\rho' \rho_{t} dt + dW_{t,\rho}, \ \ dW_{t,\rho} \sim \n(0, \Sigma_\rho')
\eea
where $\partial{C_t(p)}$ denotes partial differential of $C_t$ w.r.t. time and $W_{t,s},W_{t,r},W_{t,\rho}$ are Brownian motions \cite{papolus}, with dimensions $K$, $M_t-K$ and $2$ respectively.  $dW_{t,s}$ (similarly $dW_{t,r}, dW_{t,\rho}$) denotes the change in $W_{t,s}$ in time $dt$. Also, $0 < A_s' < I$ and $0 < A_\rho' < I$.
Assume that the observations arrive every $\deltat$ time instants. The above differential equations can be discretized as follows. We remove ``$(p)$" for clarity.
\bea
\label{defct0}
C_n \se C_{n-1} +  [B_s v_{n,s} + B_r v_{n,r} + \N_{n-1}^T \rho_n] \ \N_{n-1}      \\
v_{n,s} \se [I -A_s'\deltat] v_{n-1,s}  + \nu_{n,s}, \ \ \nu_{n,s} \sim \n(0, \Sigma_s'\deltat^2)      \\
%v_{0,s} \sim \n(0, \Sigma_0 \deltat)
v_{n,r} \se \nu_{n,r}, \ \ \nu_{n,r} \sim \n(0, \Sigma_r'\deltat)      \\
\rho_{n} \se [I -A_\rho'\deltat] \rho_{n-1} + \nu_{n,\rho}, \ \ \nu_{n,\rho} \sim \n(0, \Sigma_\rho'\deltat^2)
\eea
The discretization given in (\ref{defct0}) assumes that
\begin{ass}
The observation interval $\deltat$ is small enough (compared to $B_s v_{n,s} + B_rv_{n,r} + \N_{n-1}^T \rho_n$) so that $\N_{n-1}$ is also approximately normal to $C_n$.
\label{smallmotion}
\end{ass}
Defining $\Sigma_s \defn \Sigma_s'\deltat^2$, $\Sigma_\rho \defn \Sigma_\rho'\deltat^2$, $\Sigma_r \defn  \Sigma_r'\deltat$, $A_s \defn [I -A_s'\deltat]$, $A_\rho \defn [I -A_\rho'\deltat]$, and $\chat \defn C_{n-1} + [B_s v_{n,s}+ \N_{n-1}^T \rho_n ] \N_{n-1} $, and again removing ``$(p)$", we can rewrite the system model:% \cite{cdc06,pap1,pap2}:
\bea
\label{defct}
C_n \se \chat +   B_r v_{n,r}  \N(\chat)   \\
\label{defhatct}
\chat \se C_{n-1} + [B_s v_{n,s} + \N_{n-1}^T \rho_n ] \ \N_{n-1} , \ \  B_s \defn B_s(C_{n-1}) \ \ \ \ \ \  \\
\label{defvts}
v_{n,s} \se A_s v_{n-1,s}  + \nu_{n,s}, \ \ \nu_{n,s} \sim \n(0, \Sigma_s)     \\
\label{defvtr}
v_{n,r} \se \nu_{n,r}, \ \ \nu_{n,r} \sim \n(0, \Sigma_r)      \\
\label{defrhot}
\rho_{n} \se A_\rho \rho_{n-1} + \nu_{n,\rho}, \ \ \nu_{n,\rho} \sim \n(0, \Sigma_\rho)
\eea
where $B_s \defn B_s(C_{n-1})$ is defined by (\ref{defgeom}) or by (\ref{defparam}) given in Appendix \ref{basischoiceapp}. Note, $v_{n,r}$ is actually not part of the state vector (since no element of the next state, $X_{n+1}$, depends on $v_{n,r}$).
% for geometric basis or  for parametric basis

\subsection{Level Set Representation}
\label{levsetrep}
We use the level set method \cite{sethian1999,osher2003} since it automatically handles contour length changes. % to deform the contour
 $C_t$ is represented implicitly as the zero level set of a higher dimensional function, denoted $\phi_t(x)$, i.e. $C_t$ is the collection of all points $\{x \in \re^2: \phi_t(x)=0 \}$ \cite{sethian1999,osher2003} ($x$ denotes the x-y coordinates). The direction of the gradient of $\phi_t$, $\nabla \phi_t (x)$, is along the normal, $\N_t$.  The most common choice of $\phi_t(x)$ is the ``signed distance function" \cite{sethian1999,osher2003}, i.e. the magnitude of $\phi_t(x)$ is the minimum of the distance of $x$ from any  contour point and its sign is taken to be  negative inside the contour and positive outside the contour. Level set evolution corresponding to contour evolution of the form $\pdif{C_t}{t} = v \N$ is given by\cite{sethian1999,osher2003} $\pdif{\phi_t(x)}{t} = v_{extend}(x) ||\nabla \phi_t||$ where $v_{extend}$ is the normal extension \cite{sethian1999,osher2003} of $v$ onto non-zero level sets.




\input{pfmt}

\section{PF-MT (Particle Filter with Mode Tracker)}
\label{algo}
%In order to implement a PF algorithm, we need to evolve the state ``particles" using the system model and weight them by the observation likelihood at each time step. We first discuss how to implement (\ref{defhatct}) using the level set method and then explain the PF-MT algorithm \cite{pap1} for our problem. Finally, we explain how to detect and estimate the change in effective basis dimension.

We first explain a generic particle filtering (PF) algorithm \cite{gordon,mcip,tutorial}. A PF outputs at each time $n$, a cloud of $N$ particles, $\{ X_n^{i} \}$ with weights $\{ w_n^{i} \}$  whose empirical measure $\pi_n^N(X_n) \defn  \sum_{i=1}^N w_n^{i} \delta(X_n-X_n^{i}) $ closely approximates the true posterior, $\pi_n(X_n) \defn p(X_n|Y_{1:n})$. Here  $\delta(X-a)$ denotes the Dirac delta function at $a$. It starts with sampling $N$ times from $\pi_0$ at $n=0$ to approximate it by $\pi_0^N(X_0)$. For each $n>0$, it approximates the Bayes recursion for going from $\pi_{n-1}^N$ to $\pi_n^N$ using importance sampling. This consists of:
\ben
\item
 {\em Importance Sampling (IS):} Sample $X_n^{i} \sim q(X_n^{i})$, for $i=1,2...N$. The importance sampling density, $q$, can depend on $X_{n-1}^{i}$ and $Y_n$.
\item
 {\em Weighting:} Compute the  weights:  $w_n^{i} = \frac{\tilde{w}_n^{i}}{\sum_{j=1}^N \tilde{w}_n^{(j)} }$, where $\tilde{w}_n^{i} = w_{n-1}^{i} \frac{p(Y_n|X_n^{i}) p(X_n^{i}|X_{n-1}^{i})}{q(X_n^{i})}$.
\item
{\em Resampling:}   Replicate particles in proportion to their weights and reset $w_n^{i}$  \cite{tutorial}.
\een
Since the effective particle size decreases with increasing system noise dimension, direct application of PF becomes impractical for large dimensional problems. {\em We propose to replace the PF by the following: importance sample only on the effective basis dimensions, and replace the importance sampling step by a deterministic Mode Tracking (MT) step in the residual space \cite{pap1}.} This idea, which we call PF-MT, assumes that the effective basis dimension $K$ is large enough to ensure that Assumptions \ref{unimod} and \ref{ismt}, given below, hold \cite{pap1}.
\begin{ass}
The total residual deformation variance, $\Delta_{tot} = trace(\Sigma_r)$ is small enough so that the posterior in residual space, $p^{**,i}$ (defined below), is unimodal.
\bea
p^{**,i}(v_{n,r}) \sdefn p(v_{n,r}|v_{n,s}^i, \rho_n^i, X_{n-1}^i, Y_n) \nn \\
               %& \propto &    p(Y_n|v_{n,r}, \chat^i) p(v_{n,r}) \nn \\
                & \propto &  p(Y_n|\chat^i + B_rv_{n,r}\N) \ \n(v_{n,r};0,\Sigma_r) \nn \\
                 \sdefn \exp[-L^i(v_{n,r})]
\label{defL}
\eea
\label{unimod}
\end{ass}
When Assumption \ref{unimod} holds, one can use the following importance sampling strategy \cite{pap1}: sample $v_{n,s}^i$, $\rho_n^i$ from their state transition priors, $\n(A_sv_{n-1,s}^i, \Sigma_s)$, $\n(A_\rho \rho_{n-1}^i, \Sigma_\rho)$ respectively; compute $\chat^i$ using (\ref{defhatct}); and sample $v_{n,r}^i$ from a Gaussian approximation \cite{doucet}, denoted $\n(m_n^i, \Sigma_{IS}^i)$, to $p^{**,i}$ about its mode, $m_n^i$. Finally, compute $C_n^i$ using (\ref{defct}). Here
\bea
m_n^i \defn \arg \min_{v_{n,r}} L^i(v_{n,r}), \ \ \Sigma_{IS}^i \defn ( \nabla^2  L^i(v_{n,r}) )^{-1}
\label{modeval}
\eea
Now, by conditional variance identity \cite{stats}, $\E_{Y_n}[\Sigma_{IS}^i] \approx \E_{Y_n}[Variance(p^{**,i})] \le \Sigma_r$. Thus if the following assumption holds, we can replace importance sampling from $\n(m_n^i, \Sigma_{IS}^i)$ by \cite{pap1} deterministically setting $v_{n,r}^i = m_n^i$. We call this the Mode Tracking (MT) approximation.
\begin{ass}
The total residual deformation variance, $\Delta_{tot} = trace(\Sigma_r)$ is small enough, i.e. $\Delta_{tot} < \Delta_{tot,bnd}$, so that with high probability, there is little error in replacing a random sample from $\n(m_n^i, \Sigma_{IS}^i)$ by $m_n^i$.
%This justifies replacing importance sampling from a Gaussian approx to $p^{**,i}$ by the mode $m_n^i$ (Mode Tracking).
\label{ismt}
\end{ass}

Based on the above ideas, we develop the PF-MT algorithm for contour tracking \cite{cdc06}. We explain each step below and the approximations used to simplify the implementation. The exact stepwise algorithm is given in Algorithm \ref{pfmt} and the approximations are summarized in  Algorithm \ref{pfmtapprox}.% and its approximate version are


\subsection{Importance Sampling on Effective Basis Dimensions}
\label{lsm}
This involves sampling $v_{n,s}^i$ and $\rho_n^i$ from their state transition priors, $\n(A_sv_{n-1,s}^i, \Sigma_s)$ and $\n(A_\rho \rho_{n-1}^i, \Sigma_\rho)$ respectively and computing $\chat^i$ using (\ref{defhatct}), $\forall i=1,2,..N$. We implement (\ref{defhatct}) using the level set method.
The level set evolution  corresponding to contour evolution given by (\ref{defhatct}), is: $\tilde{\phi}_n^i(x) = \phi_{n-1}^i(x) + v_{extend}(x) ||\nabla_x \phi_{n-1}^i(x)||$ where $v_{extend}$ is the normal extension \cite{sethian1999,osher2003}  of $B_s(p) v_{n,s}^i + \N_{n-1}^T(p) \rho_n^i$ onto non-zero level sets. %Here $\phi_{n-1}^i$ is the level set function corresponding to $C_{n-1}^i$.
This implementation assumes that Assumption \ref{smallmotion} holds.
%This implementation assumes that:
%\begin{ass}
%The observation interval $\deltat$ is small enough (compared to $B_s v_{n,s} + \N_{n-1}^T \rho_n$) so that $\N_{n-1}$ is also approximately normal to $C_n$.
%\label{smallmotion}
%\end{ass}
If it does not hold (either $\deltat$ large or motion fast), then (\ref{defhatct}) will have to be  implemented using multiple iterations. If the narrowband level set method \cite{sethian1999,osher2003} is used, multiple iterations may be required to implement (\ref{defhatct}), depending on the velocity magnitude and the narrowband width. Since we do not evolve a PDE to convergence, CFL condition \cite{sethian1999,osher2003,sapiro} need not be satisfied.
%$B_s$ and its extension onto all level sets need to be computed at each step. This can be done without computing the zero level set (contour) for the geometric basis. For the parametric basis, (i) the contour needs to be computed at each step in order to compute $B_s$; (ii) it needs to always be traversed in the same order (say clockwise); (iii) starting point correspondence needs to be maintained; and (iv) x-y locations of the basis points need to be moved along with the contour using (\ref{moveknotlocs}).%  given in Appendix \ref{basischoiceapp} %which requires computing $\N$.

$B_s$ and its extension onto all level sets need to be computed at each step. This can be done without computing the zero level set (contour) for the geometric basis\footnote{assuming the requirement of normal extension velocities \cite{sethian1999,osher2003} is relaxed (in numerical implementation, this will only result in more frequent re-initialization of level set functions since embedded curves may not remain embedded \cite{sapiro}). If turning angle is used as the parameter, then one can directly get normal extension velocities at each point without computing the contour.}.
For the parametric basis, at each iteration, (i) the contour (zero level set) needs to be computed;  it needs to always be traversed in the same order (say clockwise); and starting point correspondence needs to be maintained;  (ii) the basis points need to be moved along with the contour using (\ref{moveknotlocs}) given in Appendix~\ref{basischoiceapp} and (iii) the B-spline interpolation functions need to be recomputed using the current arclength distance between the basis points. If basis points come too close or go too far, the basis needs to change.% as explained in Section \ref{basischange}.%x-y locations of
 %
%
% Note that $v_{extend} ||\nabla \phi||$ contains a term $B_{s,extend}(\phi_n) ||\nabla \phi_n || dW_{n,s}$ and the correct way to compute this is using the discrete approximation to the Stratonovich integral as explained in \cite{keriven}. This is because $dW_{n,s}$ is the differential of Brownian motion.

\input{pfmttv}



\subsection{Mode Tracking on Residual Space}
This involves computing the mode $m_n^i$ defined in (\ref{modeval}), setting $v_{n,r}^i=m_n^i$; and computing $C_n^i$ using (\ref{defct}), $\forall i =1,2..N$.  Computing $m_n^i$ and $C_n^i$ requires being able to compute $B_r$. But $B_r$ is the solution of $B_r B_r^T = I - B_s (B_s^T B_s)^{-1} B_s^T$. Since $B_s$ depends on $C_{n-1}^{i}$, it will need to be computed at each $n$ and for all  $i$, which is very expensive. By using some approximations, we avoid having to compute $B_r$.

Define $E(C_n) \defn -\log[p(Y_n|C_n)]$. We have shown \cite{pap1} that if Assumption \ref{unimod} holds,  $m_n^{i}$ can be computed by starting with $v_{n,r}=0$  as initial guess and running $k$ iterations  (for some $k$) of gradient descent to minimize $E(\chat^i + B_r v_{n,r})$ w.r.t. $v_{n,r}$. When $trace(\Sigma_r)$ is small (Assumption \ref{ismt} holds), maximum value of $k$ will also be small and a heuristic choice of $k$ suffices.  If we also allow change along $B_s$, the $k$ gradient descent iterations to minimize $E$ as a function of $v_{n,r}$ can be replaced by $k$  gradient descent iterations to minimize $E$ as a function of $C_n$ (skips the need to compute $B_r$). This approximation assumes that:
\begin{ass}
We replace (\ref{defct}), (\ref{defvtr}) by the following model:
\bea
C_n \se \chat + v_{n,r} \N(\chat), \   v_{n,r} \sim \n(0, \Sigma_r),  \ \Sigma_r= \Delta I  \ \ \
\label{approxdef}
\eea
%and assume that $\Sigma_r = \Delta I_{M_t}$.
\label{defctapprox}
\end{ass}
Gradient descent is implemented using the standard level set method\cite{sethian1999,osher2003}. We start with $\phi^{(1)} = \tilde{\phi}_n^i$ (level set function corresponding to  $\chat^i$) as initial guess and run $k$ iterations of gradient descent to minimize $E$, i.e. run $k$ iterations of the type $\phi^{(r+1)} = \phi^{(r)} + v_{extend} ||\nabla_x \phi^{(r)}||$ where $v_{extend}$ is normal extension \cite{sethian1999,osher2003} of $(\nabla_C E)$ onto non-zero level sets. The output after $k$ iterations is $\phi_n^i$ and its zero level set is $C_n^i$.


\subsection{Weighting and Resampling}
This involves computing the weights, $w_n^i$,  $\forall i =1,2..N$, and resampling \cite{tutorial}. $w_n^i$ is computed as:
\bea
w_n^i \se \frac{\tilde{w}_n^{i}}{\sum_{j=1}^N \tilde{w}_n^{j}}, \
\tilde{w}_n^{i} \defn w_{n-1}^{i} \frac{p(Y_n|C_n^{i}) \ \n(v_{n,r}^{i}; 0, \Sigma_r)}{\n(v_{n,r}^{i}; m_n^{i},  \Sigma_{IS}^{i})}. \ \ \ \ \ \
\label{compweights}
\eea
Using Assumption \ref{defctapprox}, the above only requires knowing $||v_{n,r}^{i}||^2$. Since in the mode tracking step we minimize directly over $C_n^i$, we never compute $v_{n,r}^i$. We can replace $||v_{n,r}^{i}||$  by any easily computable distance, $d$, between $C_n^{i}$ and $\chat^i$ (or between $\phi_n^i$ and $\tilde{\phi}_n^i$) without much error in practice. In our experiments, we use the set symmetric distance \cite{deformotion}.
Also, since $\E_{Y_n}[\Sigma_{IS}^i] \le \Sigma_r$, when $\Sigma_r$ is small, one can replace $\Sigma_{IS}^i$ by $\Sigma_r$.  This makes the denominator a constant (can be removed).  Thus, the weights can be computed as:
\beq
w_n^i = \frac{\tilde{w}_n^{i}}{\sum_{j=1}^N \tilde{w}_n^{j}}, \ \tilde{w}_n^{i} = w_{n-1}^{i} p(Y_n|C_n^{i}) \ e^{-\frac{d^2(C_n^i, \chat^i)}{\Delta}} \ \
\label{compweightsapprox}
\eeq

{\em The exact PF-MT method is summarized in Algorithm \ref{pfmt} and the approximations explained above are given in Algorithm \ref{pfmtapprox}.}


\subsection{Time-Varying Effective Basis: PF-MT-TV}
\label{basischange}
The effective basis dimension needs to be large enough so that the mode tracking approximation in residual space can be justified at each $n$, i.e. we need to satisfy Assumptions \ref{unimod} and \ref{ismt} at each $n$. If the contour length changes significantly, the number of basis points will need to be changed to satisfy these assumptions.
Assume in this section, that we know the maximum allowable value of the distance between consecutive basis points, $\alpha_s$, to ensure that $\Delta_{tot} <  \Delta_{tot,bnd}$. We explain how to choose $\alpha_s$ in Section \ref{spatfreq}.
%Let  $\alpha_s$ be the minimum distance between basis points needed to ensure that the total residual deformation, $\Delta_{tot}=trace(\Sigma_r)$, is small enough for the importance sampling-MT approximation to be valid.

%This is computed as explained in Section \ref{spatfreq}.correlation between the velocities at the different basis points is assumed to not depend on distance between them
% different basis points are assumed to be far enough so that the basis velocities are uncorrelated as explained in Section~\ref{learn}
 As the contour deforms, both its total length and arclength distance between consecutive basis points changes. For the parametric basis, there is a need to change effective basis if this distance becomes significantly smaller (starting to estimate noise)\footnote{Assumptions~\ref{unimod} and \ref{ismt} require $\Delta_{tot} < \Delta_{tot,bnd}$ which only translates to an upper bound on the distance between consecutive basis points, $\alpha_s$. But, in practice, if the distance between basis points becomes too small, the PF starts estimating noise (demonstrated in Fig.~\ref{Kvaryfigs}) because the velocities at the different basis points are assumed to be uncorrelated as explained in Section~\ref{learn}.  Thus, distance becoming too small also needs to be detected and corrected.} or significantly larger (residual deformation too large) than $\alpha_s$.
This is done as follows. Choose a $\alpha_{s,min} < \alpha_s$ and $\alpha_{s,max} > \alpha_s$.  We declare a need to change dimension, whenever the following occurs for ``most" (more than 50\%) of the contour particles: the arclength distance  between any two consecutive basis point locations exceeds $\alpha_{s,max}$ or goes below $\alpha_{s,min}$. We evaluate the new effective basis as follows: Compute $K = \lceil {L}/{\alpha_s} \rceil$ for the most likely contour particle.  Uniformly allocate the $K$ basis points on the arclength of all contour particles and compute the new effective basis functions. Note that in certain situations, $K$ may remain the same, but the basis points may just get placed uniform distance apart on arclength. When the effective basis changes,  the old velocity coefficients' vector, $v_{n,s}^{(i)}$, also needs to be projected into the new effective basis. In this paper, we show results for varying $K$ for only the parametric basis. Changing $\alpha_s$ and $K$ for the geometric basis is briefly discussed in Section \ref{learnchange}. The details are ongoing work.
 %In addition, the velocity variance in the new basis needs to be learnt using previously tracked deformation data.
%WRONG: Or it may be computed by interpolating the old vector of variances and then projecting into the new basis.
%

%For the {\em geometric basis}, one may need to choose non-uniform spacing of the angular knots in order to ensure uniform placement of knots along the arclength. The need to change effective basis is detected as follows: compute arclength locations of the angular knots (assuming they are unique). If the arclength distance between any two consecutive knots exceeds $\alpha_{s,max}$ or goes below $\alpha_{s,min}$ for ``most" (more than 50\%) contour particles, a change is needed. The angular coordinates of points chosen $\alpha_s$ distance apart on the arclength of the most likely contour are used as the new knot locations. This strategy will have to change if we consider the deformation to be a function of the angle and then compute its frequency response. We discuss some ideas in Section \ref{learnchange}.

%  These are used to compute  the new basis functions.
%When contour length increases, there will be a need to use more knots only if deformation frequency increases: use more knots in regions where def freq is high


The complete PF-MT algorithm with a Time-Varying effective basis (PF-MT-TV) is summarized in Algorithm \ref{pfmttv}. If the following assumptions hold, one {\em should be able to} show convergence of Algorithm \ref{pfmttv} with $N$ by extending standard results such as \cite{nadia}. Weaker assumptions are discussed in \cite{pap2}.
%
%\subsubsection{Convergence of Algorithm \ref{pfmttv} with $N$} \label{assums}
%Algorithm \ref{pfmttv} implicitly assumes the following.
\begin{ass}
Assume that there is
\ben
\item  No error in estimating the new effective basis dimension.% and the new basis knot locations in case of non-uniform knot allocation.
\label{noKerr}
\item No delay in detecting the need for effective basis change.\label{nodelay}
\item No error in projecting $v_{n,s}^{(i)}$ into the new basis.
\label{projectionerror}
\item PF-MT (Algorithm \ref{pfmt}) converges as $\Delta_{tot,bnd} \tends 0$
\een
\label{strong}
\end{ass}
%The first assumption above is very strong. Algorithm 2 of \cite{pap2} which uses modification of \cite{papa2}, can handle a weaker version of it.  The proofs are ongoing work.
% and if the mixing state transition kernel assumptions \cite{mcip} are satisfied




==> conclusions.tex <==
\section{Conclusions and Future Directions}
\label{conclusions} %p^*$ conditioned on  the effective basis, $X_{t,s}$
We have proposed the PF-EIS algorithm which applies the efficient importance sampling technique of \cite{doucet} to a part of the state space (denoted $X_{t,r}$) that has a unimodal $\pss(X_{t,r}) =p(X_{t,r}|X_{t,s}^i,X_{t-1}^i,Y_t)$. We have derived sufficient conditions (Theorem \ref{unimodthm}) to verify if this holds for given $X_{t,s}$ and $X_{t,r}$. PF-EIS can be applied to situations where OL is frequently multimodal (or unimodal at a false mode) and the STP is broad. We have shown through simulations that PF-EIS outperforms the algorithm of \cite{doucet} (PF-D) for such problems. %Also, both PF-EIS and the algorithm of \cite{doucet} greatly outperform the original PF \cite{gordon}.

 For large dimensional state space (LDSS) problems, if the variance of $\pss(X_{t,r})$ is small enough,  the EIS step for $X_{t,r}$ can be replaced by Mode Tracking (MT), i.e. by deterministically setting $X_{t,r}^i$ equal to the mode of $\pss$. This idea results in a huge reduction in importance sampling dimension and hence improves effective particle size, making PF practically implementable for LDSS. Depending on the problem at hand, a combination of PF-EIS and PF-MT (called PF-EIS-MT) can be used. We have shown extensive simulation results comparing PF-EIS and PF-MT with existing PF methods  for tracking spatially varying physical quantities using a network of sensors each of which has significant failure probability. We have also successfully used PF-MT for deformable contour tracking in \cite{cvpr05,cdc06} and for illumination tracking of moving objects \cite{kaleicassp}.
%(PF-Original, PF-Doucet and PF-Original-K dim)

%which can be understood as a generalization of \cite{doucet}

There are many open issues for generalizing/improving the unimodality result (Theorem \ref{unimodthm}).
It can directly be applied to static problems, e.g. problems that use importance sampling to approximate the posterior $p(X|Y)$. Also, it can be easily extended to situations where $\Sigma_r$ is non-diagonal or to where the residual state posterior is non-Gaussian (Assumption \ref{gausspxtr} does not hold) but its $-\log$ is strongly convex. Another useful extension will be to apply the result to test for unimodality of $p(X_{1:t,r}|X_{1:t,s}^i, Y_{1:t})$. {\em An important open issue, to make this result more practically useful, is to find conditions for unimodality of $\pss$ that can be verified a-priori.} Lastly, the result in its current form only handles certain types of outlier situations, more general situations need be studied.
 %outlier situations where OL is unimodal at the wrong mode but its $-\log$ is flat (or convex in some other way) at the true one, for e.g. Fig. \ref{kfpmtfail}(c). But other more general outlier situations need to be studied.
%Also, situations where only ``effective" unimodality (second mode is much much weaker than the dominant mode) will suffice and how to verify it need to be studied.
% (that do not depend on previous particles or on the observations)
% directly applicable to verify unimodality of $p^*$ to run PF-Doucet \cite{doucet} (which is actually a special case of PF-EIS with $K=0$). It is also
%``effective" unimodality is okay if the second mode is the bad one. If second mode is the good one, its a problem
%The unimodality result (Theorem \ref{unimodthm}) will be more practically useful, if it finds conditions that only ensure that $\pss$ is ``effectively" unimodal
%
%

Open issues for PF-MT (and PF-EIS-MT) are as follows. If the system model changes over time, the MT dimension will need to be changed on the fly. Preliminary ideas to do this are discussed in \cite{pap2}. Secondly, if all or most particles $[v_{t,s}^i, v_{t,r}^i]$ stick to a wrong region of state space somehow\footnote{because of the strong prior term, this will not happen often, will happen only if a sequence of bad observations occur},  future particles of $v_{t,s}^i$ may get back because of random sampling, but $v_{t,r}^i$ will take very long. This may result in loss of track. The problem will be much lesser if the dynamics of $v_{t,r}$ is either temporally independent or at least temporally stationary. Temporal independence is a valid model for problems where the state vector can be interpreted as a ``spatial signal"  (e.g. temperature in space or contour tracking) and the effective basis is velocity at a subsampled set of points \cite{cdc06}. {\em A third issue is to prove the experimentally observed fact that when $N$ is small, the MT approximation of IS results in smaller total error.} This effect is more pronounced when exact mode computation is replaced by approximate mode computation.
%study conditions required for convergence of the PF-MT as $N \tends \infty$ and as $\eps_1, \eps_2 \tends 0$. A more useful thing
% The PF-EIS-MT algorithm needs to be implemented and tested.
% (because of strong prior term and no random sampling)
 % This may be possible to show under the temporal independence assumption on $v_{t,r}$.
%Application specific techniques for doing this need to be developed.
%There are also many un-addressed issues for
%

Finally, PF-MT can be replaced by a modification of RB-PF \cite{chen_liu,gustaffson} if $f_r$ is linear and if one chooses to approximate OL by a Gaussian about the OL mode that is closest to the predicted previous state. Also, if $f_r$ is nonlinear, the KF in RB-PF may be replaced by an EKF.% and OL is Gaussian (or is approximated by a Gaussian about the OL mode that is closest to the predicted previous state).

%Modifications that make mode finding faster or approximate mode finding techniques need to be developed to make PF-EIS or PF-MT faster.


 %For such problems, the state change (temperature change or contour deformation) is usually approximately bandlimited (spatially) at a frequency much smaller than the sampling frequency of the sensors or the image and so the value of $K$ (computed using Nyquist criterion for the approximate bandwidth) is much smaller than $M$ \cite{cdc06}.
% Here the residual space is the space of for the difference of the true velocity from the interpolated velocity, which can easily be modeled as temporally i.i.d.

% If $\Sigma_r$ is even a bit larger or if a PF-MT particle sticks to a bad mode of $v_{t,r}$ it will not get out (because it does not importance sample) and will eventually result in loss of track. This problem will be much lesser if the dynamics of $v_{t,r}$ is either temporally independent or at least temporally stationary.


==> effbasis.tex <==

%\section{Choosing the Effective Basis and its Dimension, $K$}
\section{PF-EIS-MT and  Assumptions' Verification}
For LDSS tracking applications, a key question is the choice of the effective basis dimension $K$. In the most general case, $K$ may not remain fixed with time, but may be allowed to change.

\subsection{PF-EIS-MT}
As explained earlier, for best performance, one may choose a smaller dimensional $X_{t,r}$ for PF-MT than that for PF-EIS, i.e. split $X_{t,r}$ for PF-EIS into $X_{t,r,s}$ and $X_{t,r,r}$ and use the MT approximation only on $X_{t,r,r}$.  So we IS  $X_{t,s}$ from its STP, we EIS   $X_{t,r,s}$  from a Gaussian approximation to $\pss(X_{t,r,s},X_{t-1,r,r}^i)$ and we MT   $X_{t,r,r}$. This is summarized in Algorithm \ref{pfeismt}.
We can choose $X_{t,s}$  using knowledge about the problem and likely reasons for multimodality (or choose it on the fly as discussed in Section \ref{pfeismtassverify} and decide $\dim(X_{t,r,s}), \dim(X_{t,r,r})$  using (\ref{chooseK}) below. For example, in contour tracking if different contour modes are separated only by translation and scale, it may suffice to use only these as $X_{t,s}$. Similarly, in tracking physical quantities using sensor networks, multimodality occurs only at or near nodes which have sensors with high failure probabilities.


\subsection{Choice of $K$ to satisfy IS-MT and Unimodality Assumptions}
To ensure that IS-MT holds with a given $\eps_1$, $\eps_2$, i.e. to ensure that $Pr(||v_{t,r}^i - m_t^i|| > \eps_1) < \eps_2$, we need $\trace(\Sigma_r) \le \eps_1^2 \eps_2/M$ (Theorem \ref{ismtthm}). Thus for $\eps_1^2 = \gamma$\% of total variance ($\sum_{p=1}^M \Delta_p$), we need
to find the least $K$ s.t.
\bea
\ds \frac{\sum_{p=K+1}^M \Delta_p}{\sum_{p=1}^M \Delta_p } \le \frac{\gamma \eps_2}{100 M}
\label{chooseK}
\eea
When $B_s$ is chosen to be the eigen basis, $K$ is computed as follows. Compute the covariance of $[v_t - f_v(v_{t-1})]$ using training data and evaluate its eigenvectors and eigenvalues. $K$ is then chosen so the least integer s.t. the sum of residual eigenvalues, $\sum_{p=K+1}^M \Delta_p$, satisfies the above. If $B_s$ is the Fourier basis, the Power Spectral Density (PSD) replaces the eigenvalues. We compute the PSD of $[v_t - f_v(v_{t-1})]$ using training data and choose the minimum frequency (and a corresponding $K$) so that the residual sum of PSD values satisfies the above. This is demonstrated for contour tracking in \cite{cdc06}.
Note that  if the system model changes over time, $K$ will also need to change with time. This is demonstrated in the context of contour tracking in \cite{cdc06}.

%This can be understood as applying Nyquist criterion to an ``approximately" bandlimited signal.
%\subsection{Choice of $K$ to satisfy unimodality assumption}

 The unimodality assumption depends on the state particles and the current observation. Hence one would have to choose a $K$ to satisfy this assumption separately for each particle at each time. Alternatively, one can use heuristics (knowledge about the problem and likely reasons for multimodality) to guess a value of $K$ that works for most particles at most times (and this suffices in practice).

It is important to note that when trying to implement only the PF-MT algorithm (not PF-EIS or PF-EIS-MT), the choice of $K$ to satisfy IS-MT is, in most cases, more than sufficient to ensure that the unimodality assumption also holds.

\subsection{PF-EIS-MT with Assumption Verification}
\label{pfeismtassverify}
We summarize the algorithm that includes verifying unimodality assumption on the fly at each time and for each particle in  Algorithm \ref{pfeismtass}. It chooses a different $K < K_2$ for each particle at each $t$. Such an algorithm is practical  only if the importance sampling and weighting steps can be implemented in parallel for different particles. A more practical idea, may be to decide between two choices of $K$: use $K=0$ (PF-Doucet) if $p^*$ is unimodal for the current particle, else use PF-EIS with a predecided $K$.

%As explained earlier, for best performance, one can use a combination of PF-EIS and PF-MT, i.e. choose $X_{t,r}$ for PF-EIS that satisfies the unimodality assumption. This is done on the fly at each time and for each particle. But split this $X_{t,r}$ into $X_{t,r,s}$ and $X_{t,r,r}$ so that $K_2 = \dim([X_{t,s},X_{t,r,s}])$ satisfies the IS-MT assumption for a given $\gamma, \eps_2$. Then, importance sample from the STP for $X_{t,s}$, importance sample from a Gaussian approximation to $\pss$ for $X_{t,r,s}$ and use the Mode Tracking (MT) approximation for $X_{t,r,r}$ i.e. use the mode of $\pss$ as the new particle. The above algorithm (includes unimodality assumption verification for each $t$ and each $i$) is summarized in Algorithm \ref{pfeismtass}.



 %The algorithm with this modification is summarized in Algorithm \ref{pfeismtass}. This also assumes that $X_{t,r}$ for PF-EIS into $X_{t,r,s}$ and $X_{t,r,r}$ and use the MT approximation only on $X_{t,r,r}$.

\section{Other Practical Issues}
An important practical consideration is the type of effective basis $B_s$ (e.g. eigen, Fourier or B-spline). A second important issue is $\pss$ mode computation, which is the most expensive step in PF-EIS or PF-MT.

\subsection{Choice of Effective Basis}
 For applications where the LDSS dimension $M$ is fixed, and is not very large, and enough training data is available (to accurately estimate the eigenvectors), the eigen-basis should be used (due to its energy compaction property), i.e. $B_s$ should be the set of the top $K$ eigenvectors and $B_r$ should be its orthogonal complement. %This is because  eigen-basis has the its energy compaction property, i.e. it requires the smallest value of $K$ for a given residual error variance (and IS-MT requires choosing $K$ to ensure the residual error variance $\Delta_{K,tot}$ is less than a certain value).
   But for applications such as contour tracking where $M$ is not fixed, or if enough training data is not available (to reliably compute the eigenvectors of the estimated covariance matrix), eigen basis cannot be used.

In such cases, a Fourier basis (or equivalently an ideal interpolator) \footnote{Using the first $K$ Fourier coefficients is equivalent to using the ideal interpolator of the appropriate width}) is a better idea.
    It is worth mentioning that the DFT matrix is the eigenvectors of a periodic random sequence (e.g. contour deformation defined on a closed contour).??
    But both Fourier (or the ideal interpolator) and eigen will be inefficient for large $M$ since $B_s$ is not a sparse matrix. Fourier may be speeded up to some extent if FFT can be used, but this requires equally spaced data points for which DFT is applicable. Also, since $B_s$ is  a full matrix, neither of these can directly deal with spatially nonstationary data (e.g. contour deformation that requires a different value of $K$ in different contour regions).
% sinc function can be defined only for interpolating equally spaced basis points

Thus in many practical applications such as contour tracking it is more useful to replace the ideal interpolator with a non-ideal but local interpolator such as the B-spline (or cubic) interpolation functions. These are non-orthogonal bases and hence may require a larger value of $K$. Also they are not bandlimited. But because of their local control, $B_s$ is a sparse matrix. This makes them faster in implementation and also allows handling of spatially non-stationary data (allocate basis points at different spatial intervals in different regions, B-spline or cubic can interpolate across non-uniformly spaced basis points).

But choice of $K$ is faster to do using the Fourier (or eigen basis). This is because for any of the interpolation bases (sinc or B-spline or cubic), all basis directions, $B_s$, change when $K$ is changed. Hence, even though one uses the B-spline or cubic interpolator, choosing $K$ to satisfy IS-MT assumption is easier to do using the Fourier (or eigen) basis.





\subsection{Approximations for $\pss$ Mode Computation} %NOT NEEDED
Multiple heuristics can be used when the exact mode of $L^i$  is expensive to compute. Some of these may in fact even yield better results depending on the problem. The exact mode computation can be replaced by approximating it with a fixed number of gradient descent iterations.

Secondly, if the gradient of the distance term, $\nabla D$, is difficult to compute (this can occur when the STP of $X_{t,r}$ is not Gaussian), we can use $k$ iterations of gradient descent to minimize $E$ as an approximation to  $\pss$ mode computation. As shown in \cite{pap1}, under the assumptions of Theorem \ref{unimodthm}, if gradient descent is run slowly enough, there exists a value of $k$ for which the output will be the mode of of $L^i$ The  $k$ cannot be computed in practice, but a heuristic choice suffices.

 A third important approximation is needed in situations where $B_r$ is expensive to compute (e.g. for non-Euclidean problems like contour tracking where $B_s$ depends on the previous contour and hence needs to be computed for each previous contour particle at each $t$). In these cases, if $f_r(v_{t,r}) \equiv 0$ ($v_{t,r}$ assumed temporally independent), one can replace the first equation of (\ref{sysmod2}), by  $C_t = C_{t-1} + g_{C_{t-1}}( B_s v_{t,s} + v_{t,r} )$  for the purpose of mode computation. The variance of $v_{t,r}$ is assumed to be small in all dimensions and hence this only slightly modifies $C_t$ along $B_s$ (only a slight change from our original method). This and the previous approximation was used by us in \cite{cdc06,cvpr05}.
%Another  modification of the above idea is to  use the ori $[v_{t,s}, v_{t,r}]$. One may also choose to change $v_{t,s}^i$ from its sampled value to the value obtained after the minimization.
A related idea was used by authors of \cite{wormholes}, where they sampled $X_t$ in all dimensions from the STP and computed the OL mode (minimizer of $E$) starting with each particle as the initial guess. This resulted in all particles converging to one of the modes of OL.  This approach will fail  in case there is a sequence of bad or outlier observations (so all particles will converge to the outlier mode, resulting in loss of diversity).







==> figsNeff.tex <==

\begin{figure*}[b!]
\centerline{
\subfigure[$N_{eff}$, Avg LL for Fig. 3a]%\ref{pfeisnew2N100}]
{\label{NeffAvgLL1}
\begin{tabular}{c}
\psfig{file = \locc/unimod/PFEIS_new2/Neff_N100_iters40.eps, width=4.25cm,height=4cm} \\
\psfig{file = \locc/unimod/PFEIS_new2/AverageLL_N100_iters40.eps, width=4.25cm,height=4cm}
\end{tabular}
}
\hspace{-0.28in}
\subfigure[$N_{eff}$, Avg LL for Fig. 3b]%\ref{Ctsqr}]
{\label{NeffAvgLL2}
\begin{tabular}{c}
\psfig{file = \locc/unimod/newsims_sqr_A07/Neff_N50_iters50.eps, width=4.25cm,height=4cm} \\
\psfig{file = \locc/unimod/newsims_sqr_A07/AverageLL_N50_iters50.eps, width=4.25cm,height=4cm}
\end{tabular}
}
\hspace{-0.28in}
\subfigure[$N_{eff}$, Avg LL for Fig. 4a]%\ref{Ctsqr}]
{\label{NeffAvgLL3}
\begin{tabular}{c}
\psfig{file = \locc/unimod/newsims_PFMT3/Neff_N100_iters50.eps, width=4.25cm,height=4cm} \\
\psfig{file = \locc/unimod/newsims_PFMT3/AverageLL_N100_iters50.eps, width=4.25cm,height=4cm}
\end{tabular}
}
\hspace{-0.28in}
\subfigure[$N_{eff}$, Avg LL for Fig. 4b]%\ref{Ctsqr}]
{\label{NeffAvgLL4}
\begin{tabular}{c}
\psfig{file = \locc/unimod/newsims_PFMT_sqr_fail/Neff_N50_iters50.eps, width=4.25cm,height=4cm} \\
\psfig{file = \locc/unimod/newsims_PFMT_sqr_fail/AverageLL_N50_iters50.eps, width=4.25cm,height=4cm}
\end{tabular}
}
}
\caption{\small{Plotting the effective particle sizes ($N_{eff}$) and the Average LL (logarithm of the likelihood $p(Y_t|Y_{1:t-1})$ averaged over the all realizations). Please also look at the corresponding RMSE plots in Figs 3 and 4 of the manuscript. Note that $N_{eff}$ is a useful measure of performance, only when the RMSEs and Average LL are roughly equal. This is because $N_{eff}$ will be high even when all particles lie in a completely wrong region of the state space and all have near zero weights (resulting in very bad tracking performance). Also, Average LL in itself is also not a correct measure of performance always (see text).
}}
\label{NeffAvgLL}
\end{figure*} 

==> figsNeff_pap.tex <==

\begin{figure*}
\centerline{
\subfigure[$N_{eff}$, Avg LL for Fig. \ref{pfeisnew2N100}]
{\label{NeffAvgLL1}
\begin{tabular}{c}
\psfig{file = \locc/unimod/PFEIS_new2/Neff_N100_iters40.eps, width=4.25cm,height=4cm} \\
\psfig{file = \locc/unimod/PFEIS_new2/AverageLL_N100_iters40.eps, width=4.25cm,height=4cm}
\end{tabular}
}
\hspace{-0.28in}
\subfigure[$N_{eff}$, Avg LL for Fig. \ref{Ctsqr}]
{\label{NeffAvgLL2}
\begin{tabular}{c}
\psfig{file = \locc/unimod/newsims_sqr_A07/Neff_N50_iters50.eps, width=4.25cm,height=4cm} \\
\psfig{file = \locc/unimod/newsims_sqr_A07/AverageLL_N50_iters50.eps, width=4.25cm,height=4cm}
\end{tabular}
}
\hspace{-0.28in}
\subfigure[$N_{eff}$, Avg LL for Fig. \ref{pfmt3_N100fig}]
{\label{NeffAvgLL3}
\begin{tabular}{c}
\psfig{file = \locc/unimod/newsims_PFMT3/Neff_N100_iters50.eps, width=4.25cm,height=4cm} \\
\psfig{file = \locc/unimod/newsims_PFMT3/AverageLL_N100_iters50.eps, width=4.25cm,height=4cm}
\end{tabular}
}
\hspace{-0.28in}
\subfigure[$N_{eff}$, Avg LL for Fig. \ref{pfmtsqrfig}]
{\label{NeffAvgLL4}
\begin{tabular}{c}
\psfig{file = \locc/unimod/newsims_PFMT_sqr_fail/Neff_N50_iters50.eps, width=4.25cm,height=4cm} \\
\psfig{file = \locc/unimod/newsims_PFMT_sqr_fail/AverageLL_N50_iters50.eps, width=4.25cm,height=4cm}
\end{tabular}
}
}
\caption{\small{Plotting the effective particle sizes ($N_{eff}$) and the Average LL (logarithm of the likelihood $p(Y_t|Y_{1:t-1})$ averaged over the all realizations). Please also look at the corresponding RMSE plots in Figs \ref{pfeisfigs}, \ref{pfmtfigs}. Note that $N_{eff}$ is a useful measure of performance only when the RMSEs and Average LL are roughly equal. This is because $N_{eff}$ will be high even when all particles lie in a completely wrong region of the state space and all have near zero weights (resulting in very bad tracking performance). Also, Average LL in itself is also not a correct measure of performance always (see text).
}}
\label{NeffAvgLL}
\end{figure*} 

==> figscompare.tex <==
\begin{figure}
\centerline{
\begin{tabular}{ccc}
\hspace{-0.3in}
\psfig{file = \locc/unimod/pfeiscompareN40.eps, width=3.5cm,height=4cm} &
\hspace{-0.3in}
\psfig{file = \locc/unimod/pfmtcompareN40.eps, width=3cm,height=4cm} &
\hspace{-0.3in}
\psfig{file = \locc/unimod/pfmtcompareN20.eps, width=3.5cm,height=4cm} \hspace{-0.3in} \\
\hspace{-0.3in} (a) Examp \ref{example2},$N$=45 & \hspace{-0.3in} (b) Examp \ref{example3},$N$=40 \ & \hspace{-0.3in} (c) Examp \ref{example3},$N$=20
%(a) PF-EIS for $K=0,K_{sim},M$ & \hspace{-0.3in} (b) PF-MT, $N=40$ & \hspace{-0.3in} (c) PF-MT, $N=20$
%(a) uses 20 iterations, (b) used 15 iterations
\hspace{-0.3in}
\end{tabular}
}
\caption{{\small RMSE (root mean square error) of the tracked temperatures from true values.  RMSE is computed as square root of mean of squared norm of the error over 10 random simulations of the state space model.
(a): Comparing RMSE of PF-EIS with that of original PF\cite{gordon} and of PF-Doucet\cite{doucet} for Example \ref{example2}.
(b) and (c): Comparing RMSE of PF-MT with that of PF-$K$ dim, PF-EIS and original PF ($M$ dim) for Example \ref{example3}. (b): $N$=40 particles, (c): $N$=20 particles.
%Comparing RMSE of PF-EIS ($K=K_{sim}$)  with that of original PF ($K=M$) \cite{gordon} and of PF-Doucet ($K=0$)\cite{doucet}. RMSE is computed as square root of mean of squared norm of the state error over 20 random simulations of the state space model. We used  $K=K_{sim}=1$ for generating the observations. Also, $\sigma_{obs}^2 = 5$ and $p_f(y) = Unif(y;-100,100)$. $\Sigma_s, \Sigma_r$ is shown below each figure.
%
%Comparing PF-MT   with a K-dim PF (setting $v_{t,r} \equiv 0$), PF-EIS and PF-Original for an LDSS model with $K=3$ and $M=10$. Also, $\sigma_{obs}^2 = 5$, $p_f(y) = Unif(y;-10,10)$, $\Sigma_s = 25I_3$, $\Sigma_r =2.5 I_7$ and $[B_s \ B_r]$ was a randomly chosen $M \times M$ orthonormal matrix (not identity). RMSE is computed as square root of mean of squared norm of the state error over 10 random simulations of the state space model.
%%We used  $K=K_{sim}=1$ for generating the observations. Also, $\sigma_{obs}^2 = 5$ and $p_f(y) = Unif(y;-100,100)$ and $\Sigma_s = 25$, $\Sigma_r =2 I_4$. $\Sigma_s, \Sigma_r$ is shown below each figure.
}}
\label{pfeiscomp}
\end{figure}





%\begin{figure}
%\centerline{
%\begin{tabular}{cc}
%\psfig{file = \locc/unimod/pfeiscompareN40.eps, width=4cm,height=4cm} &
%\psfig{file = \locc/unimod/pfeiscompareN45.eps, width=4cm,height=4cm} \\
%%\psfig{file = \locc/unimod/pfeiscompareN100.eps, width=4cm,height=4cm} \\
%(a) $\Sigma_s = 10$, $\Sigma_r =2 I_4$    & (b) $\Sigma_s = 25$, $\Sigma_r =2 I_4$ %& (c) $\Sigma_s = 25$, $\Sigma_r =5 I_4$
%%(a) uses 20 iterations, (b) used 15 iterations
%\hspace{-0.3in}
%\end{tabular}
%}
%\caption{{\small
%Comparing RMSE of PF-EIS ($K=K_{sim}$)  with that of original PF ($K=M$) \cite{gordon} and of PF-Doucet ($K=0$)\cite{doucet}. RMSE is computed as square root of mean of squared norm of the state error over 20 random simulations of the state space model.
%We used  $K=K_{sim}=1$ for generating the observations. Also, $\sigma_{obs}^2 = 5$ and $p_f(y) = Unif(y;-100,100)$.
% $\Sigma_s, \Sigma_r$ is shown below each figure.
%}}
%\label{pfeiscomp}
%\end{figure}
%
%\begin{figure}
%\centerline{
%\begin{tabular}{cc}
%\psfig{file = \locc/unimod/pfmtcompareN40.eps, width=4cm,height=4cm} &
%\psfig{file = \locc/unimod/pfmtcompareN20.eps, width=4cm,height=4cm} \\
%%\psfig{file = \locc/unimod/pfeiscompareN100.eps, width=4cm,height=4cm} \\
%(a) $N=40$: PF-EIS best    & (b) $N=20$: PF-MT best
%\hspace{-0.3in}
%\end{tabular}
%}
%\caption{{\small
%Comparing PF-MT   with a K-dim PF (setting $v_{t,r} \equiv 0$), PF-EIS and PF-Original for an LDSS model with $K=3$ and $M=10$. Also, $\sigma_{obs}^2 = 5$, $p_f(y) = Unif(y;-10,10)$, $\Sigma_s = 25I_3$, $\Sigma_r =2.5 I_7$ and $[B_s \ B_r]$ was a randomly chosen $M \times M$ orthonormal matrix (not identity).
%RMSE is computed as square root of mean of squared norm of the state error over 10 random simulations of the state space model.
%%We used  $K=K_{sim}=1$ for generating the observations. Also, $\sigma_{obs}^2 = 5$ and $p_f(y) = Unif(y;-100,100)$ and $\Sigma_s = 25$, $\Sigma_r =2 I_4$. $\Sigma_s, \Sigma_r$ is shown below each figure.
%}}
%\label{pfmtcomp}
%\end{figure}




==> figseis.tex <==
\begin{figure*}
\centerline{
\begin{tabular}{cccc}
\psfig{file = \locc/unimod/PFEIS/mrmseN40.eps, width=4.5cm,height=4cm} &
\psfig{file = \locc/unimod/PFEIS/rmse099N40.eps, width=4.5cm,height=4cm} &
\psfig{file = \locc/unimod/PFEIS2/mrmseN40.eps, width=4.5cm,height=4cm} &
\psfig{file = \locc/unimod/PFEIS2/rmse099N40.eps, width=4.5cm,height=4cm} \\
(a) Mean, PFEIS & (b) Worst, PFEIS & (c) Mean, PFEIS2 & (d) Worst PFEIS2
\end{tabular}
}
\caption{{\small Comparing PF-EIS with PF-Doucet and PF-Original. Plot of average and worst case Euclidean norm of the error the tracked temperatures from true values over time.
}}
\label{pfeis12}
\end{figure*}



\begin{figure*}
\centerline{
\begin{tabular}{cccc}
\psfig{file = \locc/unimod/PFEIS_new2/mrmseN40.eps, width=4.5cm,height=4cm} &
\psfig{file = \locc/unimod/PFEIS_new2/rmse099N40.eps, width=4.5cm,height=4cm} &
\psfig{file = \locc/unimod/PFEIS_new2/mrmseN100.eps, width=4.5cm,height=4cm} &
\psfig{file = \locc/unimod/PFEIS_new2/rmse099N100.eps, width=4.5cm,height=4cm} \\
(a) Mean, N=40 PFEISnew2 & (b) Worst, N=40 PFEISnew2 & (c) Mean, N=100 PFEISnew2 & (d) Worst, N=100 PFEISnew2
\end{tabular}
}
\caption{{\small Comparing PF-EIS with PF-Doucet and PF-Original. Plot of average and worst case Euclidean norm of the error the tracked temperatures from true values over time. The worst case values are very high (linearly increasing) and almost equal for all algorithms.
}}
\label{pfeisnew2}
\end{figure*}

\begin{figure*}
\centerline{
\begin{tabular}{cccc}
\psfig{file = \locc/unimod/PFEIS_new3_addCt/mrmseN40.eps, width=4.5cm,height=4cm} &
\psfig{file = \locc/unimod/PFEIS_new3_addCt/rmse099N40.eps, width=4.5cm,height=4cm} &
\psfig{file = \locc/unimod/PFEIS_new3_addCt/mrmseN100.eps, width=4.5cm,height=4cm} &
\psfig{file = \locc/unimod/PFEIS_new3_addCt/rmse099N100.eps, width=4.5cm,height=4cm} \\
(a) Mean, N=40 PFEISnew3addCt & (b) Worst, N=40 PFEISnew3addCt& (c) Mean, N=100 PFEISnew3addCt & (d) Worst, N=100 PFEISnew3addCt
\end{tabular}
}
\caption{{\small Comparing PF-EIS with PF-Doucet and PF-Original. Plot of average and worst case Euclidean norm of the error the tracked temperatures from true values over time. The mean error for N=40 are almost equal (and both very low) for PF-D and PF-EIS. NOT NEEDED
}}
\label{pfeisnew3}
\end{figure*}


\begin{figure*}
\centerline{
\begin{tabular}{cccc}
%\psfig{file = \locc/unimod/PFMT2/correctpfmt_mrmseN20.eps, width=4.5cm,height=4cm} &
%\psfig{file = \locc/unimod/PFMT2/pfmt_rmse099N20.eps, width=4.5cm,height=4cm} &
%(a) RMSE, N=20 PFMT2 & (b) Worst, N=20 PFMT2 &
\psfig{file = \locc/unimod/PFMT2/correctpfmt_mrmseN50.eps, width=4.5cm,height=4cm} &
\psfig{file = \locc/unimod/PFMT2/pfmt_rmse099N50.eps, width=4.5cm,height=4cm} &
\psfig{file = \locc/unimod/PFMT1/correctpfmt_mrmseN50.eps, width=4.5cm,height=4cm} &
\psfig{file = \locc/unimod/PFMT1/pfmt_rmse099N50.eps, width=4.5cm,height=4cm} \\
(a) RMSE, N=50 PFMT2 & (b) Worst, N=50 PFMT2 & (c) RMSE, N=50 PFMT1 & (b) Worst, N=50 PFMT1
\end{tabular}
}
\caption{{\small  Comparing RMSE of PF-MT with that of PF-$K$ dim, PF-EIS and original PF ($M$ dim). Plot of RMSE and worst case error norm of the tracked temperatures from true values over time.
}}
\label{pfmt2}
\end{figure*}

\begin{figure}
\centerline{
\begin{tabular}{cc}
\psfig{file = \locc/unimod/pfmtcompareN40.eps, width=4.5cm,height=4cm} &
\psfig{file = \locc/unimod/pfmtcompareN20.eps, width=4.5cm,height=4cm} \hspace{-0.3in} \\
 (a) Examp \ref{example3},$N$=40  &  (b) Examp \ref{example3},$N$=20
%(a) PF-EIS for $K=0,K_{sim},M$ & \hspace{-0.3in} (b) PF-MT, $N=40$ & \hspace{-0.3in} (c) PF-MT, $N=20$
%(a) uses 20 iterations, (b) used 15 iterations
\hspace{-0.3in}
\end{tabular}
}
\caption{{\small RMSE (root mean square error) of the tracked temperatures from true values.
%RMSE is computed as square root of mean of squared norm of the error over 10 random simulations of the state space model.
 Comparing RMSE of PF-MT with that of PF-$K$ dim, PF-EIS and original PF ($M$ dim) for Example \ref{example3}. (b): $N$=40 particles, (c): $N$=20 particles.
}}
\label{pfmtold}
\end{figure} 

==> figseisbiased.tex <==
\begin{figure*}
\centerline{
\begin{tabular}{cccccc}
\psfig{file = \locc/unimod/BiasCtby2_M1/iter5histt6.eps, width=4.5cm,height=4.5cm} &
\psfig{file = \locc/unimod/BiasCtby2_M1/iter5histt7.eps, width=4.5cm,height=4.5cm} &
%\psfig{file = \locc/unimod/BiasCtby2_M1/iter5histt8.eps, width=4.5cm,height=4.5cm} &
\psfig{file = \locc/unimod/BiasCtby2_M1/iter5totbad1.eps, width=2.5cm,height=4.5cm} &
\psfig{file = \locc/unimod/BiasCtby2_M1/iter5EL_t7_i1_K0.eps, width=2.5cm,height=4.5cm} &
\psfig{file = \locc/unimod/BiasCtby2_M1/iter5Error.eps, width=2.5cm,height=4.5cm} \\
%(a) Histogram, t=6 & (b) Histogram, t=7 & (c) Histogram, t=8 & (d) K=0:Violating Ass. \ref{unimodass} & (e) K=0: E, L & (f) Error
(a) Histogram, t=6 & (b) Histogram, t=7 &  (c) K=0:Violating Ass. \ref{unimodass} & (d) K=0: E, L & (e) Error
\end{tabular}
}
\caption{{\small  Analyzing PF-D and PF-EIS (same as PF-Orig) for M=1. (a),(b),(c): Histogram of particles at t=6,7,8. With PF-Doucet (K=0) slowly all cluster around the wrong mode. (d): PF-Doucet: \% of particles of $C_{t-1}$ with bimodal $p^*$. Most of these $C_{t-1}$ particles are near the WRONG mode of $p^*$. (f) E and L for an example particle $C_{t-1}^i$ at t=7,i=1. The correct mode is the larger magnitude $Y_t$ while  dominant mode of $p^*$ is the wrong one. }}
\label{pfeisprocess}
\end{figure*}

\begin{figure*}
\centerline{
\begin{tabular}{cccccc}
\psfig{file = \locc/unimod/BiasCtby2_alpha01_M3/iter10histt6.eps, width=4.5cm,height=4.5cm} &
\psfig{file = \locc/unimod/BiasCtby2_alpha01_M3/iter10histt7.eps, width=4.5cm,height=4.5cm} &
%\psfig{file = \locc/unimod/BiasCtby2_alpha01_M3/iter10histt8.eps, width=4.5cm,height=4.5cm} &
\psfig{file = \locc/unimod/BiasCtby2_alpha01_M3/iter10totbad1.eps, width=2.5cm,height=4.5cm} &
\psfig{file = \locc/unimod/BiasCtby2_alpha01_M3/iter10EL_t6_i1_K0.eps, width=2.5cm,height=4.5cm} &
\psfig{file = \locc/unimod/BiasCtby2_alpha01_M3/iter10Error.eps, width=2.5cm,height=4.5cm} \\
%(a) Histogram, t=6 & (b) Histogram, t=7 & (c) Histogram, t=8 & (d) K=0:Violating Ass. \ref{unimodass} & (e) K=0: E, L & (f) Error
(a) Histogram, t=6 & (b) Histogram, t=7 &  (c) K=0:Violating Ass. \ref{unimodass} & (d) K=0: E, L & (e) Error
\end{tabular}
}
\caption{{\small  Analyzing PF-D and PF-EIS for M=3. (a),(b),(c): Histogram of particles at t=6,7,8. With PF-Doucet (K=0) slowly all cluster around the wrong mode. (d): PF-Doucet: \% of particles of $C_{t-1}$ with bimodal $p^*$. Most of these $C_{t-1}$ particles are near the WRONG mode of $p^*$. (f) E and L for an example particle $C_{t-1}^i$ at t=7,i=1. The correct mode is the larger magnitude $Y_t$ while  dominant mode of $p^*$ is the wrong one. }}
\label{pfeisprocess2}
\end{figure*}


\begin{figure*}
\centerline{
\begin{tabular}{cccc}
\psfig{file = \locc/unimod/BiasCtby2_M1/rmseN20.eps, width=4.5cm,height=4cm} &
\psfig{file = \locc/unimod/BiasCtby2_M1/worstN20.eps, width=4.5cm,height=4cm} &
\psfig{file = \locc/unimod/BiasCtby2_M1/rmseN100.eps, width=4.5cm,height=4cm} &
\psfig{file = \locc/unimod/BiasCtby2_M1/worstN100.eps, width=4.5cm,height=4cm} \\
(a) Mean, N=20 & (b) Worst, N=20 & (c) Mean, N=100 & (d) Worst, N=100
\end{tabular}
}
\caption{{\small Comparing PF-EIS with PF-Doucet and PF-Original for K=1, M=1. Plot of RMSE and worst case error of the tracked temperatures from true values over time.
}}
\label{pfeisM1}
\end{figure*}


\begin{figure*}
\centerline{
\begin{tabular}{cccc}
\psfig{file = \locc/unimod/biasCtby2_alpha01_M3/rmseN20_alpha01.eps, width=4.5cm,height=4cm} &
\psfig{file = \locc/unimod/biasCtby2_alpha01_M3/worstN20_alpha01.eps, width=4.5cm,height=4cm} &
\psfig{file = \locc/unimod/biasCtby2_alpha01_M3/rmseN100_alpha01.eps, width=4.5cm,height=4cm} &
\psfig{file = \locc/unimod/biasCtby2_alpha01_M3/worstN100_alpha01.eps, width=4.5cm,height=4cm} \\
(a) Mean, N=20 & (b) Worst, N=20 & (c) Mean, N=100 & (d) Worst, N=100
\end{tabular}
}
\caption{{\small Comparing PF-EIS with PF-Doucet and PF-Original for K=1, M=3. Plot of RMSE and worst case error of the tracked temperatures from true values over time.
}}
\label{pfeisM3}
\end{figure*}



\begin{figure*}
\centerline{
\begin{tabular}{cccc}
\psfig{file = \locc/unimod/biasCtby2_thm1_M3/rmseN20.eps, width=4.5cm,height=4cm} &
\psfig{file = \locc/unimod/biasCtby2_thm1_M3/worstN20.eps, width=4.5cm,height=4cm} &
\psfig{file = \locc/unimod/biasCtby2_thm1_M3/rmseN40.eps, width=4.5cm,height=4cm} &
\psfig{file = \locc/unimod/biasCtby2_thm1_M3/worstN40.eps, width=4.5cm,height=4cm} \\
(a) Mean, N=20 & (b) Worst, N=20 & (c) Mean, N=40 & (d) Worst, N=40
\end{tabular}
}
\caption{{\small Theorem \ref{unimodthm} satisfied with $\Delta^*=\infty$. Comparing PF-EIS with PF-Doucet and PF-Original for K=1, M=3. Plot of RMSE and worst case error of the tracked temperatures from true values over time.
}}
\label{pfeisM3}
\end{figure*} 

==> figsfinal.tex <==
\begin{figure*}
\subfigure[(top) Error, (bottom) no. of particles of PF-D with $\Delta^* < \Delta_1=10$]%, i.e. for which $p^*$ may be bimodal]
{\label{process_error}
%\psfig{file = \locc/unimod/BiasCtby2_M1/iter5Error.eps, width=2cm,height=2.5cm}
\psfig{file = \locc/unimod/BiasCtby2_M1/iter5_Error_totbad1.eps, width=4.25cm,height=4.5cm}
}
\hspace{0.01in}
\subfigure[$E,-\log p^*$ for a PF-D  particle with $\Delta^*=6.2 < \Delta_1$]
{\label{process_totbad1}
%\psfig{file = \locc/unimod/BiasCtby2_M1/iter5_totbad1_EL_t7ii_K0.eps, width=4.5cm,height=4.5cm}
\psfig{file = \locc/unimod/BiasCtby2_M1/iter5EL_t7_i1_K0.eps, width=4cm,height=4.5cm}
}
\hspace{0.01in}
%\subfigure[Histogram of $C_t$ particles, t=6. (top) PF-D, (bottom) PF-EIS]
%{\label{processhist6}
%\psfig{file = \locc/unimod/BiasCtby2_M1/iter5histt6.eps, width=4cm,height=4.5cm}
%}
\subfigure[Histogram of $C_t$ particles, t=7. (top) PF-D, (bottom) PF-EIS. $Y_{t}^{1,2}=9.0, 17.4$]
{\label{processhist7}
\psfig{file = \locc/unimod/BiasCtby2_M1/iter5histt7.eps, width=4cm,height=4.5cm}
}
\hspace{0.01in}
\subfigure[Histogram of $C_t$ particles, t=8. (top) PF-D, (bottom) PF-EIS. $Y_{t}^{1,2}=22.8, 22.8$]
{\label{processhist8}
\psfig{file = \locc/unimod/BiasCtby2_M1/iter5histt8.eps, width=4cm,height=4.5cm}
}
\caption{{\small Comparing PF-D (red-*) and PF-EIS (black-$\triangle$), which is same as PF-Orig for $M=1$, for a realization of Example \ref{biasctby2m1} with $M=1,K=1$.
Fig \ref{process_error} (top): Norm (here absolute value) of the error between the true between the true temperature values, $C_t$ and the tracked ones (PF estimate of $\E[C_t|Y_{1:t}]$) for PF-EIS and for PF-D; (bottom): Number of particles of PF-D at each $t$ for which $\Delta^* < \Delta_1=10$, i.e. for which $p^*$ may be bimodal.
Fig \ref{process_totbad1}:  $E,-\log p^*$ for a particle of PF-D at $t=7$, with $\Delta^*=6.2 < \Delta_1$.
Fig. \ref{processhist7}, \ref{processhist8}: histograms of $C_t$ particles  of PF-D (top) and of PF-EIS (bottom) at t=7,8.
%Fig. \ref{processhist6}, \ref{processhist7}, \ref{processhist8}: histograms of $C_t$ particles at t=6,7,8  for PF-D (top) \& PF-EIS (bottom).
% Histogram of particles at t=6,7,8. With PF-Doucet (K=0) slowly all cluster around the wrong mode.
%(d): PF-Doucet: \% of particles of $C_{t-1}$ with bimodal $p^*$. Most of these $C_{t-1}$ particles are near the WRONG mode of $p^*$. (f) E and L for an example particle $C_{t-1}^i$ at t=7,i=1. The correct mode is the larger magnitude $Y_t$ while  dominant mode of $p^*$ is the wrong one. }}
}}
\label{pfeisprocess}
\end{figure*}


\begin{figure*}
\begin{center}
\subfigure[(top) error, (bottom) no. of particles of PF-EIS (PF-D) for which $\pss$ ($p^*$) may be bimodal.]
%with $\Delta^*(X_{t-1}^i,v_{t,s}^i,Y_t) < \max_p \Delta_{p+1} =2$, no. of particles of PF-D (red -*) with $\Delta^*(X_{t-1}^i,Y_t)(v_{t,s}) < \max_p \Delta_p =10$]
%$p^*$  bimodal as a function of $v_{t,s}$ only, $\pss(v_{t,r})$ bimodal]%\% of particles with $\Delta^* < \max_{p} \Delta_{p+K}$ (black -$\triangle$)
{\label{process3_error_totbad1}
\psfig{file = \locc/unimod/BiasCtby2_alpha01_M3/iter10_Error_totbad1.eps, width=4.25cm,height=4.5cm}
}
\hspace{0.01in}
\subfigure[Histgrm of $C_{t,1}$ particles, t=6. (top) PF-D, (bottom) PF-EIS. $Y_{t,1}^{1,2}=-13.0,-25.8$]
{\label{process3hist6}
\psfig{file = \locc/unimod/BiasCtby2_alpha01_M3/iter10histt6.eps, width=4cm,height=4.5cm}
}
\hspace{0.01in}
\subfigure[Histgrm of $C_{t,1}$ particles, t=7. (top) PF-D, (bottom) PF-EIS. $Y_{t,1}^{1,2}=-14.2,-28.5$]
{\label{process3hist7}
\psfig{file = \locc/unimod/BiasCtby2_alpha01_M3/iter10histt7.eps, width=4cm,height=4.5cm}
}
\hspace{0.01in}
\subfigure[Histgrm of $C_{t,1}$ particles, t=8. (top) PF-D, (bottom) PF-EIS. $Y_{t,1}^{1,2}=-30.9,-32.3$]
{\label{process3hist8}
\psfig{file = \locc/unimod/BiasCtby2_alpha01_M3/iter10histt8.eps, width=4cm,height=4.5cm}
}
\end{center}
\caption{{\small
Comparing PF-D (red-*) and PF-EIS (black-$\triangle$) for a realization of Example \ref{biasctby2alpha01m3} with $M=3,K=1$.
Fig \ref{process3_error_totbad1}: (top) Norm of the error between the true between the true temperature values, $C_t$ and the tracked ones (PF estimate of $\E[C_t|Y_{1:t}]$) for PF-EIS and for PF-D; (bottom) Number of particles of PF-EIS (black -$\triangle$) with $\Delta^*(X_{t-1}^i,v_{t,s}^i,Y_t) < \max_p \Delta_{p+1} =2$ \ ($\pss(v_{t,r})$ may be bimodal for these particles), and number of particles of PF-D (red -*) with $\Delta^*(X_{t-1}^i,Y_t)(v_{t,s}) < \max_p \Delta_p =10$ \ ($p^*$ may be bimodal as a function of $v_{t,s}$ for these particles). Note for PF-D we  computed a $\Delta^*$, s.t. $\Delta < \Delta^*$ ensures unimodality of $p^*(v_{t,s},v_{t-1,r}^i)$.
Fig. \ref{process3hist6}, \ref{process3hist7}, \ref{process3hist8}: histograms of $C_{t,1}$ particles  of PF-D (top) and of PF-EIS (bottom)  at t=6,7,8.
%
% $p^*$ bimodal as a function of $v_{t,s}$ only ($v_{t,r}$ kept fixed at $v_{t-1,r}^i$) and number of particles of PF-EIS (black -$\triangle$) with $\pss$ bimodal as a function of $v_{t,r}$. As can be seen $\pss$ is multimodal very few times: for only 5 particles at t=4 and 2 particles at t=11, while $p^*$ is bimodal as a function of $v_{t,s}$ much more often. Note the above will give an exact number of cases where $p^*$ is multimodal only if $[B_s, B_r] = I$. %In the current example this is only a heuristic.
%Analyzing PF-D and PF-EIS for M=3. (a),(b),(c): Histogram of particles at t=6,7,8. With PF-Doucet (K=0) slowly all cluster around the wrong mode. (d): PF-Doucet: \% of particles of $C_{t-1}$ with bimodal $p^*$. Most of these $C_{t-1}$ particles are near the WRONG mode of $p^*$. (f) E and L for an example particle $C_{t-1}^i$ at t=7,i=1. The correct mode is the larger magnitude $Y_t$ while  dominant mode of $p^*$ is the wrong one. }}
}}
\label{pfeisprocess3}
\end{figure*}



\begin{figure*}
\begin{center}
%\subfigure[Example \ref{biasctby2m1}, N=20]%N=100]
%{\label{biasctby2m1fig}
%%\psfig{file = \locc/unimod/BiasCtby2_M1/rmseN100.eps, width=4cm,height=4cm}
%\psfig{file = \locc/unimod/biasCtby2_thm1_M3/rmseN20.eps, width=4cm,height=4cm}
%}
\subfigure[Example \ref{biasctby2thm1m3}, N=40]
{\label{biasctby2thm1m3fig}
\psfig{file = \locc/unimod/biasCtby2_thm1_M3/rmseN40.eps, width=4cm,height=4cm}
}
\subfigure[Example \ref{biasctby2alpha01m3}, N=20]
{\label{biasctby2alpha01m3fig1}
\psfig{file = \locc/unimod/biasCtby2_alpha01_M3/rmseN20_alpha01.eps, width=4cm,height=4cm}
}
%\subfigure[Example \ref{biasctby2alpha01m3}, N=100]
%{\label{biasctby2alpha01m3fig2}
%\psfig{file = \locc/unimod/biasCtby2_alpha01_M3/rmseN100_alpha01.eps, width=4cm,height=4cm}
%}
%\subfigure[Example \ref{pfeis12new2}(i), N=40]
%{\label{nobias1fig}
%\psfig{file = \locc/unimod/PFEIS/mrmseN40.eps, width=4cm,height=4cm}
%}
\subfigure[Example \ref{pfeis2}, N=40]
{\label{nobias2fig}
\psfig{file = \locc/unimod/PFEIS2/mrmseN40.eps, width=4cm,height=4cm}
}
\subfigure[Example \ref{pfeisnew2}, N=100]
{\label{nobias3fig1}
\psfig{file = \locc/unimod/PFEIS_new2/mrmseN100.eps, width=4cm,height=4cm}
}
%\subfigure[Example  \ref{pfeis12new2}(iii), N=100]
%{\label{nobias3fig2}
%\psfig{file = \locc/unimod/PFEIS_new2/mrmseN100.eps, width=4cm,height=4cm}
%}
\end{center}
\caption{{\small
Comparing RMSE (root mean squared error) of PF-EIS (black-$\triangle$) with that of PF-D (red-*) and PF-Orig (magenta-o).
RMSE is computed by taking the square root of the average (over 30 realizations) of the squared error norm
between the true temperature values, $C_t$ and the tracked ones (PF estimate of $\E[C_t|Y_{1:t}]$).
State dimension $M=3$ and effective basis dim $K=1$. PF-EIS ($K=1$),  outperforms both PF-D ($K=0$) and PF-Orig ($K=M$).
%State dimension $M=1$ and effective basis dim $K_{sim}=1$ for the first figure. $M=3$ and $K_{sim}=1$ in the last three figures.
}}
\label{pfeisbias}
\end{figure*}

\begin{figure*}
\begin{center}
\subfigure[Example  \ref{pfmtbias}, N=20]
{\label{pfmtbiasfig1}
%\psfig{file = \locc/unimod/pfmtbiasN20rmse.eps, width=4cm,height=4cm} %5 iterations version
\psfig{file = \locc/unimod/PFMT_biasctby2_all/rmseN20.eps, width=4cm,height=4cm} % 25 iterations version
}
\subfigure[Example \ref{pfmtbias}, N=50]
{\label{pfmtbiasfig2}
%\psfig{file = \locc/unimod/pfmtbiasN20rmse.eps, width=4cm,height=4cm} %5 iterations version
\psfig{file = \locc/unimod/PFMT_biasctby2_all/rmseN50.eps, width=4cm,height=4cm} % 25 iterations version
}
\subfigure[Example  \ref{pfmt12}, N=50]
{\label{pfmt12fig}
\psfig{file = \locc/unimod/PFMT2/correctpfmt_mrmseN50.eps, width=4cm,height=4cm}
}
\subfigure[Example  \ref{pfmtold}, N=20]
{\label{pfmtoldfig1}
\psfig{file = \locc/unimod/pfmtcompareN20.eps, width=4cm,height=4cm}
}
%\subfigure[Example  \ref{pfmtold}, N=40]
%{\label{pfmtoldfig2}
%\psfig{file = \locc/unimod/pfmtcompareN40.eps, width=4cm,height=4cm}
%}
\end{center}
\caption{{\small
Comparing RMSE (root mean squared error) of  PF-MT (blue-$\square$) with that of  PF-D (red-*), PF-EIS (black-$\triangle$), PF-Orig (magenta-o) and PF-K dim (green-x). State dimension $M=10$. $K=1$ for all except the last figure where $K=3$. Since $N$ is small compared to the dimension $M=10$, PF-MT has the best performance. If $N$ is increased, PF-EIS or PF-D will have better performance.
%For large dimensions (and small $N$ compared to the dimension),
%Use only pfmtbias and pfmtold. Show N=20,50 for pfmtbias N=20,40 for pfmtold
}}
\label{pfmtfigs}
\end{figure*}




%\begin{figure*}
%\begin{center}
%\subfigure[Example \ref{pfeis12new2}(i), N=40]
%{\label{nobias1fig}
%\psfig{file = \locc/unimod/PFEIS/mrmseN40.eps, width=4cm,height=4cm}
%}
%\subfigure[Example \ref{pfeis12new2}(ii), N=40]
%{\label{nobias2fig}
%\psfig{file = \locc/unimod/PFEIS2/mrmseN40.eps, width=4cm,height=4cm}
%}
%\subfigure[Example \ref{pfeis12new2}(iii), N=40]
%{\label{nobias3fig1}
%\psfig{file = \locc/unimod/PFEIS_new2/mrmseN40.eps, width=4cm,height=4cm}
%}
%\subfigure[Example  \ref{pfeis12new2}(iii), N=100]
%{\label{nobias3fig2}
%\psfig{file = \locc/unimod/PFEIS_new2/mrmseN100.eps, width=4cm,height=4cm}
%}
%\end{center}
%\caption{{\small Comparing PF-EIS with PF-D and PF-Orig.
%State dimension $M=3$ and effective basis dim $K_{sim}=1$.
%PF-EIS ($K=1$) outperforms both PF-D ($K=0$) and PF-Orig ($K=M$).
%%Plot of RMSE and worst case error of the tracked temperatures from true values over time.
%}}
%\label{pfeisnobias}
%\end{figure*}



==> figsnew.tex <==


\begin{figure*}
\begin{center}
\subfigure[(top) error, (bottom) no. of particles of PF-EIS (PF-D) for which $\pss$ ($p^*$) may be bimodal.]
%with $\Delta^*(X_{t-1}^i,v_{t,s}^i,Y_t) < \max_p \Delta_{p+1} =2$, no. of particles of PF-D (red -*) with $\Delta^*(X_{t-1}^i,Y_t)(v_{t,s}) < \max_p \Delta_p =10$]
%$p^*$  bimodal as a function of $v_{t,s}$ only, $\pss(v_{t,r})$ bimodal]%\% of particles with $\Delta^* < \max_{p} \Delta_{p+K}$ (black -$\triangle$)
{\label{process3_error_totbad1}
\psfig{file = \locc/unimod/BiasCtby2_alpha01_M3/iter10_Error_totbad1.eps, width=4.25cm,height=4.5cm}
}
\hspace{0.01in}
\subfigure[Histgrm of $C_{t,1}$ particles, t=6. (top) PF-D, (bottom) PF-EIS. $Y_{t,1}^{1,2}=-13.0,-25.8$]
{\label{process3hist6}
\psfig{file = \locc/unimod/BiasCtby2_alpha01_M3/iter10histt6.eps, width=4cm,height=4.5cm}
}
\hspace{0.01in}
\subfigure[Histgrm of $C_{t,1}$ particles, t=7. (top) PF-D, (bottom) PF-EIS. $Y_{t,1}^{1,2}=-14.2,-28.5$]
{\label{process3hist7}
\psfig{file = \locc/unimod/BiasCtby2_alpha01_M3/iter10histt7.eps, width=4cm,height=4.5cm}
}
\hspace{0.01in}
\subfigure[Histgrm of $C_{t,1}$ particles, t=8. (top) PF-D, (bottom) PF-EIS. $Y_{t,1}^{1,2}=-30.9,-32.3$]
{\label{process3hist8}
\psfig{file = \locc/unimod/BiasCtby2_alpha01_M3/iter10histt8.eps, width=4cm,height=4.5cm}
}
\end{center}
\caption{{\small
Comparing PF-D (red-*) and PF-EIS (black-$\triangle$) for a realization of Example \ref{biasctby2alpha01m3} with $M=3,K=1$.
Fig \ref{process3_error_totbad1}: (top) Norm of the error between the true between the true temperature values, $C_t$ and the tracked ones (PF estimate of $\E[C_t|Y_{1:t}]$) for PF-EIS and for PF-D; (bottom) Number of particles of PF-EIS (black -$\triangle$) with $\Delta^*(X_{t-1}^i,v_{t,s}^i,Y_t) < \max_p \Delta_{p+1} =2$ \ ($\pss(v_{t,r})$ may be bimodal for these particles), and number of particles of PF-D (red -*) with $\Delta^*(X_{t-1}^i,Y_t)(v_{t,s}) < \max_p \Delta_p =10$ \ ($p^*$ may be bimodal as a function of $v_{t,s}$ for these particles). Note for PF-D we  computed a $\Delta^*$, s.t. $\Delta < \Delta^*$ ensures unimodality of $p^*(v_{t,s},v_{t-1,r}^i)$.
Fig. \ref{process3hist6}, \ref{process3hist7}, \ref{process3hist8}: histograms of $C_{t,1}$ particles  of PF-D (top) and of PF-EIS (bottom)  at t=6,7,8.
%
% $p^*$ bimodal as a function of $v_{t,s}$ only ($v_{t,r}$ kept fixed at $v_{t-1,r}^i$) and number of particles of PF-EIS (black -$\triangle$) with $\pss$ bimodal as a function of $v_{t,r}$. As can be seen $\pss$ is multimodal very few times: for only 5 particles at t=4 and 2 particles at t=11, while $p^*$ is bimodal as a function of $v_{t,s}$ much more often. Note the above will give an exact number of cases where $p^*$ is multimodal only if $[B_s, B_r] = I$. %In the current example this is only a heuristic.
%Analyzing PF-D and PF-EIS for M=3. (a),(b),(c): Histogram of particles at t=6,7,8. With PF-Doucet (K=0) slowly all cluster around the wrong mode. (d): PF-Doucet: \% of particles of $C_{t-1}$ with bimodal $p^*$. Most of these $C_{t-1}$ particles are near the WRONG mode of $p^*$. (f) E and L for an example particle $C_{t-1}^i$ at t=7,i=1. The correct mode is the larger magnitude $Y_t$ while  dominant mode of $p^*$ is the wrong one. }}
}}
\label{pfeisprocess3}
\end{figure*}


\begin{figure*}
\begin{center}
%\subfigure[N=50, RMSE]
%{
%\psfig{file = \locc/unimod/newsims_sqr_A07/rmseN50_iters50.eps, width=4cm,height=4cm}
%}
\subfigure[N=100, RMSE]
{
\psfig{file = \locc/unimod/newsims_sqr_A07/rmseN50_iters50.eps, width=4cm,height=4cm}
}
\subfigure[N=100, Out of track \%]
{
\psfig{file = \locc/unimod/newsims_sqr_A07/numlarge20N50_iters50.eps, width=4cm,height=4cm}
}
\subfigure[N=100, Median]
{
\psfig{file = \locc/unimod/newsims_sqr_A07/medianN50_iters50.eps, width=4cm,height=4cm}
}
\end{center}
\caption{{\small Example \ref{Ctsqr}:  The first sensor node observes squared temperature value (and zero sensor failure probability). One sensor per node. Observation model is $Y_{t,1} = C_{t,1}^2 + w_t, \ w_t \sim \n(0,3)$, $Y_{t,2:3} = C_{t,2:3} + w_{t}, \ w_t \sim \n(0,1)$.
Temperature change follows an AR model with $A = 0.7 I_3$. Other parameters are:
$\Sigma_s = 10 $, $\Sigma_r = 5 I_2 $, $B_s = [0.95 \ 0.21 \ 0.21]'$, $C_0 = [5 \ 5 \ 5]'$
$\sigma_{obs}^2 = [3 \ 1 \ 1]'$, $\alpha_1 = 0$. % $p_f^1 = p_f^2 = \N(0.2C_t, \sigma_{obs}^2 I_3)$
50 realizations were used.
``Out of track" \% is the percentage of realizations for which the squared error norm exceeds 20.
%Comparing RMSE (root mean squared error), median, and percentage of times ``out of track"  when using PF-EIS (black-$\triangle$) with that of PF-D (red-*) and PF-Orig (magenta-o).
%State dimension $M=3$ and effective basis dim $K=1$. PF-EIS ($K=1$),  outperforms both PF-D ($K=0$) and PF-Orig ($K=M$).
}}
% generate an example with 0.01 failure probability (to avoid comparison with RB-PF,
% generate an example with 100 particles
\label{Ctsqrfigs}
\end{figure*}




\begin{figure*}
\begin{center}
\subfigure[Example \ref{twoYmodes}(a), N=50, RMSE]
{
\psfig{file = \locc/unimod/newsims_twoYmodes/rmse_gditerN50_iters50.eps, width=4cm,height=4cm}
}
\subfigure[Example \ref{twoYmodes}(a), N=50, Median]
{
\psfig{file = \locc/unimod/newsims_twoYmodes/median_gditerN50_iters50.eps, width=4cm,height=4cm}
}
\subfigure[Example \ref{twoYmodes}(b), N=50, RMSE]
{
\psfig{file = \locc/unimod/newsims_outlier_all_gditer5/rmseN50_100iters.eps, width=4cm,height=4cm}
}
%\subfigure[Example \ref{twoYmodes}(b), N=50, Median]
%{
%\psfig{file = \locc/unimod/newsims_outlier_all_gditer5/medianN50_100iters.eps, width=4cm,height=4cm}
%}
\subfigure[Examp\ref{twoYmodes}(b), N=50, Out of track \%]
{
\psfig{file = \locc/unimod/newsims_outlier_all_gditer5/numlarge12N50_100iters.eps, width=4cm,height=4cm}
}
\end{center}
\caption{{\small Comparing PF-EIS (black-$\triangle$) with PF-D (red-*) and PF-Orig (magenta-o) for Example \ref{twoYmodes}. Non-zero failure probability and observation depends on current temperature when sensor fails.
Temperature change follows a random walk model. Model parameters are:
$\Sigma_s = 10 $, $\Sigma_r = 5 I_2 $, $B_s = [0.95 \ 0.21 \ 0.21]$, $C_0 = [0 \ 0 \ 0]'$.
$\sigma_{obs}^2 = [1 \ 1 \ 1]'$.
For first two figures, one sensor per node was used and $p_f^1 =  \n(0.2 C_t,  I_3)$,  $\alpha_1 =  [0.4 \ 0.1 \ 0.1]$.
For last two figures, two sensors per node were used and $p_f^1 = p_f^2 = \n(0.2 C_t, 100 I_3)$,  $\alpha_1 = \alpha_2 = [0.4 \ 0.01 \ 0.01]$.
``Out of track" \% is the percentage of realizations for which the squared error norm exceeds 12.
}}
% (b): replace median by out of track %
\label{twoYmodesfigs}
\end{figure*}
%RMSE (root mean squared error), median, and percentage of times ``out of track"  when using

\begin{figure*}
\begin{center}
\subfigure[N=100, RMSE]
{
\psfig{file = \locc/unimod/newsims_outlier_correl_gditer5/rmse_N100_totiter50.eps, width=4cm,height=4cm}
}
\subfigure[N=100, Median]
{
\psfig{file = \locc/unimod/newsims_outlier_correl_gditer5/median_N100_totiter50.eps, width=4cm,height=4cm}
}
\subfigure[N=100, Out of track \%]
{
\psfig{file = \locc/unimod/newsims_outlier_correl_gditer5/numlarge24_N100_totiter50.eps, width=4cm,height=4cm}
}
\end{center}
\caption{{\small Comparing  PF-EIS (black-$\triangle$) with PF-D (red-*) and PF-Orig (magenta-o) for Example \ref{twoYmodes} (c). Strongly correlated states, observation depends on current temperature when sensor fails. Temperature change follows a random walk model. Parameters are:
$\Sigma_s = 10 $, $\Sigma_r = 2 I_2 $, $B_s = [0.47 \ 0.62 \ 0.62]$, $C_0 = [0 \ 0 \ 0]'$
$\sigma_{obs}^2 = [1 \ 1 \ 1]'$, $\alpha_1 = \alpha_2 = [0.2 \ 0.2 \ 0.2]$,  $p_f^1 = p_f^2 = \n(0.2 C_t, 100 I_3)$.
``Out of track" \% is the percentage of realizations for which the squared error norm exceeds 24.
}}
\label{twoYmodes}
\end{figure*}
%RMSE (root mean squared error), median, and percentage of times ``out of track"  when using


\begin{figure*}
\begin{center}
\subfigure[N=50, RMSE (Robust)]
{
\psfig{file = \locc/unimod/newsims_outlier_correl_impsamp/robust_rmse_N50_iters50.eps, width=4cm,height=4cm}
}
%\subfigure[N=50, Median]
%{
%\psfig{file = \locc/unimod/newsims_outlier_correl_impsamp/robust_median_N50_iters50.eps, width=4cm,height=4cm}
%}
\subfigure[Out of track \%  (Robust)]
{
\psfig{file = \locc/unimod/newsims_outlier_correl_impsamp/robust_numlarge24_N50_iters50.eps, width=4cm,height=4cm}
}
\subfigure[N=50, RMSE (Imp Samp)]
{
\psfig{file = \locc/unimod/newsims_outlier_correl_impsamp/impsamp_rmse_N50_iters50.eps, width=4cm,height=4cm}
}
\subfigure[Out of track \% (Imp Samp)]
{
\psfig{file = \locc/unimod/newsims_outlier_correl_impsamp/impsamp_numlarge24_N50_iters50.eps, width=4cm,height=4cm}
}
\end{center}
\caption{{\small Robustness to model error for Example \ref{twoYmodes} (d). Observation depends on current temperature when sensor fails. Temperature change follows a random walk model. Two sensors per node were used.
Model error is simulated by using $\alpha_1(1) = 0.9$ while simulating the observations' sequence.
System parameters are:
$\Sigma_s = 10 $, $\Sigma_r = 2 I_2 $, $B_s = [0.82 \ 0.41 \ 0.41]$, $C_0 = [0 \ 0 \ 0]'$
$\sigma_{obs}^2 = [1 \ 1 \ 1]'$, $\alpha_1 = \alpha_2 = [0.2 \ 0.1 \ 0.1]$,  $p_f^1 = p_f^2 = \n(0.2 C_t, 100 I_3)$.
``Out of track" \% is the percentage of realizations for which the squared error norm exceeds 24.
In the last two figures, we show errors assuming that instead of regular Monte Carlo, we have importance sampled $Y_{1:t}$ from a density for which the error norm is higher (while computing RMSE we weight each realization by its importance weight).
}}
\label{twoYmodesfigs3}
\end{figure*}


\begin{figure*}
\begin{center}
\subfigure[N=40, RMSE]
{\label{pfeisnew2N40}
\psfig{file = \locc/unimod/PFEIS_new2/mrmseN40.eps, width=4cm,height=4cm}
}
\subfigure[N=100, RMSE]
{\label{pfeisnew2N100}
\psfig{file = \locc/unimod/PFEIS_new2/mrmseN100.eps, width=4cm,height=4cm}
}
\subfigure[N=100, Out of track \%]
{\label{pfeisnew2N100}
\psfig{file = \locc/unimod/PFEIS_new2/numlarge48_N100.eps, width=4cm,height=4cm}
}
\subfigure[N=100, median error]
{\label{pfeisnew2N100}
\psfig{file = \locc/unimod/PFEIS_new2/median_N100.eps, width=4cm,height=4cm}
}
\end{center}
\caption{{\small Example \ref{pfeisnew2}: observation independent of current temperature when sensor fails, temperature change follows a random walk model.
$\Sigma_s = 10 $, $\Sigma_r = 5 I_2 $, $B_s = [0.99, 0.1, 0.1] $, $C_0 = [0 \ 0 \ 0]'$
$\sigma_{obs}^2 = [10 \ 1 \ 1]'$, $\alpha_1 = [0.9 \ 0.1 \ 0.1]$, $\alpha_2 = [0.4 \ 0.01 \ 0.01]$.
 $p_f^1 = p_f^2 = \n(0, 100 I_3)$.
 ``Out of track" \% is the percentage of realizations for which the squared error norm exceeds 48.
%Comparing RMSE (root mean squared error), median, and percentage of times ``out of track"  when using PF-EIS (black-$\triangle$) with that of PF-D (red-*) and PF-Orig (magenta-o).
}}
\label{pfeisnew2figs}
\end{figure*} 

==> figsnew2.tex <==
 \linespread{1}

\begin{figure*}
%\begin{center}
%\subfigure[N=40, RMSE]
%{\label{pfeisnew2N40}
%\psfig{file = \locc/unimod/PFEIS_new2/mrmseN40.eps, width=4cm,height=4cm}
%}
\subfigure[Temperature Independent Failure (TIF)] %N=100, $\alpha_1 = [0.9 \ 0.1 \ 0.1]$, $\alpha^{(2)} = [0.4 \ 0.01 \ 0.01]$, $p_f^1 = p_f^2 = \n(0, 100 I_3)$. $N=100$.
{\label{pfeisnew2N100}
\begin{tabular}{c}
\psfig{file = \locc/unimod/PFEIS_new2/correctmrmseN100_gspf.eps, width=5.5cm,height=4cm} \\ %_2types
% RMSE \\
\psfig{file = \locc/unimod/PFEIS_new2/numlarge48_N100.eps, width=5.5cm,height=4cm}
% \\ Out-of-track \%
\end{tabular}
}
\subfigure[One Squared Sensor] %N=50,
{\label{Ctsqr}
\begin{tabular}{c}
\psfig{file = \locc/unimod/newsims_sqr_A07/rmseN50_iters50_gspf.eps, width=5.5cm,height=4cm} \\
\psfig{file = \locc/unimod/newsims_sqr_A07/numlarge20N50_iters50.eps, width=5.5cm,height=4cm}
\end{tabular}
}
\subfigure[Temperature Dependent Failure (TDF)]
{\label{outlier_all}
\begin{tabular}{c}
\psfig{file = \locc/unimod/newsims_outlier_all_gditer5/rmseN50_100iters_gspf_2type.eps, width=5.5cm,height=4cm} \\
\psfig{file = \locc/unimod/newsims_outlier_all_gditer5/numlarge12N50_100iters.eps, width=5.5cm,height=4cm}
\end{tabular}
}
%
%\subfigure[$p_f=\n(C_{t,p},100)$, RMSE] %N=50
%{\label{outlier_noise}
%\psfig{file = \locc/unimod/newsims_outlier_noise/rmse_N50_iters100.eps, width=5.5cm,height=4cm}
%%\psfig{file = \locc/unimod/newsims_outlier_noise/numlarge12_N50_iters100.eps, width=4cm,height=4cm}
%}
\subfigure[TDF, Outlier Noise] %N=50
{\label{outlier_noise2}
\psfig{file = \locc/unimod/newsims_outlier_noise2/rmse_N50_iters90_gspf.eps, width=5.5cm,height=4cm}
%\psfig{file = \locc/unimod/newsims_outlier_noise2/numlarge9_N50_iters90.eps, width=5.5cm,height=4cm}
}
%
\subfigure[TDF, always bimodal] %N=50
{\label{twoYmodes}
\psfig{file = \locc/unimod/newsims_twoYmodes/rmse_gditerN50_iters50_gspf.eps, width=5.54cm,height=4cm}
%\psfig{file = \locc/unimod/newsims_outlier_all_gditer5/numlarge12N50_100iters.eps, width=4cm,height=4cm}
}
\subfigure[TDF, Model Error Robustness] %N=50
{\label{impsamprobust}
\psfig{file = \locc/unimod/newsims_outlier_correl_impsamp/robust_rmse_N50_iters50_gspf.eps, width=5.5cm,height=4cm}
%\psfig{file = \locc/unimod/newsims_twoYmodes/numlarge12_gditerN50_iters50.eps, width=4cm,height=4cm}
}
%\subfigure[$p_f=\n(0.2C_{t,p},100)$]
%{\label{outlier_new}
%%\begin{tabular}{c}
%\psfig{file = \locc/unimod/newsims_outlier_correl_new/rmse_epls02_N50_iters50.eps, width=5.25cm,height=4cm}
%\psfig{file = \locc/unimod/newsims_outlier_correl_new/numlarge24_epls02_N50_iters50.eps, width=5.25cm,height=4cm}
%%\end{tabular}
%}
\subfigure[Table of parameters]
{\small
%\begin{table*}
\centerline{
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|}
\hline
Fig. & $h(C_t)$ & $p_f(Y_{t,p}^{(j)} | C_{t,p})$ & $\alpha^{(1)}, \alpha^{(2)}$ & $\sigma_{obs}^2$ & $\Delta_\nu$ & $B$ & $C_0$ & $a$ & N \\
\hline
\ref{pfeisnew2N100} & $h(C_t)=C_t$ & $\n(0,100)$ & $\alpha^{(1)} = [.9, .1, .1]$, & [10, 1, 1] & $diag(10,5,5)$, & $[.99, .1, .1]';$ &  $[0, 0, 0]'$ & $1$ & 100 \\
& & & $\alpha^{(2)} = [.4, .01, .01];$ &  &  & $[-.10, 0.99, -.01]';$  & & & \\
 &  & & & & &  $[-.10, 0,.99]'$ & & & \\
\hline
%
\ref{Ctsqr} & $h_1(C_t)= C_{t,1}^2$   &  & $\alpha^{(1)} = [0, 0, 0]$ & $[3, 1, 1]$ & $diag(10,5,5)$, & $[.95, .21, .21]';$ & $[5, 5, 5]'$ & $.7$ & 50 \\
& $h_p(C_t)= C_{t,p}^2$, $p>1$ & & & &   &  $[-.21,.98,-.05]';$  & & &  \\
 &  & & & & &  $[-.22, 0, .98]'$ & & & \\
\hline
%
\ref{outlier_all} &  $h(C_t)=C_t$   & $\n(.2C_{t,p},100)$ & $\alpha^{(1)} =  [.4, .01, .01]$ & $[1,1,1]$ & $diag(10,5,5)$ & $[.95, .21, .21]';$ & $[0, 0, 0]'$ & $1$ & 50 \\
 &  & & $\alpha^{(2)} =  [.4, .01, .01]$ & &   &  $[-.21,.98,-.05]';$ & & & \\
 &  & & & & &  $[-.22, 0, .98]'$ & & & \\
\hline
%\ref{outlier_noise} &  $\n(C_{t,p}, \sigma_{obs,p}^2)$   & $\n(C_{t,p},100)$ & $\alpha_j = [.4, .2, .2]$ & $[1,1,1]$ & $\Sigma_s = 10 $ & $[.82, .41, .41]'$ & $[0, 0, 0]'$ & $ I_3$ & 50 \\
% &  & & & & $\Sigma_r = 5 I_2$  & & & & \\
% \hline
 \ref{outlier_noise2} &  $h(C_t)=C_t$   & $\n(C_{t,p},1600)$ & $\alpha^{(1)} = [.4, .1, .1]$ & $[1,1,1]$ & $diag(10,5,5)$ & $[.95, .21, .21]';$ & $[0, 0, 0]'$ & $1$ & 50 \\
 &  & & $\alpha^{(2)} = [.4, .01, .01]$ & &   &  $[-.21,.98,-.05]';$ & & & \\
  &  & & & & & $[-.22, 0, .98]'$ &  & & \\
 \hline
 \ref{twoYmodes} &   $h(C_t)=C_t$   & $\n(.2C_{t,p},1)$ & $\alpha^{(1)} = [.4, .1, .1]$ & $[1,1,1]$ & $diag(10,5,5)$ & $[.95, .21, .21]';$ & $[0, 0, 0]'$ & $1$ & 50 \\
 &  & & & &    & $[-.21,.98,-.05]';$ & &  & \\
  &  & & & & & $[-.22, 0, .98]'$ &  & & \\
\hline
 \ref{impsamprobust} &  $h(C_t)=C_t$   & $\n(.2C_{t,p},100)$ & $\alpha^{(1)} = [.2, .1, .1]$ & $[1,1,1]$ & $diag(10,2,2)$ & $[.82, .41, .41]';$ & $[0, 0, 0]'$ & $1$ & 50 \\
 &  & & $\alpha^{(2)} = [.2, .1, .1]$  &  &   & $[-.37, .91, -0.18]';$ & & & \\
   &  & & $\alpha^{(1)}_{sim}=[.9,.1,.1]$ & & & $[ -.45,  0, 0.89]'$ &  & &  \\
\hline
%\ref{outlier_new} &  $\n(C_{t,p}, \sigma_{obs,p}^2)$   & $\n(.2C_{t,p},100)$ & $\alpha_j =  [.4, .2, .2]$ & $[1,1,1]$ & $\Sigma_s = 10 $ & $[.95, .21, .21]'$ & $[0, 0, 0]'$ & $ I_3$ \\
% &  & & & & $\Sigma_r = 5 I_2$  & & &  \\
%\hline
\end{tabular}
\label{fig1parameters}
}
%\end{table*}
}
%\subfigure[Ex  \ref{pfeisnew2}, Out-of-track \%] %N=100
%{\label{pfeisnew2N100}
%\psfig{file = \locc/unimod/PFEIS_new2/numlarge48_N10.eps, width=6cm,height=6cm}
%}
%\subfigure[Ex \ref{Ctsqr}, Out-of-track \%] %N=50
%{
%\psfig{file = \locc/unimod/newsims_sqr_A07/numlarge20N50_iters50.eps, width=6cm,height=6cm}
%}
%\subfigure[N=100, median error]
%{\label{pfeisnew2N100}
%\psfig{file = \locc/unimod/PFEIS_new2/median_N100.eps, width=4cm,height=4cm}
%}
%\end{center}
\caption{{\small
Comparing RMSE and out-of-track \% of PF-EIS (black-$\triangle$) with that of  PF-Doucet (red-*), PF-Orig (magenta-o) and GSPF-I (magenta -+). $N=100$ particles were used in  Fig. \ref{pfeisnew2N100} since  $N=50$ gave large RMSE (but same trend) for all algorithms. All other figures used $N=50$. We also simulated $N=100$ but the trends were similar and so we only show $N=50$.
RMSE at time $t$ is the square root of the mean of the squared error between the true $C_t$ and the tracked one ($N$-particle PF estimate of $\E[C_t|Y_{1:t}]$).
Out-of-track \% is the percentage of realizations for which the squared error norm exceeds an in-track threshold (2-4 times of total observation noise variance). In-track threshold for Fig. \ref{pfeisnew2N100} was 48, for Fig. \ref{Ctsqr} was 20 and for Fig. \ref{outlier_all} was 12.
All figures used between 40 and 100 Monte Carlo simulations. We  used 90 simulations for Fig. \ref{outlier_all}, \ref{outlier_noise2}, 50 for Fig. \ref{Ctsqr}, \ref{twoYmodes}, \ref{impsamprobust} and 40  for Fig. \ref{pfeisnew2N100} (taken from old set of simulations).
Note $C_0$ refers to the starting value of $C_t$.
%Fig. \ref{outlier_all} used 5 gradient descent iterations.
%
%
%{\bf Fig. \ref{pfeisnew2N100}. } Observation independent of current temperature when sensor fails, temperature change follows a random walk model. $N=100$. ``Out of track" \% is the percentage of realizations for which the squared error norm exceeds 48. %$\Sigma_s = 10 $, $\Sigma_r = 5 I_2 $, $B_s = [0.99, 0.1, 0.1] $, $C_0 = [0 \ 0 \ 0]'$, $\sigma_{obs}^2 = [10 \ 1 \ 1]'$, $\alpha^{(1)} = [0.9 \ 0.1 \ 0.1]$, $\alpha^{(2)} = [0.4 \ 0.01 \ 0.01]$, $p_f^1 = p_f^2 = \n(0, 100 I_3)$.
%{\bf Fig. \ref{Ctsqr}. }   The first sensor node observes squared temperature value (and zero sensor failure probability). One sensor per node. Observation model is $Y_{t,1} = C_{t,1}^2 + w_t, \ w_t \sim \n(0,3)$, $Y_{t,2:3} = C_{t,2:3} + w_{t}, \ w_t \sim \n(0,1)$. Temperature change follows an AR model with $A = 0.7 I_3$. %Other parameters are: $\Sigma_s = 10 $, $\Sigma_r = 5 I_2 $, $B_s = [0.95 \ 0.21 \ 0.21]'$, $C_0 = [5 \ 5 \ 5]'$, $\sigma_{obs}^2 = [3 \ 1 \ 1]'$, $\alpha^{(1)} = 0$. $N=50$. % $p_f^1 = p_f^2 = \N(0.2C_t, \sigma_{obs}^2 I_3)$
%% 50 realizations were used.
%{\bf Fig. \ref{outlier_all}, \ref{outlier_new}. } Observation depends on current temperature when sensor fails. Temperature change follows a random walk model. ``Out of track" \% is the percentage of realizations for which the squared error norm exceeds 24.
%{\bf Fig. \ref{impsamprobust}. } Model error is simulated by using $\alpha^{(1)}(1) = 0.9$ while simulating the observations' sequence.
%$\Sigma_s = 10 $, $\Sigma_r = 5 I_2 $, $B_s = [0.95 \ 0.21 \ 0.21]$, $C_0 = [0 \ 0 \ 0]'$, $\sigma_{obs}^2 = [1 \ 1 \ 1]'$, $\alpha^{(1)} =  [0.4 \ 0.01 \ 0.01]$, $N=50$. ``Out of track" \% is the percentage of realizations for which the squared error norm exceeds 12. %, one sensor per node
%
%{\bf Fig. \ref{outlier_new}. } Example \ref{}. Non-zero failure probability and observation depends on current temperature when sensor fails. Temperature change follows a random walk model. $\Sigma_s = 10 $, $\Sigma_r = 5 I_2 $, $B_s = [0.95 \ 0.21 \ 0.21]$, $C_0 = [0 \ 0 \ 0]'$, $\sigma_{obs}^2 = [1 \ 1 \ 1]'$, $\alpha^{(1)} = \alpha^{(2)} = [0.4 \ 0.2 \ 0.2]$, $N=50$. ``Out of track" \% is the percentage of realizations for which the squared error norm exceeds 24.
%``Out of track" \% is the percentage of realizations for which the squared error norm exceeds 20.
%Comparing RMSE (root mean squared error), median, and percentage of times ``out of track"  when using PF-EIS (black-$\triangle$) with that of PF-D (red-*) and PF-Orig (magenta-o).
}}
\label{pfeisfigs}
\end{figure*}

\begin{figure*}
%\begin{center}
%\subfigure[Example  \ref{pfmt12}, N=50]
%{\label{pfmt12fig_old}
%\begin{tabular}{c}
%\psfig{file = \locc/unimod/PFMT2/correctpfmt_mrmseN50.eps, width=5cm,height=4cm} \\
%%\psfig{file = \locc/unimod/PFMT2/numlarge100_N50.eps, width=5cm,height=4cm}
%\psfig{file = \locc/unimod/PFMT2/numlarge150_N50.eps, width=5cm,height=4cm}
%\end{tabular}
%}
%\subfigure[Example  \ref{pfmt12}, N=50]
%{\label{pfmt12fig}
%\begin{tabular}{c}
%\psfig{file = \locc/unimod/newsims_PFMT2/rmse.eps, width=5cm,height=4cm} \\
%\psfig{file = \locc/unimod/newsims_PFMT2/numlarge150.eps, width=5cm,height=4cm}
%\end{tabular}
%}
%\subfigure[$p_f = \n(0,100)$, N=50]
%{\label{pfmt3fig}
%\begin{tabular}{c}
%\psfig{file = \locc/unimod/newsims_PFMT3/rmse_N50_iters50.eps, width=5cm,height=4cm} \\
%\psfig{file = \locc/unimod/newsims_PFMT3/numlarge30_N50_iters50.eps, width=5cm,height=4cm}
%\end{tabular}
%}
\subfigure[Temperature Independent Failure (TIF)]%$p_f = \n(0,100)$, N=100]
{\label{pfmt3_N100fig}
\begin{tabular}{c}
\psfig{file = \locc/unimod/newsims_PFMT3/rmse_N100_iters50.eps,  width=5.5cm,height=4cm} \\
\psfig{file = \locc/unimod/newsims_PFMT3/numlarge30_N100_iters50.eps,  width=5.5cm,height=4cm}
\end{tabular}
}
\subfigure[One Squared Sensor]%, N=50]
{\label{pfmtsqrfig}
\begin{tabular}{c}
\psfig{file = \locc/unimod/newsims_PFMT_sqr_fail/rmse_N50_iters50.eps,  width=5.5cm,height=4cm} \\
\psfig{file = \locc/unimod/newsims_PFMT_sqr_fail/numlarge24_N50_iters50.eps,  width=5.5cm,height=4cm}
\end{tabular}
}
\subfigure[Temperature Dependent Failure (TDF)] %$p_f = \n(0.2C_{t,p},400)$, N=50]
{\label{pfmtoutlierfig}
\begin{tabular}{c}
\psfig{file = \locc/unimod/newsims_PFMT_outlier/rmse_N50_iters50.eps,  width=5.5cm,height=4cm} \\
\psfig{file = \locc/unimod/newsims_PFMT_outlier/numlarge30_N50_iters50.eps,  width=5.5cm,height=4cm}
\end{tabular}
}
\subfigure[Table of parameters]
{\small
%\begin{table*}
\centerline{
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|}
\hline
Fig. & $h(C_t)$ & $p_f(Y_{t,p}^{(j)} | C_{t,p})$ & $\alpha^{(1)}, \alpha^{(2)}$ & $\sigma_{obs}^2$ & $\Delta_\nu$ & $B_{1,:}$ & $C_0$ & $a$ & N \\
\hline
%\ref{pfmt12fig} &  $\n(C_{t,p}, \sigma_{obs,p}^2)$   & $Unif(-10,10)$ & $\alpha^{(1)} = [0.4, 0_9]$ & $5_{10}$ & $\Sigma_s = 10 $ & $[0.56, 0.28_9]'$ & $0_{10}$ & $ I_{10}$ \\
% &  &  & $\alpha^{(2)} = [0.1, 0_9]$ & & $\Sigma_r = 1 I_9$  & & &  \\
% \hline
\ref{pfmt3_N100fig} &  $h(C_t)=C_t$   & $\n(0,100)$ & $\alpha^{(1)} = [0.9, 0.01_9]$ & $1_{10}$ & $diag([10,1_9])$ & $[0.83, 0.18_9 ]'$ & $0_{10}$ & $1$ & 100 \\
 &  & & $\alpha^{(2)} = [0.4, 0.01_9]$ & &   & & & &  \\
% \ref{pfmt3fig} N=50
\hline
\ref{pfmtsqrfig} & $h_1(C_{t}) = C_{t,1}^2$   & $\n(0,100)$  & $\alpha^{(1)} = 0.001_{10}$ & $[3, 1_9]$ & $diag([10,1_9])$ & $[0.83, 0.18_9]'$ & $5_{10}$ & $0.7$ & 50 \\
& $h_p(C_{t})= C_{t,p}$, $p>1$ & & & &     & & & & \\
\hline
 \ref{pfmtoutlierfig} &  $h(C_t)=C_t$   & $\n(0.2C_{t,p},400)$ & $\alpha^{(1)} = [0.4, 0.01_9]$ & $1_{10}$ & $diag([10,2_9])$ & $[0.83, 0.18_9 ]'$ & $0_{10}$ & $1$ & 50 \\
 &  & & $\alpha^{(2)} = [0.4, 0.01_9]$ & &     & & & & \\
\hline
\end{tabular}
}
%\end{table*}
\label{fig3parameters}
}
%\end{center}
\caption{{\small PF-MT:
Comparing RMSE  and out-of-track \% of  PF-MT (blue-$\square$) with that of  PF-Doucet (red-*), PF-EIS (black-$\triangle$), PF-Orig (magenta-o) and PF-Orig-K dim (green-x). State dimension $M=10$. $K=1$ dim effective basis used for both PF-EIS and PF-MT.
$N=100$ particles were used in  Fig. \ref{pfmt3_N100fig} since  $N=50$ gave large RMSE (though same trend) for all algorithms.  All other figures used $N=50$. ``Out of track" \% is the percentage of realizations for which the squared error norm exceeds an in-track threshold (2-3 times of total observation noise variance). In-track threshold for Fig. \ref{pfmt3_N100fig} was 30, for Fig. \ref{pfmtsqrfig} was 24 and for Fig. \ref{pfmtoutlierfig} was 30. All figures used 50 Monte Carlo simulations.
{\em The notation $b_k$ denotes a row vector of $bs$ of length $k$, e.g. $1_9$ denotes a row vector of 1s of length 9.} {\em The ``;" notation follows MATLAB notation.}
%
% $K=1$ for all except the last figure where $K=3$. Since $N$ is small compared to the dimension $M=10$, PF-MT has the best performance. If $N$ is increased, PF-EIS or PF-D will have better performance.
%For large dimensions (and small $N$ compared to the dimension),
%Use only pfmtbias and pfmtold. Show N=20,50 for pfmtbias N=20,40 for pfmtold
}}
\label{pfmtfigs}
\end{figure*}

%\begin{figure*}[b!]
%%\begin{center}
%\subfigure[Top: Error. Bottom: \# of particles of PF-EIS (PF-D) for which $\pss(C_{t,1})$ ($p^*(C_{t,1})$) may be multimodal]
%%with $\Delta^*(X_{t-1}^i,v_{t,s}^i,Y_t) < \max_p \Delta_{p+1} =2$, no. of particles of PF-D (red -*) with $\Delta^*(X_{t-1}^i,Y_t)(v_{t,s}) < \max_p \Delta_p =10$]
%%$p^*$  bimodal as a function of $v_{t,s}$ only, $\pss(v_{t,r})$ bimodal]%\% of particles with $\Delta^* < \max_{p} \Delta_{p+K}$ (black -$\triangle$)
%{\label{process3_error_totbad1}
%\psfig{file = \locc/unimod/BiasCtby2_alpha01_M3/iter10_Error_totbad1.eps, width=4.25cm,height=4.5cm}
%}
%\hspace{0.01in}
%\subfigure[Histgrm of $C_{t,1}$ particles, t=6.]% Top: PF-Doucet, Bottom: PF-EIS. $Y_{t,1}^{1,2}=-13.0,-25.8$]
%{\label{process3hist6}
%\psfig{file = \locc/unimod/BiasCtby2_alpha01_M3/iter10histt6.eps, width=4cm,height=4.5cm}
%}
%\hspace{0.01in}
%\subfigure[Histgrm of $C_{t,1}$ particles, t=7.]% Top: PF-Doucet, Bottom: PF-EIS. $Y_{t,1}^{1,2}=-14.2,-28.5$]
%{\label{process3hist7}
%\psfig{file = \locc/unimod/BiasCtby2_alpha01_M3/iter10histt7.eps, width=4cm,height=4.5cm}
%}
%\hspace{0.01in}
%\subfigure[Histgrm of $C_{t,1}$ particles, t=8.]% Top: PF-Doucet, Bottom: PF-EIS. $Y_{t,1}^{1,2}=-30.9,-32.3$]
%{\label{process3hist8}
%\psfig{file = \locc/unimod/BiasCtby2_alpha01_M3/iter10histt8.eps, width=4cm,height=4.5cm}
%}
%%\end{center}
%\caption{{\small %\ref{biasctby2alpha01m3}
%Comparing PF-Doucet with PF-EIS for a realization of Example \ref{example1}  with $M=3,K=1$ but with sensor failure model error.
%System parameters were $\alpha^{(1)} = [0.1, 0.1, 0.1]$, $\alpha^{(2)} = [0.1, 0.1, 0.1]$, $\sigma_{obs}^2 = [1, 1, 1]$, $p_f^1=p_f^2 = Unif(-100,100)$, $a=1$, $\Sigma_\nu = diag(10,2,2)$, $B_s =[0.82 \   0.41   \ 0.41]$, $B_r$ = its orthogonal complement. Model error simulating by using used $\alpha_1^{(1)} = 0.99$ and $p_f(Y_{t,1}^{(1)}|C_{t,1}) = \n(C_{t}/2,0)$  for $t \le 7$, during simulation.
%In case of PF-Doucet, as OL modes move further away, more and more particles cluster around one mode (which happens to be the wrong one). Until $t=6$ there are still some particles near both modes. But at $t=7$, all particles are clustered at the wrong mode. This results in loss of track. PF-EIS samples $X_{t,s}$ from the STP and hence has particles around both modes.
%}}
%\label{pfeisprocess3}
%\end{figure*}


%\begin{figure*}
%\subfigure[(top) Error, (bottom) no. of particles of PF-D with $\Delta^* < \Delta_1=10$]%, i.e. for which $p^*$ may be bimodal]
%{\label{process_error}
%%\psfig{file = \locc/unimod/BiasCtby2_M1/iter5Error.eps, width=2cm,height=2.5cm}
%\psfig{file = \locc/unimod/BiasCtby2_M1/iter5_Error_totbad1.eps, width=4.25cm,height=4.5cm}
%}
%\hspace{0.01in}
%\subfigure[$E,-\log p^*$ for a PF-D  particle at $t=7$ with $\Delta^*=6.2 < \Delta_1$]
%{\label{process_totbad1}
%%\psfig{file = \locc/unimod/BiasCtby2_M1/iter5_totbad1_EL_t7ii_K0.eps, width=4.5cm,height=4.5cm}
%\psfig{file = \locc/unimod/BiasCtby2_M1/iter5EL_t7_i1_K0.eps, width=4cm,height=4.5cm}
%}
%\hspace{0.01in}
%\subfigure[Histogram of $C_t$ particles, t=6. (top) PF-D, (bottom) PF-EIS]
%{\label{processhist6}
%\psfig{file = \locc/unimod/BiasCtby2_M1/iter5histt6.eps, width=4cm,height=4.5cm}
%}
%\subfigure[Histogram of $C_t$ particles, t=7. (top) PF-D, (bottom) PF-EIS. $Y_{t}^{1,2}=9.0, 17.4$]
%{\label{processhist7}
%\psfig{file = \locc/unimod/BiasCtby2_M1/iter5histt7.eps, width=4cm,height=4.5cm}
%}
%\hspace{0.01in}
%\subfigure[Histogram of $C_t$ particles, t=8. (top) PF-D, (bottom) PF-EIS. $Y_{t}^{1,2}=22.8, 22.8$]
%{\label{processhist8}
%\psfig{file = \locc/unimod/BiasCtby2_M1/iter5histt8.eps, width=4cm,height=4.5cm}
%}
%\caption{{\small Detailed comparison of PF-D (red-*) and PF-EIS (black-$\triangle$), which is same as PF-Orig for $M=1,K=1$.
%%Fig \ref{process_error} (top): Norm (here absolute value) of the error between the true between the true temperature values, $C_t$ and the tracked ones (PF estimate of $\E[C_t|Y_{1:t}]$) for PF-EIS and for PF-D; (bottom): Number of particles of PF-D at each $t$ for which $\Delta^* < \Delta_1=10$, i.e. for which $p^*$ may be bimodal.
%%Fig \ref{process_totbad1}:  $E,-\log p^*$ for a particle of PF-D at $t=7$, with $\Delta^*=6.2 < \Delta_1$.
%%Fig. \ref{processhist6}, \ref{processhist7}, \ref{processhist8}: histograms of $C_t$ particles at t=6,7,8  for PF-D (top) \& PF-EIS (bottom).
%%
% We used the following system parameters:
%$\alpha^{(1)} = 0.1$, $\alpha^{(2)} = 0.1$, $\sigma_{obs}^2 = 1$, $p_f^1 = p_f^2 = Unif(-100,100)$, $\Delta_1 = 10$, $A = 0.7$. To demonstrate a typical situation where PF-Doucet fails, we simulated with $\alpha^{(1)} = 0.99$  and $p_f^1 = \n(C_{t}/2,0)$ for $t \le 7$ (and $\alpha^{(1)} = 0.1$ and  $p_f^1 = Unif(-100,100)$ for $t > 7$) during simulation. This simulates a modeling error situation: the learnt sensor failure model for one sensor is wrong. It keeps outputting a value of $C_t/2$ for the first 7 time instants.
%% \footnote{Since this is a model error situation, one is not looking out for it and hence cannot use finite state HMMs or any other simpler algorithm to detect this}
%%
%Since we  began with $C_t=0$ at $t=1$, for the first few time instants,  most particles had small magnitude and so they were in the BoA of $Y_t^1$ (failure mode). Thus, in most cases, PF-Doucet sampled from a narrow Gaussian ($\Sigma_{IS}^i \approx  1/ (1/1 + 1/10) \approx 0.9$) about a $p^*$ mode that was near the failure mode. As a result, once again, only a few samples fell in the basin-of-attraction of the true mode at the next time instant. This thing repeated at every $t \le 7$. As $t$ increased, the OL modes drifted further apart, while the variance of the IS density remained the same. Thus by $t=7$ all particles were near the wrong mode. At $t=8$ when only the true mode appears, PF-D has lost track. In contrast, PF-EIS (same as PF-Orig in this case) samples from the STP which is broad ($\Delta_1 =10$) and hence has particles near both OL modes, and so it does not lose track.
%%
%%Fig. \ref{processhist7}, \ref{processhist8}: histograms of $C_t$ particles  of PF-D (top) and of PF-EIS (bottom) at t=7,8.
%% Histogram of particles at t=6,7,8. With PF-Doucet (K=0) slowly all cluster around the wrong mode.
%%(d): PF-Doucet: \% of particles of $C_{t-1}$ with bimodal $p^*$. Most of these $C_{t-1}$ particles are near the WRONG mode of $p^*$. (f) E and L for an example particle $C_{t-1}^i$ at t=7,i=1. The correct mode is the larger magnitude $Y_t$ while  dominant mode of $p^*$ is the wrong one. }}
%}}
%\label{pfeisprocess}
%\end{figure*}




% Put in Review Comments
%\begin{figure*}
%\begin{center}
%\subfigure[$K=2, M=4$, $N = 200$] %N=50
%{\label{chM4N200}
%\psfig{file = \locc/unimod/newsims_ChoiceBsBr/rmse_excluding_iter18_N200_K2M4.eps, width=5.5cm,height=4cm}
%}
%\subfigure[$K=1, M=3$, $N = 200$] %N=50
%{\label{chM3N200}
%\psfig{file =\locc/unimod/newsims_ChoiceBsBr/rmse_N200_K1M3.eps, width=5.5cm,height=4cm}
%}
%\subfigure[$K=1, M=3$, $N = 50$] %N=50
%{\label{chM3N50}
%\psfig{file = \locc/unimod/newsims_ChoiceBsBr/rmse_N50_K1M3.eps, width=5.5cm,height=4cm}
%}
%\end{center}
%\caption{{\small
%Fig. \ref{chM4N200}:
% We simulated data for a $K=2, M=4$ (2D effective basis, 2D residual space) example using $B_s = [ ]$, $B_r = [ ]$ $\Sigma_s = 7 I_2$, $\Sigma_r = 5 I_2$. For tracking (choice 1), we also tracked with the same $B_s, B_r$. For tracking (choice 2), we computed the orthogonal eigenvectors  of $\Sigma = B_s \Sigma_s B_s^T + B_r \Sigma_r B_r^T$ and used them as $[B_s, B_r]$.
%Fig. \ref{chM3N200}: $K=1, M=3$ example with $N=200$. $B_r = [ ]$ for simulation and for choice 1. For choice 2, $B_r = [ ]$.
%Fig. \ref{chM3N50}: Same example tracked with $N=50$.
%}}
%\label{ch}
%\end{figure*}


%\begin{figure*}
%\begin{center}
%\subfigure[$p_f=\n(C_{t,p},100)$, RMSE] %N=50
%{\label{outlier_noise}
%\psfig{file = \locc/unimod/newsims_outlier_noise/rmse_N50_iters100.eps, width=5.5cm,height=4cm}
%%\psfig{file = \locc/unimod/newsims_outlier_noise/numlarge12_N50_iters100.eps, width=4cm,height=4cm}
%}
%%\subfigure[$p_f=\n(0.2C_t,100I_3)$, RMSE] %N=50
%%{\label{outlier_all}
%%\psfig{file = \locc/unimod/newsims_outlier_all_gditer5/rmseN50_100iters.eps, width=4cm,height=4cm}
%%%\psfig{file = \locc/unimod/newsims_outlier_correl_gditer5/rmse_N100_totiter50.eps, width=4cm,height=4cm} %N=100, strong correlation
%%%\psfig{file = \locc/unimod/newsims_outlier_all_gditer5/numlarge12N50_100iters.eps, width=4cm,height=4cm}
%%%\psfig{file = \locc/unimod/newsims_outlier_correl_gditer5/numlarge24_N50_totiter100.eps, width=4cm,height=4cm} %N=100, strong correlation
%%}
%\subfigure[$p_f=\n(0.2C_{t,p},1)$, RMSE] %N=50
%{\label{twoYmodes}
%\psfig{file = \locc/unimod/newsims_twoYmodes/rmse_gditerN50_iters50.eps, width=5.54cm,height=4cm}
%%\psfig{file = \locc/unimod/newsims_outlier_all_gditer5/numlarge12N50_100iters.eps, width=4cm,height=4cm}
%}
%\subfigure[Model error robustness, RMSE] %N=50
%{\label{impsamprobust}
%\psfig{file = \locc/unimod/newsims_outlier_correl_impsamp/robust_rmse_N50_iters50.eps, width=5.5cm,height=4cm}
%%\psfig{file = \locc/unimod/newsims_twoYmodes/numlarge12_gditerN50_iters50.eps, width=4cm,height=4cm}
%}
%%
%%\subfigure[$p_f=\n(0.2C_t,100I_3)$, Out-of-track \%] %N=50
%%{\label{outlier_all2}
%%\psfig{file = \locc/unimod/newsims_outlier_all_gditer5/numlarge12N50_100iters.eps, width=4cm,height=4cm}
%%%\psfig{file = \locc/unimod/newsims_outlier_correl_gditer5/numlarge24_N50_totiter100.eps, width=4cm,height=4cm} %N=100, strong correlation
%%}
%%\subfigure[$p_f=\n(0.2C_t,I_3)$, Out-of-track \%] %Median error] %N=50
%%{\label{twoYmodes2}
%%\psfig{file = \locc/unimod/newsims_twoYmodes/numlarge12_gditerN50_iters50.eps, width=4cm,height=4cm}
%%}
%%\subfigure[Model error, Out-of-track \%]
%%{\label{impsamprobust2}
%%\psfig{file = \locc/unimod/newsims_outlier_correl_impsamp/robust_numlarge24_N50_iters50.eps, width=4cm,height=4cm}
%%}
%\subfigure[Table of parameters]
%{\small
%%\begin{table*}
%\centerline{
%\begin{tabular}{|l|l|l|l|l|l|l|l|l|}
%\hline
%Fig. & $p_{nf}(Y_{t,p}^{(j)} | C_{t,p})$ & $p_f(Y_{t,p}^{(j)} | C_{t,p})$ & $\alpha_1, \alpha^{(2)}$ & $\sigma_{obs}^2$ & $\Sigma_s, \Sigma_r$ & $B_s$ & $C_0$ & $A$ \\
%\hline
%\ref{outlier_noise} &  $\n(C_{t,p}, \sigma_{obs,p}^2)$   & $\n(C_{t,p},100)$ & $\alpha_j = [0.4, 0.2, 0.2]$ & $[1,1,1]$ & $\Sigma_s = 10 $ & $[0.82, 0.41, 0.41]'$ & $[0, 0, 0]'$ & $ I_3$ \\
% &  & & & & $\Sigma_r = 5 I_2$  & & &  \\
% \hline
% \ref{twoYmodes} &  $\n(C_{t,p}, \sigma_{obs,p}^2)$   & $\n(0.2C_{t,p},1)$ & $\alpha_1 = [0.4, 0.1, 0.1]$ & $[1,1,1]$ & $\Sigma_s = 10 $ & $[0.95, 0.21, 0.21]'$ & $[0, 0, 0]'$ & $ I_3$ \\
% &  & & & & $\Sigma_r = 5 I_2$  & & &  \\
%\hline
% \ref{impsamprobust} &  $\n(C_{t,p}, \sigma_{obs,p}^2)$   & $\n(0.2C_{t,p},100)$ & $\alpha_j = [0.2, 0.1, 0.1]$ & $[1,1,1]$ & $\Sigma_s = 10 $ & $[0.82, 0.41, 0.41]'$ & $[0, 0, 0]'$ & $ I_3$ \\
% &  & & $\alpha_{1,sim}=[0.9,0.1,0.1]$  & & $\Sigma_r = 2 I_2$  & & &  \\
%\hline
%%$\alpha_1(1) = 0.9$ while simulating the observations' sequence.
%\end{tabular}
%}
%%\end{table*}
%\label{fig2parameters}
%}
%\end{center}
%\caption{{\small  Observation depends on current temperature when sensor fails. Temperature change follows a random walk model. $N=50$.
%Fig. \ref{impsamprobust}: Model error is simulated by using $\alpha_1(1) = 0.9$ while simulating the observations' sequence.
%%System parameters are: $\Sigma_s = 10 $, $\Sigma_r = 2 I_2 $, $B_s = [0.82 \ 0.41 \ 0.41]$, $C_0 = [0 \ 0 \ 0]'$, $\sigma_{obs}^2 = [1 \ 1 \ 1]'$, $\alpha_1 = \alpha_2 = [0.2 \ 0.1 \ 0.1]$,  $p_f^1 = p_f^2 = \n(0.2 C_t, 100 I_3)$. %$N=50$. ``Out of track" \% is the percentage of realizations for which the squared error norm exceeds 24.
%%Fig. \ref{outlier_noise}: $N=50$.
%%``Out of track" \% is the percentage of realizations for which the squared error norm exceeds 12.%$\Sigma_s = 10 $, $\Sigma_r = 5 I_2 $, $B_s = [0.82 \ 0.41 \ 0.41]$, $C_0 = [0 \ 0 \ 0]'$, $\sigma_{obs}^2 = [1 \ 1 \ 1]'$, $\alpha_1 = \alpha_2= [0.4 \ 0.2 \ 0.2]$.
%%
%%Parameters for \ref{twoYmodes}: $\Sigma_s = 10 $, $\Sigma_r = 5 I_2 $, $B_s = [0.95 \ 0.21 \ 0.21]$, $C_0 = [0 \ 0 \ 0]'$, $\sigma_{obs}^2 = [1 \ 1 \ 1]'$, one sensor per node, $\alpha_1 =  [0.4 \ 0.1 \ 0.1]$, $N=50$.
%%
%}}
%\label{aa}
%\end{figure*}




%\begin{figure*}
%\begin{center}
%\subfigure[N=100, RMSE]
%{
%\psfig{file = \locc/unimod/newsims_outlier_correl_gditer5/rmse_N100_totiter50.eps, width=4cm,height=4cm}
%}
%\subfigure[N=100, Median]
%{
%\psfig{file = \locc/unimod/newsims_outlier_correl_gditer5/median_N100_totiter50.eps, width=4cm,height=4cm}
%}
%\subfigure[N=100, Out of track \%]
%{
%\psfig{file = \locc/unimod/newsims_outlier_correl_gditer5/numlarge24_N100_totiter50.eps, width=4cm,height=4cm}
%}
%\end{center}
%\caption{{\small Comparing  PF-EIS (black-$\triangle$) with PF-D (red-*) and PF-Orig (magenta-o) for Example \ref{twoYmodes} (c). Strongly correlated states, observation depends on current temperature when sensor fails. Temperature change follows a random walk model. Parameters are:
%$\Sigma_s = 10 $, $\Sigma_r = 2 I_2 $, $B_s = [0.47 \ 0.62 \ 0.62]$, $C_0 = [0 \ 0 \ 0]'$
%$\sigma_{obs}^2 = [1 \ 1 \ 1]'$, $\alpha_1 = \alpha_2 = [0.2 \ 0.2 \ 0.2]$,  $p_f^1 = p_f^2 = \n(0.2 C_t, 100 I_3)$.
%``Out of track" \% is the percentage of realizations for which the squared error norm exceeds 24.
%}}
%\label{twoYmodes}
%\end{figure*}
%%RMSE (root mean squared error), median, and percentage of times ``out of track"  when using


%
%\begin{figure*}
%\begin{center}
%%\subfigure[N=50, RMSE]
%%{
%%\psfig{file = \locc/unimod/newsims_sqr_A07/rmseN50_iters50.eps, width=4cm,height=4cm}
%%}
%\subfigure[N=50, RMSE]
%{
%\psfig{file = \locc/unimod/newsims_sqr_A07/rmseN50_iters50.eps, width=4cm,height=4cm}
%}
%\subfigure[N=50, Out of track \%]
%{
%\psfig{file = \locc/unimod/newsims_sqr_A07/numlarge20N50_iters50.eps, width=4cm,height=4cm}
%}
%\subfigure[N=50, Median]
%{
%\psfig{file = \locc/unimod/newsims_sqr_A07/medianN50_iters50.eps, width=4cm,height=4cm}
%}
%\end{center}
%\caption{{\small Example \ref{Ctsqr}:  The first sensor node observes squared temperature value (and zero sensor failure probability). One sensor per node. Observation model is $Y_{t,1} = C_{t,1}^2 + w_t, \ w_t \sim \n(0,3)$, $Y_{t,2:3} = C_{t,2:3} + w_{t}, \ w_t \sim \n(0,1)$.
%Temperature change follows an AR model with $A = 0.7 I_3$. Other parameters are:
%$\Sigma_s = 10 $, $\Sigma_r = 5 I_2 $, $B_s = [0.95 \ 0.21 \ 0.21]'$, $C_0 = [5 \ 5 \ 5]'$
%$\sigma_{obs}^2 = [3 \ 1 \ 1]'$, $\alpha_1 = 0$. % $p_f^1 = p_f^2 = \N(0.2C_t, \sigma_{obs}^2 I_3)$
%50 realizations were used.
%``Out of track" \% is the percentage of realizations for which the squared error norm exceeds 20.
%%Comparing RMSE (root mean squared error), median, and percentage of times ``out of track"  when using PF-EIS (black-$\triangle$) with that of PF-D (red-*) and PF-Orig (magenta-o).
%%State dimension $M=3$ and effective basis dim $K=1$. PF-EIS ($K=1$),  outperforms both PF-D ($K=0$) and PF-Orig ($K=M$).
%}}
%% generate an example with 0.01 failure probability (to avoid comparison with RB-PF,
%% generate an example with 100 particles
%\label{Ctsqrfigs}
%\end{figure*}


%\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|}
%\hline
%Fig. & $p_{nf}(Y_{t,p}^{(j)} | C_{t,p})$ & $p_f(Y_{t,p}^{(j)} | C_{t,p})$ & $\alpha_1, \alpha_2$ & $\sigma_{obs}^2$ & $\Sigma_s, \Sigma_r$ & $B_s$ & $C_0$ & $A$ & N \\
%\hline
%\ref{pfeisnew2N100} & $\n(C_{t,p}, \sigma_{obs,p}^2)$ & $\n(0,100)$ & $\alpha_1 = [0.9, 0.1, 0.1]$, & [10, 1, 1] & $\Sigma_s = 10$, & $[0.99, 0.1, 0.1]'$ &  $[0, 0, 0]'$ & $I_3$ & 100 \\
%& & & $\alpha_2 = [0.4, 0.01, 0.01]$ &  & $\Sigma_r = 5 I_2$ & & & & \\
%\hline
%%
%\ref{Ctsqr} & $\n(C_{t,1}^2, \sigma_{obs,p}^2)$   &  & $\alpha_1 = [0, 0, 0]$ & $[3, 1, 1]$ & $\Sigma_s = 10$, & $[0.95, 0.21, 0.21]'$ & $[5, 5, 5]'$ & $0.7 I_3$ & 50 \\
%& $\n(C_{t,p}, \sigma_{obs,p}^2)$, $p>1$ & & & & $\Sigma_r = 5 I_2$  & & & &  \\
%\hline
%%
%\ref{outlier_all} &  $\n(C_{t,p}, \sigma_{obs,p}^2)$   & $\n(0.2C_{t,p},100)$ & $\alpha_1 =  [0.4, 0.01, 0.01]$ & $[1,1,1]$ & $\Sigma_s = 10 $ & $[0.95, 0.21, 0.21]'$ & $[0, 0, 0]'$ & $ I_3$ & 50 \\
% &  & & $\alpha_2 =  [0.4, 0.01, 0.01]$ & & $\Sigma_r = 5 I_2$  & & & & \\
%\hline
%%\ref{outlier_noise} &  $\n(C_{t,p}, \sigma_{obs,p}^2)$   & $\n(C_{t,p},100)$ & $\alpha_j = [0.4, 0.2, 0.2]$ & $[1,1,1]$ & $\Sigma_s = 10 $ & $[0.82, 0.41, 0.41]'$ & $[0, 0, 0]'$ & $ I_3$ & 50 \\
%% &  & & & & $\Sigma_r = 5 I_2$  & & & & \\
%% \hline
% \ref{outlier_noise2} &  $\n(C_{t,p}, \sigma_{obs,p}^2)$   & $\n(C_{t,p},1600)$ & $\alpha_1 = [0.4, 0.1, 0.1]$ & $[1,1,1]$ & $\Sigma_s = 10 $ & $[0.95, 0.21, 0.21]'$ & $[0, 0, 0]'$ & $ I_3$ & 50 \\
% &  & & $\alpha_2 = [0.4, 0.01, 0.01]$ & & $\Sigma_r = 5 I_2$  & & & & \\
% \hline
% \ref{twoYmodes} &  $\n(C_{t,p}, \sigma_{obs,p}^2)$   & $\n(0.2C_{t,p},1)$ & $\alpha_1 = [0.4, 0.1, 0.1]$ & $[1,1,1]$ & $\Sigma_s = 10 $ & $[0.95, 0.21, 0.21]'$ & $[0, 0, 0]'$ & $ I_3$ & 50 \\
% &  & & & & $\Sigma_r = 5 I_2$  & & &  & \\
%\hline
% \ref{impsamprobust} &  $\n(C_{t,p}, \sigma_{obs,p}^2)$   & $\n(0.2C_{t,p},100)$ & $\alpha_j = [0.2, 0.1, 0.1]$ & $[1,1,1]$ & $\Sigma_s = 10 $ & $[0.82, 0.41, 0.41]'$ & $[0, 0, 0]'$ & $ I_3$ & 50 \\
% &  & & $\alpha_{1,sim}=[0.9,0.1,0.1]$  & & $\Sigma_r = 2 I_2$  & & & & \\
%\hline
%%\ref{outlier_new} &  $\n(C_{t,p}, \sigma_{obs,p}^2)$   & $\n(0.2C_{t,p},100)$ & $\alpha_j =  [0.4, 0.2, 0.2]$ & $[1,1,1]$ & $\Sigma_s = 10 $ & $[0.95, 0.21, 0.21]'$ & $[0, 0, 0]'$ & $ I_3$ \\
%% &  & & & & $\Sigma_r = 5 I_2$  & & &  \\
%%\hline
%\end{tabular}
%\label{fig1parameters}

%\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|}
%\hline
%Fig. & $p_{nf}(Y_{t,p}^{(j)} | C_{t,p})$ & $p_f(Y_{t,p}^{(j)} | C_{t,p})$ & $\alpha_1, \alpha_2$ & $\sigma_{obs}^2$ & $\Sigma_s, \Sigma_r$ & $B_s$ & $C_0$ & $A$ & N \\
%\hline
%%\ref{pfmt12fig} &  $\n(C_{t,p}, \sigma_{obs,p}^2)$   & $Unif(-10,10)$ & $\alpha_1 = [0.4, 0_9]$ & $5_{10}$ & $\Sigma_s = 10 $ & $[0.56, 0.28_9]'$ & $0_{10}$ & $ I_{10}$ \\
%% &  &  & $\alpha_2 = [0.1, 0_9]$ & & $\Sigma_r = 1 I_9$  & & &  \\
%% \hline
%\ref{pfmt3_N100fig} &  $\n(C_{t,p}, \sigma_{obs,p}^2)$   & $\n(0,100)$ & $\alpha_1 = [0.9, 0.01_9]$ & $1_{10}$ & $\Sigma_s = 10 $ & $[0.83, 0.18_9 ]'$ & $0_{10}$ & $ I_{10}$ & 100 \\
% &  & & $\alpha_2 = [0.4, 0.01_9]$ & & $\Sigma_r = 1 I_9$  & & & &  \\
%% \ref{pfmt3fig} N=50
%\hline
%\ref{pfmtsqrfig} & $\n(C_{t,1}^2, \sigma_{obs,p}^2)$   & $\n(0,100)$  & $\alpha_j = 0.001_{10}$ & $[3, 1_9]$ & $\Sigma_s = 10$, & $[0.83, 0.18_9]'$ & $5_{10}$ & $0.7 I_3$ & 50 \\
%& $\n(C_{t,p}, \sigma_{obs,p}^2)$, $p>1$ & & & & $\Sigma_r = 1 I_9$  & & & & \\
%\hline
% \ref{pfmtoutlierfig} &  $\n(C_{t,p}, \sigma_{obs,p}^2)$   & $\n(0.2C_{t,p},400)$ & $\alpha_1 = [0.4, 0.01_9]$ & $1_{10}$ & $\Sigma_s = 10 $ & $[0.83, 0.18_9 ]'$ & $0_{10}$ & $ I_{10}$ & 50 \\
% &  & & & & $\Sigma_r = 2 I_9$  & & & & \\
%\hline
%\end{tabular}
%}
%%\end{table*}
%\label{fig3parameters}
%


==> intro.tex <==

\begin{abstract}

Consider tracking a state space model with multimodal observation likelihoods using a particle filter (PF). Under certain assumptions that imply narrowness of the state transition prior, many efficient importance sampling techniques have been proposed in literature. For large dimensional state spaces (LDSS), these assumptions may not always hold. But, it is usually true that at a given time, state change in all except a few dimensions is small. We use this fact to design a simple modification (PF-EIS) of an existing importance sampling technique. Also, importance sampling on an LDSS is expensive (requires large number of particles, $N$) even with the best  technique. But if the ``residual space" variance is small enough, we can replace importance sampling in residual space by Mode Tracking (PF-MT). This drastically reduces the importance sampling dimension for LDSS, hence greatly reducing the required $N$.
\end{abstract}

{\bf Index Terms:} particle filter, mode tracking, importance sampling, Monte Carlo methods, sensor networks.

\Section{Introduction}
Tracking is the problem of causally estimating a hidden state sequence, $\{X_t\}$, from a sequence of observations, $\{Y_t\}$ that satisfy the Hidden Markov Model assumption, i.e. $X_t \rightarrow Y_t$ is a Markov chain for each $t$, with observation likelihood (OL),  $p(Y_t|X_t)$; and $X_{t-1} \rightarrow X_t$ is also Markov with state transition pdf (STP), $p(X_t|X_{t-1})$. The posterior $p(X_t|Y_{1:t}) \defn \pi_t(X_t)$. For nonlinear and/or nonGaussian state space models, $\pi_t$ can be efficiently approximated using a particle filter (PF) \cite{gordon,tutorial,mcip}. One of two main issues in PF design is the choice of importance sampling density that reduces the variance of importance weights (improves effective particle size)\cite{tutorial}.

%$p^*$ is the ``optimal" IS density but cannot be computed in closed form in most cases.
%($p(Y_t|X_t)$ as a function of $X_t$ has multiple local maxima)
%For multimodal STPs, if the number of modes and their initial locations are known, \cite{gspf} can be used.
The most commonly used importance sampling density is  the STP, $p(X_t|X_{t-1}^{i})$  \cite{gordon}(assumes nothing). But since this does not use knowledge of $Y_t$, the weight variance can be large.  For situations where the OL is multimodal, but the STP is unimodal and narrow enough to ensure that $p^*(X_t) \defn p(X_t|X_{t-1}^{i},Y_t)$ is unimodal, \cite{doucet} proposes to approximate $p^*$ by a Gaussian at its mode and importance sample from it. Other solutions that also assume $p^*$ is unimodal are \cite{tutorial,upf,volkan_is}.
In many situations, $p^*$ may be multimodal but conditioned on a small part of the state space, denoted $X_{t,s}$, it is unimodal (Assumption \ref{unimodass}). When this holds, we propose to modify Doucet \cite{doucet}'s method as follows. Let $X_t= [X_{t,s}, X_{t,r}]$.  Sample $X_{t,s}$ from its STP but compute a Gaussian approximation to $p^*(X_t|X_{t,s}^i)=p^*(X_{t,r}|X_{t,s}^i)$ about its mode and importance sample $X_{t,r}$ from it. We refer to this idea as PF-EIS (Algorithm \ref{pfeis}).

For large dimensional state spaces (LDSS), which have dimension more than 10 or 12, the number of particles required for reasonable accuracy is very large \cite{gordon,gustaffson} and this makes PF an impractical algorithm. One class of techniques for LDSS is \cite[Ch~13]{mcip},\cite{cormick} which  resample more than once within a time interval. Alternatively, if conditioned on a small part of the state ($X_{1:t,s}$), the rest ($X_{t,r}$) has a linear Gaussian state space model, Rao Blackwellization (RB-PF) \cite{chen_liu,gustaffson} can be used. Now, this assumption may not always hold.  But,  in most large dimensional systems, at any given time, ``most of the state change" occurs in a small number of dimensions (``effective basis") while the change in the rest of the state space (``residual space") is ``small" \cite{pap1,pap2}. If the variance of residual state change is ``small enough" so that Theorem \ref{unimodthm} is applicable, Assumption \ref{unimodass} will hold. In addition, if it is even ``smaller" to ensure that Theorem \ref{ismtthm} holds with a small enough $\eps$, the importance sampling of $X_{t,r}$ can be replaced by Mode Tracking (MT). We call this idea PF-MT (Algorithm \ref{pfmt}).
%from a Gaussian approximation to $p^*(X_{t,r}|X_{t,s}^i)$ about its mode can be replaced by deterministically setting $X_{t,r}^i$ equal to the mode.

%, thus greatly improving the effective particle size
MT reduces the importance sampling dimension from $\dim(X_t)$ to $\dim(X_{t,s})$ (huge reduction for large dimensional problems). Of course, the error in the estimate of $X_{t,r}$ will also increase. But for 200-250 dim problems such as contour tracking \cite{cdc06,cvpr05}, this error is more than offset by the reduction in error due to improved effective particle size. Note that PF-MT  is a generalization of the contour tracking idea of \cite{cvpr05} which was first generalized in \cite{pap1,pap2} and used in \cite{cdc06}. It can also be understood as an approximate RB-PF \cite{chen_liu,gustaffson}.% (replace the Kalman filter by a posterior Mode Tracker).
%but there were two errors in expression (10) (in defining the set $A$) of \cite{pap1} and the numerical verifications were missing. Also, in this work we present comparisons of PF-EIS with PF-Doucet \cite{doucet} and PF-Original \cite{gordon} and also of PF-MT with PF-EIS, PF-Original (small dim) and PF-Original (full). PF-MT can also be understood as an approximation to Rao-Blackwellized PF \cite{chen_liu,gustaffson} (we replace the Kalman filter by a posterior Mode Tracker).

Some example applications are as follows. (i) When there are two different types of sensors tracking temperature at one location, each with some probability of failure, OL will be bimodal if one of them fails (Example \ref{example1}). When tracking temperature at a large number of nodes in a sensor network, the state space dimension can be very large and also the number of possible OL modes can be very large. For the situation discussed  in Example \ref{example2}, Theorem \ref{unimodthm} applies with $\Delta^*=\infty$. In other situations, Theorem \ref{unimodthm} may still apply with a finite $\Delta^*$ if temperature change at a subsampled set of sensor nodes is used as the effective basis.
%Here Theorem \ref{unimodthm} applies with $\Delta^*=\infty$ if temperature change at different nodes is uncorrelated and if some nodes have zero failure probability. In other situations, Theorem \ref{unimodthm} may still apply with a finite $\Delta^*$ if temperature change at a subsampled set of sensor nodes is used as the effective basis.
(ii) In visual tracking problems such as deforming contour tracking \cite{cdc06,cvpr05,cormick} or tracking illumination change of moving objects \cite{kaleicassp}, OL is multimodal (due to multiple objects, occlusions or clutter) and state space dimension is large. %dimension of contour or of entire image.
%Here if the multimodality is only due to multiple non-overlapping objects then Theorem \ref{unimodthm} applies  with $\Delta^*=\infty$ and $X_{t,s}$= translation. It may also hold with finite $\Delta^*$ even for images with occlusions and clutter if local deformation at a subsampled set of contour points (or illumination at a subsampled set of image points) is used as the effective basis.
%

Note PF-EIS or PF-MT will still work if Theorem \ref{unimodthm} applies  most of the time. Also, if system model changes with time, effective basis dimension can be changed over time. Also, note that PF-EIS is also applicable to smaller dimensional problems and PF-MT is also useful in situations where $p^*$ is actually unimodal.% (combine Doucet \cite{doucet}'s idea with the MT step).
% in order to ensure that Theorem \ref{ismtthm} holds
%The paper is organized as follows.

{\em Organization: } In Sec. \ref{pfeissec}, we explain PF-EIS, give sufficient conditions for Assumption \ref{unimodass} to hold for an LDSS model and show how to verify these. PF-MT is explained in Sec. \ref{pfmtsec}. Comparisons with existing PF methods and discussion are given in Sec. \ref{results}.
% comparing PF-EIS and PF-MT with existing PF methods for a temperature tracking application, and discussion are given in Sec. \ref{results}.



==> ismt.tex <==

\section{PF-EIS-MT: PF-EIS with Mode Tracker}
\label{pfmtsec}
For any PF (including efficient PFs such as PF-EIS or PF-Doucet), the effective particle size \cite{tutorial,doucet} reduces with increasing dimension, i.e. the $N$ required for a given tracking accuracy increases with dimension. This makes all PFs impractically expensive for LDSS problems. We discuss one possible solution to this problem here.

%Consider designing a PF for a large dimensional tracking problem. So far we have not discussed how to address the problem of reduced effective particle size \cite{tutorial,doucet} that occurs with increasing dimension. We focus on this issue here.

%(at any given time, ``most of the state change" occurs in a small number of dimensions, while the change in the rest of the state space is small)

\subsection{PF-EIS-MT and PF-MT Algorithm}
%For most LDSS problems, the LDSS property holds, i.e. at any given time, ``most of the state change" occurs in a small number of dimensions, while the change in the rest of the state space is small.   with $L^i$ defined in (\ref{defL}) the covariance of the STP of $X_{t,r}$  of Theorem \ref{unimodthm} the HMM property (
%Now sampling $X_{t,r}^i$ from $\n(m_t^i, \Sigma_{IS}^i)$ and $\Sigma_{IS,s}^i$ denotes the $M_{r,s} \times M_{r,s}$ block of $\Sigma_{IS}^i$)
 %The state space model satisfies the HMM property (Assumption \ref{hmmass}).
 %the covariance of the STP of $X_{t,r}$

% (where  $m_{t,s}^i$ denotes the chosen $M_{r,s}$ length part of $m_{t}^i$ and $\Sigma_{IS,s}^i$ is the corresponding $M_{r,s} \times M_{r,s}$ block of $\Sigma_{IS}^i$)

Consider the LDSS model (\ref{ldssmod}). To apply PF-EIS, we split the state $X_t$ into $[X_{t,s}, X_{t,r}]$, such that $p^*$ is unimodal w.h.p. conditioned on $X_{t,s}$.
As explained earlier, this is ensured if the eigenvalues of $\Sigma_{r}$ are small enough to satisfy (\ref{suff}).
Now, because of the LDSS property, $X_{t,r}$ can further be split into $[X_{t,r,s}, X_{t,r,r}]$ so that the maximum eigenvalue of the covariance of the STP of $X_{t,r,r}$ is small enough to ensure that there is little error in approximating the conditional posterior of $X_{t,r,r}$ by a Dirac delta function at its mode. We call this the Mode Tracking (MT) approximation of importance sampling (IS), or IS-MT. We refer to $\tilde{X}_{t,s} \defn [X_{t,s}, X_{t,r,s}]$ as the ``effective" state and to $\tilde{X}_{t,r} \defn X_{t,r,r}$ as the ``residual" state. We explain IS-MT in detail below.
 %$\Sigma_{r,r}$ (

In PF-EIS, we IS  $X_{t,s}^i$ from its STP, and we EIS $X_{t,r}^i$ from $\n(m_t^i,\Sigma_{IS}^i)$ where $m_t^i$, $\Sigma_{IS}^i$ are defined in (\ref{defsigis}). Let $m_t^i = \vc{m_{t,s}^i}{m_{t,r}^i}$ and $\Sigma_{IS}^i = \matr{\Sigma_{IS,s} & \Sigma_{IS,s,r}}{\Sigma_{IS,r,s} & \Sigma_{IS,r}}$.
This is equivalent to first sampling $X_{t,r,s}^i \sim \n(m_{t,s}^i, \Sigma_{IS,s}^i)$ and then sampling $X_{t,r,r}^i \sim \n({m_{t,r}^*}^i, \Sigma_{IS,r}^i)$ where%\cite{poor}
 \bea
{m_{t,r}^*}^i \sdefn m_{t,r}^i + \Sigma_{IS,r,s}^i {\Sigma_{IS,s}^i}^{-1} (X_{t,r,s}^i - m_{t,s}^i), \nn \\
{\Sigma_{IS,r}^*}^i \sdefn \Sigma_{IS,r}^i - \Sigma_{IS,r,s}^i {\Sigma_{IS,s}^i}^{-1} {\Sigma_{IS,r,s}^i}^T
\label{defsigisrr}
\eea
%Now, $\Sigma_{IS,r,s}^i {\Sigma_{IS,s}^i}^{-1} {\Sigma_{IS,r,s}^i}^T \ge 0$.
%The second term in (\ref{defsigisrr}) is positive definite and thus  ${\Sigma_{IS,r}^*}^i \le \Sigma_{IS,r}^i$.
Now, from (\ref{defsigisrr}), ${\Sigma_{IS,r}^*}^i \le \Sigma_{IS,r}^i$.
Also, since $m_t^i$ lies in a locally convex region of $E_{Y_t}(X_{t,s}^i,X_{t,r})$, i.e. $\nabla^2 E_{Y_t} (X_{t,s}^i,m_t^i) \ge 0$ (by Theorem \ref{unimodthm}), $\Sigma_{IS}^i \le \Delta_{r}$. This implies that $\Delta_{r,r}-\Sigma_{IS,r}^i$, which is a square sub-matrix of $\Delta_{r}-\Sigma_{IS}^i$, is also non-negative definite. Thus,
%, i.e. $\nabla_{X_{t,r}}^2 E_{Y_t} (X_{t,s}^i,m_t^i) \ge 0$. Thus,
\bea
{\Sigma_{IS,r}^*}^i \le \Sigma_{IS,r}^i  \le \Delta_{r,r}
\label{Deltarrbnd}
\eea
If the maximum eigenvalue of $\Delta_{r,r}$ is small enough, any sample from $\n({m_{t,r}^*}^i, {\Sigma_{IS,r}^*}^i)$ will be close to ${m_{t,r}^*}^i$ w.h.p. So we can set $X_{t,r,r}^i= {m_{t,r}^*}^i$ with little extra error (quantified in the next subsection).
%(instead of sampling $X_{t,r,r}^i \sim \n({m_{t,r}}^*^i, {\Sigma_{IS,r}^*}^i)$).
{\em The algorithm is then called PF-EIS-MT. It is summarized in Algorithm \ref{pfeismt}.}
 A more accurate, but also more expensive modification (need to implement it on-the-fly) would be do MT on the low eigenvalue directions of $\Sigma_{IS}^i$. %eigen-
%
%We quantify the error due to this approximation in the next subsection.  computationally expensive, but
%with high probability there is little error in setting $X_{t,r,r}^i= m_{t,r,r}^i$ (instead of sampling $X_{t,r,r}^i \sim \n(m_{t,r,r}^i, {\Sigma_{IS,r}^*}^i)$).  So in PF-EIS-MT, we sample $X_{t,r,s}^i \sim \n(m_{t,s}^i, \Sigma_{IS,s}^i)$, but set $X_{t,r,r}^i= m_{t,r,r}^i$. The algorithm is summarized in Algorithm \ref{pfeismt}.
%
A simpler modification is PF-MT. In PF-MT, we combine $X_{t,r,s}$ with $X_{t,s}$ and importance sample the combined state $\tilde{X}_{t,s} = [X_{t,s},X_{t,r,s}]$ from its STP (or in some cases $X_{t,r,s}$ is empty), while performing mode tracking (MT) on $\tilde{X}_{t,r} = X_{t,r,r}$. {\em PF-MT is summarized in Algorithm \ref{pfmt}.}
% (see step \ref{weightmt}). %A further approximation sets ${\Sigma_{IS,r}^*}^i = \Delta_{r,r}$ and with this, the denominator term in the weighting step disappears.



The IS-MT approximation introduces some error in the estimate of $X_{t,r,r}$ (error decreases with decreasing spread of $\pss(X_{t,r,r})$). But it also reduces the sampling dimension from $\dim(X_t)$ to $\dim([X_{t,s} ; X_{t,r,s}])$ (significant reduction for large dimensional problems), thus improving the effective particle size. For carefully chosen dimension of $X_{t,s}$, this results in smaller total error, especially when the available number of particles, $N$, is small. This is observed experimentally, but proving it theoretically is an open problem for future research.
We say that the {\em IS-MT approximation is ``valid"} for a given choice of $X_{t,r,r}$ if it results in smaller total error than if it were not used.
% But for 100-200 dim problems such as contour tracking \cite{cdc06journal,pami07}, this error is more than offset by the reduction in error due to improved effective particle size (observed experimentally).



\subsection{IS-MT Approximation}
\label{ismtanal}
We quantify the error introduced by IS-MT. If we did not use the MT approximation,  $X_{t,r,r}^i \sim \n({m_{t,r}^*}^i, {\Sigma_{IS,r}^*}^i)$. %Let its eigenvalue decomposition is ${\Sigma_{IS,r}^*}^i = U {\Lambda_{IS,r}^*}^i U^T$.
%
But using MT, we set $X_{t,r,r}^i = {m_{t,r}^*}^i$. Consider the max norm of $e \defn  X_{t,r,r}^i - {m_{t,r}^*}^i$, denoted $||e||_\infty$. The components of $e$ are not independent, but those of $U^T e$ are independent, where ${\Sigma_{IS,r}^*}^i = U {\Lambda_{IS,r}^*}^i U^T$. Also, it is easy to see that $||e||_\infty \le \sqrt{M_{r,r}}||U^T e||_\infty$. Thus we have
\bea
&& Pr( ||e ||_{\infty} > \eps )  \le  Pr( ||U^T e ||_{\infty} > \frac{\eps}{\sqrt{M_{r,r}}} ) =  \nn \\
&& 1- \prod_{p=1}^{M_{r,r}} [1- Pr( | [U^T e]_p | > \frac{\eps}{\sqrt{M_{r,r}}})]
\eea
Combining  Vysochanskij-Petunin \cite[Pg 137]{stats} (tighter version of Chebyshev for unimodal pdfs) and Chebyshev inequalities,
\bea
Pr( | [U^T e]_p | > \frac{\eps}{\sqrt{M_{r,r}}}) & \le & \min\{1, \kappa( \frac{ M_{r,r} {\Lambda_{IS,r,p}^*}^i}{\eps^2}) \} \ \ \ \nn \\
\mbox{where~}
\kappa (x) \sdefn \left\{ \begin{array}{cc}
4x/9, & \ x < 3/8  \\
x, & \ x \ge 3/8
\end{array} \right.
\eea
\bea
\mbox{Thus,~}
&& Pr( ||e ||_{\infty} > \eps  ) \nn \\
&& \le 1 - \prod_{p=1}^{M_{r,r}} [1-  \min\{1, \kappa(\frac{M_{r,r} {\Lambda_{IS,r,p}^*}^i}{\eps^2} ) \} ]  \nn \\
\label{SigISbnd}
&& \le 1 -  [1-  \min\{1, \kappa( \frac{M_{r,r}  \max_p {\Lambda_{IS,r,p}^*}^i}{\eps^2} ) \}]^{M_{r,r}}  \ \ \   \\
\label{Sigrrbnd}
&& \le 1 -  [1-  \min\{1, \kappa(M_{r,r}  \frac{ \max_p \Delta_{r,r,p} }{ \eps^2} ) \} ]^{M_{r,r}}
\eea
(\ref{Sigrrbnd}) follows directly from (\ref{Deltarrbnd}). %Note that similar bounds also apply to $|| X_{t,r,r}^i - {m_{t,r}^*}^i ||_\infty$ (or to the Euclidean norm) but with $\eps$ replaced by $\eps/\sqrt{M_{r,r}}$.
Now, (\ref{SigISbnd}) and (\ref{Sigrrbnd}) hold almost surely for each value of $X_{1:t,s}^i,X_{1:t,r,s}^i,Y_{1:t}$. They also hold if we take $\E_{X_{1:t,s}^i,X_{1:t,r,s}^i,Y_{1:t}}[.]$ on both sides (since both left and right hand sides are bounded by 1). This leads directly to the following convergence in probability result:%and hence their difference is also bounded
%\footnote{${m_{t,r}^*}^i$ is a function of $\Delta_{r,r}$ and of $X_{t-1:t,s}^i,X_{t-1:t,r,s}^i$, $Y_t$ and  $X_{t-1,r,r}^i={m_{t-1,r}^*}^i$. ${m_{t-1,r}^*}^i$  is itself a function of $\Delta_{r,r}$ and of $X_{t-2:t-1,s}^i,X_{t-2:t-1,r,s}^i$, $Y_{t-1}$ and $X_{t-2,r,r}^i = {m_{t-2,r}^*}^i$ and so on. Thus, ${m_{t,r}^*}^i$ is a function of $\Delta_{r,r}$, $X_{1:t,s}^i,X_{1:t,r,s}^i, Y_{1:t}$.}
%the left hand side is a probability which is bounded by 1 and the right hand side is bounded by a constant). %Thus, they also holds if we took $\E_{X_{1:t,s}^i,X_{1:t,r,s}^i,Y_{1:t}}[.]$ on both sides.
%
\begin{theorem}
Consider model (\ref{ldssmod}) and assume that the conditions of Theorem \ref{unimodthm} hold. Let $X_{t,r,r}^i \sim \n({m_{t,r}^*}^i, {\Sigma_{IS,r}^*}^i)$. Given any $\eps, \eps_2 >0$, if $\max_p \Delta_{r,r,p} \le [ 1 - (1-\eps_2)^{1/M_{r,r}} ]\frac{\eps^2}{M_{r,r}}$,
$Pr( || X_{t,r,r}^i - {m_{t,r}^*}^i ||_{\infty} > \eps ) < \eps_2$, i.e. $X_{t,r,r}^i$ converges in probability to ${m_{t,r}^*}^i$ in the max norm as $\max_p \Delta_{r,r,p} \tends 0$.% goes to zero. ~$\blacksquare$%norm defined in (\ref{defnorm})
\label{ismtthm}
\end{theorem}
\begin{remark} %but averaged over $Y_t$ X_{1:t,s}^i ,Y_{1:t}
Even if the conditions of Theorem \ref{unimodthm} do not hold, we can still prove Theorem \ref{ismtthm} if we assume that ${\Sigma_{IS,r}^*}^i = Covar[\pss(X_{t,r,r})]$ (actually $\Sigma_{IS}^i$ is only an approximation to $Covar[\pss(X_{t,r,r})]$). The result will then follow directly by using the conditional variance identity \cite[Theorem 4.4.7]{stats} to show that $\E_{Y_{t}}[{\Sigma_{IS,r}^*}^i] \le \Delta_{r,r}$. ~$\blacksquare$ %$\E_{Y_t}[.]$ denotes expectation only w.r.t. $Y_t$.
%If Assumption \ref{gausspxtr} or the conditions of Theorem \ref{unimodthm} do not hold, but we can claim that\footnote{Actually $\Sigma_{IS}^i$ is only an approximation to $Covariance[\pss(X_{t,r})]$.} $\Sigma_{IS}^i = Covariance[\pss(X_{t,r})]$, then we can prove the above two results averaged over $Y_t$. $Covariance[\pss(X_{t,r})]$.
\end{remark}

In summary, PF-EIS-MT applies if $\pss(X_{t,r})$ is unimodal with high probability (needed for PF-EIS) and the largest eigenvalue of ${\Sigma_{IS,r}^*}^i$ is small enough to ensure the validity of IS-MT, i.e. the bound in (\ref{SigISbnd}) is small enough. A sufficient condition is that the largest eigenvalue of $\Delta_{r,r}$ be small enough. The best choice of $\eps,\eps_2$ of Theorem \ref{ismtthm} (to ensure maximum reduction in error) is governed by the tradeoff between the increase in error due to IS-MT and decrease in error due to the decrease in IS dimension and will be studied in future work.% ($\le \eps_2$)
%(as $\eps,\eps_2$ increase, IS dimension reduces and IS-MT error increases).% bound in (\ref{Sigrrbnd}), which is proportional to
%largest entry of $\Delta_{r,r}$ be small enough. ,
%, i.e. Theorem \ref{ismtthm} applies with a small enough $\eps_1$. The choice of $\eps_1$ is governed by the error tradeoff discussed above and will be studied in future research.
%\end{ass}

%
%Consider $e \defn X_{t,r,r}^i - m_{t,r,r}^i$ projected along the eigen-space of ${\Sigma_{IS,r}^*}^i$, i.e. consider $e_u \defn U^T e$ where ${\Sigma_{IS,r}^*}^i = U {\Lambda_{IS,r}^*}^i U^T$ is the eigenvalue decomposition of ${\Sigma_{IS,r}^*}^i$. We obtain a bound on the probability that the magnitude of any element of $e_u$ is larger than an $\eps$. To do this, consider the following max norm on $\re^{M_{r,r}}$:%
%\bea
%||x||_{mx} \defn ||U^T x||_{\infty} \defn \max_{p=1, \dots M_{r,r}} | [U^T x]_p |
%\eea
%%where $||a||_\infty \defn \max_{p} a_p$ denotes the max norm.
%Since each element of $U^T (X_{t,r,r}^i-m_{t,r,r}^i)$ is independent,
%\bea
%&& Pr( || X_{t,r,r}^i - m_{t,r,r}^i ||_{mx} > \eps ) \nn \\
%&& = 1- \prod_{p=1}^{M_{r,r}} [1- Pr( | [X_{t,r,r}^i - m_{t,r,r}^i]_p | > \eps)]
%\eea
%



%\subsection{PF-EIS-MT}
%For best performance, one may choose a smaller dimensional $X_{t,r}$ for PF-MT than that for PF-EIS, i.e. split $X_{t,r}$ for PF-EIS into $X_{t,r,s}$ and $X_{t,r,r}$ and use the MT approximation only on $X_{t,r,r}$.  So we importance sample  $X_{t,s}$ from its STP, we EIS   $X_{t,r,s}$  from a Gaussian approximation to $\pss(X_{t,r,s},X_{t-1,r,r}^i)$ and we MT on  $X_{t,r,r}$.  We call this idea PF-EIS-MT. The stepwise algorithm is given in Algorithm \ref{pfeismt}.
%
%\input{ismtpractical}

\subsection{Choosing the MT-Residual states, $X_{t,r,r}$}
\label{chooseKismt}
We first choose an $X_{t,s}, X_{t,r}$ for the EIS step using the unimodality heuristics discussed earlier in Sec. \ref{chooseKunimod}. Then we split $X_{t,r}$ into $X_{t,r,s}$ and $X_{t,r,r}$ so that IS-MT is valid for $X_{t,r,r}$. Then PF-EIS-MT can be implemented with the chosen $X_{t,s}, X_{t,r,s}, X_{t,r,r}$. Alternatively, one can implement PF-MT (faster) with $\tilde{X}_{t,s} =[X_{t,s}; X_{t,r,s}]$, $\tilde{X}_{t,r} = X_{t,r,r}$.
For a given value of $\eps, \eps_2$, two approaches can be used to choose $X_{t,r,r}$: the first uses (\ref{Sigrrbnd}) and the second uses (\ref{SigISbnd}).% based on the analysis of Sec. \ref{ismtanal}  does an approximate analysis of
\begin{heuristic}
 Begin with $M_{r,r} = M_r$ and keep reducing its value. For each value of $M_{r,r}$, choose the states with the $M_{r,r}$ smallest values of $\Delta_{\nu,r,p}$ (so that $\max_p \Delta_{\nu,r,r,p}$ is smallest) as $X_{t,r,r}$. With this choice, compute the bound of (\ref{Sigrrbnd}) and check if it is smaller than $\eps_2$. If it is smaller, then stop, else reduce $M_{r,r}$ by 1 and repeat the same steps.
\\
A second approach is to do the same thing on-the-fly, using (\ref{SigISbnd}).% This needs to be done on-the-fly.
\label{hSigrr}
\end{heuristic}
%This heuristic was used in \cite{kaleicassp}.
%Note that (\ref{SigISbnd}) also holds if expected value is taken on both sides. Let $\E[.]$ denote $\E_{X_t}[.]$. Using a first order approximation, $\E[\Sigma_{IS,r,r}^i] \approx ( \E[ \nabla_{X_{t,r,r}}^2 E_{Y_t} ] + \Delta_{\nu,r,r}^{-1} )^{-1}$.
%$\E_{X_{1:t,s}^i,X_{1:t,r,s}^i,Y_{1:t} }[.]$.
%For given $M_{r,r}$, choose the set of states for which the largest eigenvalue of this term is smallest as $X_{t,r,r}$. Thus,
%\begin{heuristic}
%Consider an observation model of the form $Y_t = h_a(X_{t,a}) h_b(X_{t,b}) + w_t$ (some examples are bearings-only tracking\cite{gordon} or Example \ref{illumtrack}). Let $X_{t,s} = X_{t,a}$. If $w_t$ is white Gaussian, $\nabla^2_{X_{t,r}} E_{Y_t} = \nabla^2_{X_{t,b}} E_{Y_t} = \sum_{k=1}^P [ h_{a,k}(X_{t,s}^i)^2  \nabla h_{b,k}(m_{t}^i)  \nabla h_{b,k}(m_{t}^i)^T - \nabla^2 h_{b,k}(m_{t}^i) (Y_{t,k} - h_{a,k}(X_{t,s}^i) h_{b,k}(m_{t}^i) ) ]/\sigma_{obs,k}^2$ where $P=\dim(Y_t)$. Choose $X_{t,r,r}$ on-the-fly by applying Heuristic \ref{hSigrr} but with $\Delta_{\nu,r,p}$ replaced by the $p^{th}$ eigenvalue of  $(\nabla^2 E_{Y_t} + \Delta_{\nu,r}^{-1} )^{-1}$. To choose $X_{t,r,r}$ a-priori, can replace $\nabla^2 E_{Y_t}$ by its expected value. If $w_t$ is not Gaussian, modify $E_{Y_t}$ and its Hessian appropriately.%
%\label{hSigIS}
% \end{heuristic}
%Heuristic \ref{hSigIS},  along with Heuristic \ref{h1}, explains the choice of $X_{t,r,r} = X_{t,r} =\lambda_t$ in Example \ref{illumtrack} \cite{kaleicassp}. %It can be shown that $\nabla^2_{X_{t,r}} E_{Y_t}$ has much larger values if $X_{t,r}=\lambda_t$ than if $X_{t,r}=u_t$.



\subsection{Connection with Rao-Blackwellized PF (RB-PF)}
\label{approxrbpf}
%PF-MT can be understood as an approximation of the RB-PF, which is  explained in detail in \cite{gustaffson}. %Consider (7) of cc.
% For simplicity of notation, assume that $X_{t,r,s}$ is empty. Then PF-EIS-MT is equivalent to PF-MT with $\tilde{X}_{t,s} = X_{t,s}$ and $\tilde{X}_{t,r} = X_{t,r}$.
%
We first discuss the connection of PF-MT to RB-PF. PF-MT can be interpreted as an approximation of the RB-PF of \cite{gustaffson}. The RBPF of \cite{gustaffson} is applicable when the state vector can be split as $X_t = [X_{t,nl},X_{t,l}]$ with the following property: $X_{t,nl}$ has any general nonlinear or non-Gaussian state space model; but conditioned on $X_{1:t,nl}$, $X_{t,l}$ has a linear Gaussian state space model. Thus the RB-PF of \cite{gustaffson} importance samples $X_{t,nl}$ from its STP but applies the Kalman recursion to compute the conditional prediction and posterior densities (both are Gaussian) of $X_{t,l}$  conditioned on each particle $X_{1:t,nl}^i$. The OL of each particle $X_{1:t,nl}^i$, is computed by marginalizing over the prediction density of $X_{t,l}$.

PF-MT can be understood as an approximation to the RB-PF in the following sense: replace the ``nonlinear" part of the state space by $\tilde{X}_{t,s}$, i.e. $X_{t,nl} \equiv \tilde{X}_{t,s}$, and the ``linear" part by $\tilde{X}_{t,r}$, i.e. $X_{t,l} \equiv \tilde{X}_{t,r}$. In PF-MT, the conditional prediction and posterior densities of $\tilde{X}_{t,r}$ (conditioned on  $\tilde{X}_{1:t,s}^i$) are assumed to be unimodal (not necessarily Gaussian), but narrow. In general, it is not possible to marginalize over any unimodal density.
% Since the prediction is not Gaussian, it is not possible to marginalize over it. RB-PF requires both densities to be Gaussian (though not necessarily narrow).
But if the product of the STP of $\tilde{X}_{t,r}$ and the OL given $\tilde{X}_{t,s}^i$ is narrow enough to be be approximated by its maximum value times a Dirac delta function at its unique maximizer, PF-MT can be interpreted as an RB-PF. In that case, the conditional posterior of $\tilde{X}_{t,r}$ is also approximated by a Dirac delta function. Thus,%
%PF-MT approximates the conditional posterior of $X_{t,r}$, conditioned on  $X_{1:t,s}^i$ by a Dirac delta function at its mode (instead of a Gaussian in case of RB-PF). Thus, in summary,
%The above can be summarized as follows.
\begin{theorem}
PF-MT (Algorithm \ref{pfmt}) is  RB-PF (Algorithm 1 of \cite{gustaffson}) with the following approximation at each $t$:
\bea
&& p(Y_t|\tilde{X}_{t,s}^i, \tilde{X}_{t,r}) p (\tilde{X}_{t,r}|X_{t-1}^i, \tilde{X}_{t,s}^i)   \nn \\
\label{pfmtapprox}
& & = p(Y_t|\tilde{X}_{t,s}^i, \tilde{X}_{t,r}^i) p (\tilde{X}_{t,r}^i|X_{t-1}^i, \tilde{X}_{t,s}^i) \delta(\tilde{X}_{t,r}-\tilde{X}_{t,r}^i) \\ %\ \mbox{where}   \\
&& \tilde{X}_{t,r}^i = m_t^i = \arg \max_{\tilde{X}_{t,r}} [ p(Y_t|\tilde{X}_{t,s}^i, \tilde{X}_{t,r}) p (\tilde{X}_{t,r}|X_{t-1}^i, \tilde{X}_{t,s}^i) ] \nn
\eea
With the above approximation, the following also holds:
\bea
\pss(\tilde{X}_{t,r}) \defn p(\tilde{X}_{t,r}|X_{t-1}^i,\tilde{X}_{t,s}^i,Y_t) = \delta(\tilde{X}_{t,r} - m_t^i) \ \ \
\eea
%i.e. when the product of the STP of $X_{t,r}$ and the OL given $X_{t,s}^i$ is narrow enough to be be approximated by its maximum value times a Dirac delta function at the maximum, RB-PF and PF-MT are equivalent. ~~$\blacksquare$
\vspace{-0.2in}
\label{pfmtrbpf}
\end{theorem}
 The proof is a simple exercise of simplifying RB-PF expressions using (\ref{pfmtapprox}) and hence is skipped.

For PF-EIS-MT, replace $\tilde{X}_{t,r}$ by $X_{t,r,r}$ and $\tilde{X}_{t,s}$ by $[X_{t,s};X_{t,r,s}]$ in the above discussion. Also, importance sampling from the STP in case of RB-PF is replaced by EIS.
%%{\em Proof: } See Appendix.
%The proof follows directly from the following Lemma.
% \begin{lemma}
%Approximation (\ref{pfmtapprox}) implies that
%\ben
%\item $\forall \ t$,  $p(X_{t,r}|X_{1:t,s}^i,Y_{1:t}) = \delta(X_{t,r}-X_{t,r}^i)$ with $X_{t,r}^i$ defined in (\ref{pfmtapprox}).
%\label{postr}
%
%\item $\forall \ t$, $p(Y_t|X_{1:t,s}^i,Y_{1:t-1}) = p(Y_t|X_{t}^i) p(X_{t,r}^i |X_{t-1}^i, X_{t,s}^i)$.%p(Y_t|X_{t,s}^i, X_{t,r}^i) p(X_{t,r}^i |X_{t-1,r}^i)$.
%\label{obslik}
%
%\item $\forall \ t$, $p(X_{t,s}|X_{1:t-1,s}^i,Y_{1:t-1}) = p(X_{t,s}|X_{t-1}^i)$. ~~$\blacksquare$
%%p(X_{t,s}|X_{t-1,s}^i,X_{t-1,r}^i)$ .
%\label{stpxts}
%\een
%\label{rbpflemma}
%\end{lemma}
%{\em Proof:} The proof is a simple exercise of simplifying RB-PF expressions using (\ref{pfmtapprox}).
%%See Appendix.


==> ismtoldtheorem.tex <==
% $X_{t,r}$ converges to $m_t^i$ in probability as $\trace(\Sigma_r) \tends 0$, for almost all values of $X_{t,s}^i, X_{t-1}^i, Y_t$. %\sum_{p=1}^{M-K} \Delta_{p+K} \tends 0


If Assumption \ref{hmmass} holds and assuming that $\Sigma_{IS}^i \approx Covariance(\pss(X_{t,r})$, we can claim that $X_{t,r}$ approaches $m_t^i$ in probability, as $\trace(\Sigma_r)$ approaches 0, for almost all values of $X_{1:t,s}^i$.

Proof:
By conditional variance identity \cite{Theorem 4.4.7]{stats}, $\E_{Y_t}[Covariance(\pss(X_{t,r})] \le Covariance(p(X_{t,r}|X_{t-1,r}^i,X_{t,s}^i) = \Sigma_r$
\bea
\ds
Pr(||X_{t,r} - m_t^{i}|| > \eps_1) \se \int Pr(||X_{t,r} - m_t^{i}|| > \eps_1 | Y_{1:t}) dY_{1:t}
\label{eq1}
\eea
Now
\bea
Pr(||X_{t,r} - m_t^{i}|| > \eps_1 | Y_{1:t}) \sle  \sum_{p=1}^{M_r} Pr([X_{t,r} - m_t^{i}]_p^2> \frac{\eps_1^2}{M_r} ) \nn \\
\sle \sum_{p=1}^{M_r} \frac{4(\Sigma_{IS}^i)_{p,p} }{9\eps_1^2/(M_r)} 
\label{eq2}
\eea
Substituting (\ref{eq2}) in (\ref{eq1}), we get
\bea
Pr(||X_{t,r} - m_t^{i}|| > \eps_1) \sle 
= \frac{4 M_r\trace(\Sigma_{IS}^i)}{9\eps_1^2} \nn \\
\sle \frac{4M \trace(\Sigma_r)}{9\eps_1^2}  % \frac{\sum_{p=1}^{M-K} \Delta_{p+K}(M-K)}{\eps^2} = %\defn \frac{\Delta_{tot}(M)}{\eps^2}
\label{convinprob}
\eea



==> ismtpractical.tex <==
\subsection{Practical Ways to Choose the MT-Residual states, $X_{t,r,r}$}
%Choosing $X_{t,r,r}$ for Applying PF-EIS-MT/PF-MT}  % instead of (\ref{Sigrrbnd})
\label{chooseKismt}
We first choose an $X_{t,s}, X_{t,r}$ for the EIS step using the unimodality heuristics discussed earlier in Sec. \ref{chooseKunimod}. Then we split $X_{t,r}$ into $X_{t,r,s}$ and $X_{t,r,r}$ so that $X_{t,r,r}$ satisfies the IS-MT assumption. Then  PF-EIS-MT can be implemented with the chosen $X_{t,s}, X_{t,r,s}, X_{t,r,r}$. Alternatively, one can implement PF-MT (faster) with $\tilde{X}_{t,s} =[X_{t,s}; X_{t,r,s}]$, $\tilde{X}_{t,r} = X_{t,r,r}$.
For a given value of $\eps, \eps_2$, two approaches can be used to choose $X_{t,r,r}$: the first uses (\ref{Sigrrbnd}) and the second does an approximate analysis of (\ref{SigISbnd}).% based on the analysis of Sec. \ref{ismtanal}
\begin{heuristic}
 Begin with $M_{r,r} = M_r$ and keep reducing its value. For each value of $M_{r,r}$, choose the states with the $M_{r,r}$ smallest values of $\Delta_{\nu,r,p}$ (so that $\max_p \Delta_{\nu,r,r,p}$ is smallest) as $X_{t,r,r}$. With this choice, compute the bound of (\ref{Sigrrbnd}) and check if it is smaller than $\eps_2$. If it is smaller, then stop, else reduce $M_{r,r}$ by 1 and repeat the same steps.
A second approach is to do the same thing using inequality (\ref{SigISbnd}). This needs to be done on-the-fly.
\label{hSigrr}
\end{heuristic}
%This heuristic was used in \cite{kaleicassp}.
%Note that (\ref{SigISbnd}) also holds if expected value is taken on both sides. Let $\E[.]$ denote $\E_{X_t}[.]$. Using a first order approximation, $\E[\Sigma_{IS,r,r}^i] \approx ( \E[ \nabla_{X_{t,r,r}}^2 E_{Y_t} ] + \Delta_{\nu,r,r}^{-1} )^{-1}$.
%$\E_{X_{1:t,s}^i,X_{1:t,r,s}^i,Y_{1:t} }[.]$.
%For given $M_{r,r}$, choose the set of states for which the largest eigenvalue of this term is smallest as $X_{t,r,r}$. Thus,
%\begin{heuristic}
%Consider an observation model of the form $Y_t = h_a(X_{t,a}) h_b(X_{t,b}) + w_t$ (some examples are bearings-only tracking\cite{gordon} or Example \ref{illumtrack}). Let $X_{t,s} = X_{t,a}$. If $w_t$ is white Gaussian, $\nabla^2_{X_{t,r}} E_{Y_t} = \nabla^2_{X_{t,b}} E_{Y_t} = \sum_{k=1}^P [ h_{a,k}(X_{t,s}^i)^2  \nabla h_{b,k}(m_{t}^i)  \nabla h_{b,k}(m_{t}^i)^T - \nabla^2 h_{b,k}(m_{t}^i) (Y_{t,k} - h_{a,k}(X_{t,s}^i) h_{b,k}(m_{t}^i) ) ]/\sigma_{obs,k}^2$ where $P=\dim(Y_t)$. Choose $X_{t,r,r}$ on-the-fly by applying Heuristic \ref{hSigrr} but with $\Delta_{\nu,r,p}$ replaced by the $p^{th}$ eigenvalue of  $(\nabla^2 E_{Y_t} + \Delta_{\nu,r}^{-1} )^{-1}$. To choose $X_{t,r,r}$ a-priori, can replace $\nabla^2 E_{Y_t}$ by its expected value. If $w_t$ is not Gaussian, modify $E_{Y_t}$ and its Hessian appropriately.%
%\label{hSigIS}
% \end{heuristic}
%Heuristic \ref{hSigIS},  along with Heuristic \ref{h1}, explains the choice of $X_{t,r,r} = X_{t,r} =\lambda_t$ in Example \ref{illumtrack} \cite{kaleicassp}. %It can be shown that $\nabla^2_{X_{t,r}} E_{Y_t}$ has much larger values if $X_{t,r}=\lambda_t$ than if $X_{t,r}=u_t$.

%
%
%Then apply Heuristic \ref{hSigrr} but with $\Delta_{\nu,r,p}$ replaced by the $p^{th}$ eigenvalue of  $( \E[\nabla^2 E_{Y_t}] + \Delta_{\nu,r}^{-1} )^{-1}$. We do an average case analysis to choose $X_{t,r,r}$ a-priori. Alternatively, this can be done on the fly by using eigenvalues of $(\nabla^2 E_{Y_t} + \Delta_{\nu,r}^{-1} )^{-1}$.%
%the dominant term of $\E[\nabla_{X_{t,r}}^2 E_{Y_t}]$ is $\E[\pdif{h}{X_{t,r}}(X_t)^T \pdif{h}{X_{t,r}}(X_t)] \defn Q$. Choose those states which have largest diagonal entries\footnote{For a symmetric matrix, largest eigenvalue is $\ge$ all diagonal entries.} in $Q + \Delta_{\nu,r}^{-1}$ as $X_{t,r,r}$.%(larger diagonal entries of $\E[\pdif{h}{X_{t,r}}^T \pdif{h}{X_{t,r}}]$ and smaller entries of $\Delta_{\nu,r}$). A simple heuristic is to

%heuristic, along with Heuristic \ref{h1} was used in choosing the illumination states as $X_{t,r,r} =X_{t,r}$ in \cite{kaleicassp} (Example \ref{illumtrack}). If $X_{t,r,r} = \lambda_t$ then the $p^{th}$ diagonal entry of $Q$ would be $\sum_{i,j} ( P_{\lambda,p}(i,j) T_0( u_{t,3}(i-u_{t,1}), u_{t,3}(i-u_{t,2}) ) )^2 + \Delta_{\lambda,p}^{-1}$. If $X_{t,r,r} =  u_t$ were used, then the first diagonal entry of $Q$ will have the form $\sum_{i,j}  ( P_{\lambda}(i,j) \lambda_t u_{t,3} \pdif{T_0}{x}( u_{t,3}(i-u_{t,1}), u_{t,3}(i-u_{t,2}) ) )^2   + \Delta_{u,1}^{-1} $ and the other two entries will also have similar order. Now for most pixels of most images, the illumination component times the x gradient of template intensity  will be much smaller than the actual template intensity. Illumination is usually less than 1 or 2, magnitude of x gradient of template is usually less than 5 or 6, while the template intensity varies between 0 and 255 (if image is histogram equalized then it varies uniformly in this range). Thus $Q$ will be much smaller in the second case than in the first. Also the variance of motion over time is smaller than that for illumination.  Thus both terms in the second case will be much smaller than in the first case. Thus, the first case was chosen.% (any histogram equalized image (usually less than 4-5) (lies between 0 to 255) , and thus the sum taken over all pixels will also be much smaller illumination ($\Delta_{\lambda,p}$) is smaller than that of motion.





==> ldss0.tex <==
%\footnote{When tracking with a Kalman filter, the same noise (with scaling 0.5 and 1) is added to both the location and velocity equations, i.e. $C_t= C_{t-1} + V_{t-1} + 0.5 n_t$, $V_t = V_{t-1} + n_t$. This is done in order to get a linear model of the form $X_t = AX_{t-1} + B n_t$. Here  But the same model can equivalently be written as $C_t = C_{t-1}+V_t$, }

\section{A Generic Class of LDSS Models}
For a large class of LDSS problems, including those discussed in the introduction, the state space model can be expressed as a generalization of the second order target motion model as follows %(replace ``velocity" by time derivative of state, replace Euclidean space by a smooth manifold with tangent space mappings defined, and replace observed position by some nonlinear function of the position plus some noise):
\bea
V_t \se f_V( V_{t-1} ) + n_t, \ \ n_t \sim \n(0,\Sigma_n), \nn \\
C_t \se C_{t-1} + g_{C_{t-1}}(V_t)  \nn \\
Y_t \se h(C_t, w_t), \ \ w_t \sim p_w(.)
\label{ldssmod0}
\eea
where the noises $n_t$, $w_t$ are independent of each other and over time.
The quantity $C_t$ may denote the $M$ contour point locations (in case of contour tracking) or it may denote temperature, or any other physical quantity, at $M$ sensor nodes (in case of temperature tracking). The quantity $V_t$ denotes its time derivative (normal direction contour point velocity in case of contour tracking) and is assumed to follow a first order Markov model. If $C$ belongs to a space $\spc$, then $g_C(V)$ denotes the mapping from the tangent space at $C \in \spc$ to $\spc$. For Euclidean spaces, $\spc = \re^M$ and so $g_C(V) \equiv V$.
As an aside, note that the system noise dimension here is $M = \dim(V_t)$ and we claim that the state $X_t = [C_t, V_t]$ has dimension $M$ (and not $2M$). This is analogous to the 1D second order target motion model case\footnote{The commonly used form of the 1D target motion model (follows by using central differences to approximate the derivative of target location) is $C_t = C_{t-1} + V_{t-1} + 0.5 n_t$, $V_t = V_{t-1} + n_t$. But, instead if we use forward differences, we get $C_t = C_{t-1}+V_t$, $V_t = V_{t-1} + n_t$ which is the same as (\ref{ldssmod0}) with $g_C(V)=V$ and $f_V(V)=V$. In either case, noise is 1D not 2D and hence state dimension is 1D}. For this, and many other tracking problems in PF, one can distinguish between an ``accumulator state" and a ``noisy state". Accumulator state (here $C_t$) is a deterministic function of the previous state and the current value of the noisy state, i.e. given the noisy state its STP is degenerate. Noisy state (here $V_t$) has a non-degenerate pdf. The state dimension is equal to the noisy state dimension. %and this governs the number of particles required.

By taking the eigenvalue decomposition of $\Sigma_n$, (\ref{ldssmod0}) can be rewritten so as to separate out the large and small variance STP directions. Let the EVD of $\Sigma_n = B \Sigma_\nu B^T$. Also, let the projections of $V_t$, $n_t$ along $B$ be $v_t \defn B^T V_t$, $\nu_t \defn B^T n_t$.  Redefining the state $X_t = [C_t,v_t]$, (\ref{ldssmod0}) can be rewritten as:
\bea
v_t \se B^T f_V( B v_{t-1}) + \nu_t,  \nu_t \sim \n(0,\Sigma_\nu),  \Sigma_\nu \defn diag(\Delta_{v,p})_{p=1}^M  \nn \\
C_t \se C_{t-1} + g_{C_{t-1}}(B v_t)    \nn \\
Y_t \se h(C_t, w_t), \ \ w_t \sim p_w(.)
\label{ldssmod}
\eea
Note that in the above, we are diagonalizing the covariance of noise $n_t$, in order to get a model s.t. the different components of noise $\nu_t$ are independent. The different components of $v_t$ are not independent, except when $f_V(V) = a V$ where $a$ is a scalar. In this case, $B$ also diagonalizes the covariance of $V_t$ at any $t$ and so $v_t$ components are independent. All examples simulated in this paper use $f_V(V) = a V$.
Also note that in certain problems, the model may directly be specified in the form (\ref{ldssmod}) (with independent noise components). We discuss some examples below. Also note that sometimes the observation model may be implicitly specified by only defining $p(Y_t|C_t) \defn \beta \exp[-E_{Y_t}(C_t)]$.
%, instead of (\ref{defyt}). But any OL can be expressed in either form. Henceforth, we use the following form for OL:
%\bea
%p(Y_t|C_t) \defn \beta exp[-E_{Y_t}(C_t)]
%\eea

%u_t \se u_{t-1} + n_{t,u}, \ \ n_{t,u} \sim \n(0, \Sigma_u)  \\
%\lambda_t \se lambda_{t-1} + n_{t,\lambda}, \ \ n_{t,\lambda} \sim \n(0, \Sigma_\lambda),  \\
%C_t (i,j)
%Y_t(i,j) \se C_t(i,j) +
%Note here  $g_{C_{t-1}}(B v) (i,j) = -C_{t-1}(i,j) + \mbox{the last term in (\ref{defintensity})}$ and
%g_{C_{t-1}}(B v) (i,j) \se -C_{t-1}(i,j) + ( B_{\lambda}(i,j) \lambda_t ) T_0( u_{t,3}(i-u_{t,1}), u_{t,3}(i-u_{t,2}) )
%$B = [B_{\lambda}, I_3]$,

\subsection{Unimodality Result applied to the LDSS model}
Consider any model of the form (\ref{ldssmod}). Assume that $v_t$ can be partitioned into $v_t = [v_{t,s}', v_{t,r}']'$ where $v_{t,s}$ denotes the temperature change coefficients along the effective basis, while $v_{t,r}$ denotes the residual space coefficients. Similarly partition $B = [B_s, B_r]$, $\Sigma_\nu = diag(\Sigma_s, \Sigma_r)$ and $\nu_t = [\nu_{t,s}', \nu_{t,r}']'$. We discuss how to select $v_{t,s}$ and $v_{t,r}$ in the next section. For now, assume that the choice of effective basis state $X_{t,s} = v_{t,s}$ is given. Then $X_{t,r} = [v_{t,r}, C_t]$. The effective basis dimension, $K = \dim(v_{t,s})$ and so $M_r = M-K$.

For simplicity of notation, first consider the case of a vector space, i.e. $\spc = \re^M$ so that $g_C(V)  = V$.
Denote
\bea
\chat^i \sdefn C_{t-1}^i + B_s v_{t,s}^i, \\
\fr \sdefn   B_r^T f_V(B v_{t-1}^i)
\eea
Then we have
\bea
&& \pss(v_{t,r}, C_{t}) \nn \\
&& = p(v_{t,r}, C_t | v_{t-1}^i, C_{t-1}^i, v_{t,s}^i, Y_t) \nn \\
&& = \beta  \n(v_{t,r}; \fr, \Sigma_r) \delta(C_t - [\chat^i + B_r v_{t,r}]) \ p(Y_t|C_t)  \nn \\ %&& \propto
&& = \underbrace{\beta  \n(v_{t,r}; \fr, \Sigma_r)  p(Y_t|\chat^i + B_r v_{t,r})}_{\pss(v_{t,r})} \delta(C_t - [\chat^i + B_r v_{t,r}]) \nn %\nn \\
%&& \defn \pss(v_{t,r}) \  \delta(C_t - [\chat^i + B_r v_{t,r}])
\eea
where $\delta$ denotes the Dirac delta function.
Since $C_t$ is an accumulator state (a deterministic function of $C_{t-1}^i, v_{t,s}^i, v_{t,r}$), its pdf is a Dirac delta function (which is trivially unimodal at $\chat^i + B_r v_{t,r}$). Thus for the purpose of importance sampling, $X_{t,r} = v_{t,r}$ only, and we need conditions to ensure that $\pss(v_{t,r})$ is unimodal. Define $L^i(v_{t,r}) = -\log \pss(v_{t,r}) + \const$ as
\bea
L^i = E(\chat^i + B_r v_{t,r}) + \sum_{p=1}^{M-K} \frac{ ( [v_{t,r} - \fr ]_p )^2 }{ 2 \Delta_{p+K} }
\label{defLm1}
\eea
Applying Theorem \ref{unimodthm} to $L^i$ defined in (\ref{defLm1}) we get the following result.
\begin{corollary}
Consider model (\ref{ldssmod}) with $g_C(V) \equiv V$. $\pss(v_{t,r})$ is unimodal ($L^i$ defined in (\ref{defLm1}) has a unique minimizer) if Assumptions \ref{hmmass} and \ref{gausspxtr} and the conditions of Theorem \ref{unimodthm} hold with the following substitutions:
\\ $X_{t,s} \equiv v_{t,s}$, $X_{t,r} \equiv v_{t,r}$,  $M_r \equiv M-K$,
 $\Delta_{r,p} \equiv (\Sigma_r)_{p,p}$,   %\Delta_{p+K}$,
 $\fr \equiv B_r^T f_V(B v_{t-1}^i)$,
 $\nabla E \equiv B_r^T \nabla_C E (\chat^i + B_r v_{t,r})$, ~~ $\nabla \Dnum \equiv v_{t,r} - \fr$,
 $\R_{LC} \subseteq \re^{M-K}$ is the largest contiguous region in the neighborhood of $\fr$ where $E(\chat^i + B_r v_{t,r})$ is convex as a function of $v_{t,r}$ (i.e. $\nabla_{v_{t,r}}^2 E \ge 0$). ~~$\blacksquare$
%$E(X_{t,s}^i, X_{t,r}) \equiv E(\chat^i + B_r v_{t,r})$.
\label{ldssvec}
\end{corollary}

When $\spc$ is not a vector space, for example for contour tracking or for landmark shape tracking,  $g_C(v)$ is not the identity map. In that case, $L^i$ is defined as
\bea
L^i \se E(C_{t-1}^i + g_{C_{t-1}^i}(B_s v_{t,s}^i + B_r v_{t,r}) ) \nn \\
   && + \sum_{p=1}^{M-K} \frac{ ( [v_{t,r} - \fr) ]_p )^2 }{ 2 \Delta_{p+K} }
\label{defLm2}
\eea
%Then we have the following result.
\begin{corollary}
Consider (\ref{ldssmod}) with any general $g_C(V)$. In this case Corollary \ref{ldssvec} applies with the following two changes:
\\ $\nabla E \equiv B_r^T  [\pdif{g}{V}(B_s v_{t,s}^i + B_r v_{t,r})]^T \nabla_C E (C_{t-1}^i + g_{C_{t-1}^i}(B_s v_{t,s}^i + B_r v_{t,r}) )$, and
$\R_{LC} \subseteq \re^{M-K}$ is the largest contiguous region in the neighborhood of $\fr$ where $E(C_{t-1}^i + g_{C_{t-1}^i}(B_s v_{t,s}^i + B_r v_{t,r}) )$ is convex as a function of $v_{t,r}$ (i.e. $\nabla_{v_{t,r}}^2 E \ge 0$). ~~$\blacksquare$
\label{ldssnvec}
\end{corollary}
%$\pss(v_{t,r})$ is unimodal ($L^i$ defined in (\ref{defLm2}) has a unique minimizer) if Assumptions \ref{hmmass} and \ref{gausspxtr} and the conditions of Theorem \ref{unimodthm} hold with the following substitutions:
%\\ $X_{t,s} \equiv v_{t,s}$, $X_{t,r} \equiv v_{t,r}$,  $M_r \equiv M-K$,  $\Delta_{r,p} \equiv (\Sigma_r)_{p,p}$,   %\Delta_{p+K}$, $\fr \equiv B_r^T f_V( B v_{t-1}^i)$, $\nabla E \equiv B_r^T  [\pdif{g}{V}(B_s v_{t,s}^i + B_r v_{t,r})]^T \nabla_C E (C_{t-1}^i + g_{C_{t-1}^i}(B_s v_{t,s}^i + B_r v_{t,r}) )$,  $\nabla \Dnum \equiv v_{t,r} - \fr$, $\R_{LC} \subseteq \re^{M-K}$ is the largest contiguous region in the neighborhood of $\fr$ where $E(C_{t-1}^i + g_{C_{t-1}^i}(B_s v_{t,s}^i + B_r v_{t,r}) )$ is convex as a function of $v_{t,r}$ (i.e. $\nabla_{v_{t,r}}^2 E \ge 0$). ~~$\blacksquare$



\subsection{Application to Temperature Tracking}
We demonstrate how to verify the conditions of Corollary \ref{ldssvec} using a temperature tracking example with $M=3$, $K=1$, i.e. $M_r = 2$. We use numerical (finite difference) computations of gradients. Here $\eps_0$ needs to be chosen carefully, depending on the resolution of the discretization grid of $v_{t,r}$. It should be just large enough\footnote{If $\eps_0$ is too small, $\nep$ may transition from a value smaller than $-\eps_0$ to a value larger than $+\eps_0$ (or vice versa) over one grid point, and this region will not be included in $\Z_p$ (even if $\ndp$ has the same sign as $\nep$), thus getting a wrong (too large) value of $\Delta^*$. If $\eps_0$ is larger than required, the region $\Z_p$ may be bigger than needed, thus giving a smaller value $\Delta^*$ than what can actually be allowed.} so that one does not miss any stationary point of $E$.

\begin{example}[Temperature Change]
Consider tracking temperature at $M$ locations. $\spc$ is a Euclidean space and so $g_C(V) \equiv V$.   $C_{t,p}$ denotes temperature at node location $p$ ($p=1,2, \dots M$). $V_{t,p}$ denotes the first derivative of temperature at node $p$ which is assumed to be zero mean.
For simplicity, we assume $f_V(V) = aV$ \footnote{$a=1$ if temperature change follows a random walk model, while $a<1$ if it follows a first order AR model}, and hence $B^T f_V(B v_{t-1}) = a v_{t-1}$. Thus $B= [B_s, B_r]$ are also the eigenvectors of the covariance of $V_t$ (since $Covar(V_t)$ is a scalar multiple of $\Sigma_n$). Temperature change, $V_t$, is spatially correlated, i.e. $B \neq I$.

%and $Y_{t,p}$ denotes observed values of temperature obtained from $J$ ($J=1$ or 2) sensors located at node $p$
 Temperature at each location, $p$, is measured using $J$ ($J=1$ or 2) types of sensors that have failure probabilities $\alpha^j(p), j=1,2$. The observation is denoted  $Y_{t,p}^j, j=1,2$. Failure of all the $2M$ sensors is independent.
If the sensor is working, the observation is the actual temperature (or some function of it) plus Gaussian noise. The noise is independent of noise in other sensors. Two types of sensor failure models are considered. The first is temperature independent failure (TIF), i.e. when a sensor fails it outputs a random number that is independent of the true temperature value. The second is temperature dependent failure (TDF), i.e. when a sensor fails it outputs a random number that depends (usually weakly) on the true temperature value. The general form of the OL is:
\bea
p(Y_t|C_t) \se \prod_{p=1}^M  p(Y_{t,p}^1|C_{t,p}) p(Y_{t,p}^2|C_{t,p}) \nn \\
p(Y_{t,p}^j|C_{t,p}) \se (1-\alpha_p^j)  \n(Y_{t,p}^j; h(C_{t,p}), {\sigma_{obs}}^2)  + \nn \\
 &&   \alpha_p^j \   p_f^j(Y_{t,p}^j|C_{t,p}),  \ j=1,2, \ p=1,\dots M \ \ \ \ \ \ \ \
\label{sensorobsmod}
\eea
In the current example, we use $h(C_{t,p}) = C_{t,p}$ (direct sensor) and TIF, i.e. $p_f^j(Y_{t,p}^j|C_{t,p}) = p_f^j(Y_{t,p}^j)$. Other models for $h$ and for $p_f$ are considered in the simulation section. %The form of this model is a very common one. It is also the same model used for modeling clutter in traditional radar tracking applications \cite{barshalom} or also in contour tracking applications \cite{condensation}.
%
Let $M=3$ and $K=1$ and let $v_{t,s} = v_{t,1}$ and $v_{t,r} = v_{t,2:3}$, i.e $v_{t,r} \in \re^2$. We show in Fig. \ref{computeDelta} how to verify the conditions of Corollary \ref{ldssvec}. Assume a given value of $C_{t-1}^i$, $\fr$ and of $Y_t$.
We first verify condition \ref{close} and then use (\ref{suff}) to find $\Delta^*$ which is the upper bound on $\max(\Delta_2, \Delta_3)$ to ensure that $\pss(v_{t,r})$ is unimodal. Here $\reg = \cap_{p=1}^2 (\A_p \cup \Z_p)$ is a subset of $\re^2$ and is a union of 4 regions: $\A_{1} \cap \A_{2}$, $\Z_{1} \cap \A_{2}$, $\A_{1} \cap \Z_{2}$, $\Z_{1} \cap \Z_{2}$.
%we use condition \ref{suffdeltacond} (which is sufficient for condition \ref{deltacond}), i.e. we compute $\Delta^*$ which is an upper bound on $\Delta_2, \Delta_3$.
%Since the second term of (\ref{defLm1}) is strongly convex with minimizer $\fr$ which belongs to $\R_{LC}$, there is no point in $\R_{LC}^c$ where both $[\nabla \Dnum]_1 = 0$ and $[\nabla \Dnum]_2 = 0$. Thus $\Z_{1} \cap \Z_{2}$ will always be an empty set.
% for which we calculated $\Delta^*=4.84$.
\label{example1}
\end{example}

%Two types of $h$ models are simulated: $h(C_{t,p}) = C_{t,p}$ is called a regular sensor (RS) while $h(C_{t,p}) = C_{t,p}^2$ is called a squared sensor (SS). distributed according to a pdf $p_f^j(y), \ j=1,2$.   Thus we have the following OL:

%  p_f^j(Y_{t,p}^j),  \ j=1,2, \ p=1,\dots M \ \ \ \ \ \ \ \
% The eigenvectors of the covariance of $V_t$ (same as the eigenvectors of $n_t = V_t-V_{t-1}$ since $A_v=aI$) are $[B_s \ B_r]$ and the eigenvalues are $\{\Delta_p\}_{p=1}^M$. The coefficients along $B_s, B_r$ are $v_{t,s},v_{t,r}$. These are assumed to follow a random walk model.

%The above sensor failure model is a very common one. It is also the same model as that used for clutter in traditional radar tracking applications \cite{barshalom} (e.g. if one gets two radar observations, both could be from the target, or one or both could be due to clutter). It is also similar to the clutter model used in contour tracking papers such as Condensation \cite{condensation} where false edges result because of background clutter. The same model is also used in \cite{cdc06} where we show application of PF-MT for contour tracking.







\subsection{Some More Examples}
{\em Temperature Change. } $C_{t}$ may denote temperature at $M$ locations in a region and $V_t$ its time derivative. This is described in detail in Example \ref{example1}.


{\em Contour Deformation. }
For the contour tracking application \cite{cdc06}, $C_t$ denotes the contour and $v_t = [\rho_t, v_{d,t}]$ where $\rho_t$ denotes translation and $v_{d,t}$ denotes deformation. $B = [I_2, B_s, B_r]$ with $B_s$ denoting the B-spline basis to interpolate deformation velocity at subsampled arclength locations onto all arclength locations and $B_r$ is the orthogonal complement of $B_s$. Here $\Sigma_\nu = diag(\Sigma_\rho, \Sigma_d)$ where both $\Sigma_\rho, \Sigma_d$ are modeled to be diagonal matrices, so that the model fits the form (\ref{ldssmod}) ????
Also, $E_{Y_t}(C_t)$ is any edge or region based segmentation energy and
\bea
[g_{C}(Bv)]_p \se ( \ [[B_s,B_r] v_d]_p  +  \N( [C]_p)^T \rho \ ) \ \N( [C]_p) \nn
\eea
 where $\N( [C]_p)$ denotes the normal direction to the contour at point $[C]_p$.  %and $h(C_t,w_t)$ models the edge based OL given in Condensation \cite{condensation}.
 %To verify condition \ref{deltacond}, we compute $\Delta^*$ defined in (\ref{suff}) and check if  $\Delta_2, \Delta_3$ are smaller than it.


{\em Illumination and Motion. } %Product of functions of subsets of states:
The illumination and motion tracking model of \cite{kalecvpr} can be rewritten in the form (\ref{ldssmod}) with $C_t = [ u_t, \lambda_t]$ where $\lambda_t$ are coefficients of the Legendre polynomial basis functions (denoted $P_{\lambda}$), used to parameterize spatial illumination variation and $u_t$ denotes the motion (x-y translation and scale) parameters. Also,  $A_v = 0$ (first order Markov model on $\lambda_t$,$u_t$), $B = I$, $\Sigma_\nu = diag(\Sigma_u, \Sigma_\lambda)$, $g_{C_{t-1}}(B v_t) =  B v_t = v_t$. Unlike the previous two examples, in this case, the observation, $Y_t$ (the image intensity) is a {\em product of functions of subsets of states}, i.e.
\bea
%g_{C_{t-1}}(B v_t) \se  B v_t = v_t,  \\
h(C_t, w_t)(i,j) \se ( P_{\lambda}(i,j) \lambda_t ) T_0( u_{t,3}(i-u_{t,1}), u_{t,3}(i-u_{t,2}) ) \nn \\
&& \ + \  w_t(i,j), \nn \\
 w_t(i,j) & \sim & (1-\alpha) \n(0,\sigma_{obs}^2) +  \alpha  \n(\mu,b\sigma_{obs}^2)
 \label{defintensity}
\eea
where $(i,j)$ denotes the $(i,j)^{th}$ pixel and $T_0(i,j)$ is the original template's intensity at $(i,j)$. The noise, $w_t(i,j)$, is the CCD sensor noise with probability $(1-\alpha)$ and with small probability $\alpha$, it is large variance outlier noise ($b>>1$).
%$Y_t(i,j)$ is the observed image intensity at pixel $(i,j)$

{\em Landmark Shape Change. }
% (aligned with previous orthogonal basis)
For the landmark shape tracking application \cite{cdc05, tip}, $C_t = [l_t, \theta_t, z_t]$, where $l_t$ denotes
log-scale, $\theta_t$ denotes rotation and $z_t$ denotes shape. $v_t = [v_{l,t}, v_{\theta,t}, v_{z,t}]$, where $v_{l,t}, v_{\theta,t}$ denote time derivative of log-scale, and of rotation (rotation velocity) and $v_{z,t}$ denotes the coefficients of time derivative of shape, defined in tangent space to shape space at $z_{t-1}$. Also, $B = [I_2, U(z_{t-1})]$ where $U(z_{t-1})$ denotes an orthogonal basis for this tangent space, $A_v=diag(1,1,A_{z})$, $\Sigma_\nu = diag(\sigma_{l}^2,\sigma_{\theta}^2, \Sigma_{z})$, and
\bea
g_{C_{t-1}}(Bv_t) \se [v_{l,t}, v_{\theta,t}, \sqrt{1-z_{t-1}^* z_{t-1}}v_{z,t} + v_{z,t}]
\eea
Also, here again, the observation $Y_t$ (observed landmark locations) is a {\em product of functions of subsets of states}, i.e.
\bea
h(C_t,w_t) \se e^{l_t + j \theta_t} z_t + w_t
\eea



 %Conditions of Theorem \ref{unimodthm}}
%%Also, we need to define $\R_{K,LC}$ as the region in the neighborhood of $\chat^i + B_r \fr$ where $\nabla^2 E > -\eps_0$.
%
%When trying to verify (\ref{suff}) for the model of (\ref{sysmod2}) using numerical (finite difference) computations of gradients and Hessians, $0$ needs to be replaced by a small number $\eps_0>0$, i.e. we need conditions to ensure $|[\nabla L]_p| > \eps_0$ for some $p$ for all $v_{t,r} \in \R_{LC}^c$.  To ensure $|[\nabla L]_p| > \eps_0$ for some $p$ for all $v_{t,r} \in \R_{LC}^c$, we need to redefine\footnote{
%To ensure $|[\nabla L]_p| > \eps_0$, we need to modify the first row for $\gamma_p$. The definition of $\A_p$ does not change. But the region $\Z_{p}$ needs to be redefined to  include all points where $|[\nabla E]_p| < \eps_0$ (irrespective of the value of $\nabla \Dnum$). This is because if $\Delta_{p+K}$ is large enough,  $[\nabla E]_p + [\nabla \Dnum]_p/\Delta_{p+K}$ can be less than $\eps_0$ even when $[\nabla \Dnum]_p  > \eps_0$. Also with this change in the definition of $\Z_p$,   the smallest acceptable value of $\Delta_{p+K}$ inside $\Z_{p}$ is actually greater than zero, i.e. it is $\frac{|[\nabla \Dnum]_p|}{\eps_0 -|[\nabla E]_p|}$, thus the modification to the second row of $\gamma_p$.}
%$\Z_{p}$ and $\gamma_p(v_{t,r})$ as follows:
%\bea
%\gamma_p(v_{t,r}) \sdefn \left\{ \begin{array}{cc}
%                     \frac{|[\nabla \Dnum]_p|}{\eps_0 +|[\nabla E]_p|}, & \ \ \ \ v_{t,r} \in \A_{p} \\ \\
%                     \frac{|[\nabla \Dnum]_p|}{\eps_0 -|[\nabla E]_p|} ,   & \ \  \ \ v_{t,r} \in \Z_{p}
%                     \end{array}
%                     \right.  \nn \\ \nn \\
%\Z_{p} \sdefn \{v_{t,r} \in \R_{LC}^c: |[\nabla E]_p| < \eps_0,  \& [\nabla E]_p. [\nabla D]_p \ge 0 \} \nn
%\eea
%%Note that  $\Z_{p}$ as defined in Theorem \ref{unimodthm} will result in an empty set in numerical computation. As soon as we replace $0$ by $\eps_0$ there

% Theorem \ref{unimodthm}


%Now for $M-K=2$, we need to find the smallest value of $\max \{\gamma_1(v_{t,r}), \gamma_2(v_{t,r}) \}$  over all $v_{t,r} \in \reg$.
% \prod_{p=1}^M p(Y_{t,p}^1, Y_{t,p}^2|C_{t,p}) =%and $E(C_t) = -\log [p(Y_t|C_t)]$.
%With slight abuse of notation, define
%\bea
%\pss(v_{t,r}) \defn p(Y_t|\chat^i + B_r v_{t,r}) \n(v_{t,r}; f_{v,r}(v_{t-1,r}^i), \Sigma_r)
%\eea
%We obtain the condition for unimodality of $\pss(v_{t,r})$ (conditions for unique


==> notation.tex <==

\section*{Notation and Acronyms}
Most notation and acronyms of the paper are defined when they are used. We summarize them again here for ease of review.

\ben

\item We use the following notation for a pdf (probability density function), $f_X(X) \defn p(X)$ and conditional pdf $f_{X|Y}(X|Y) \defn p(X|Y)$.

\item OL denotes Observation Likelihood, $p(Y_t|X_t)$.

\item STP denotes state transition pdf, $p(X_t|X_{t-1})$.

\item We use
$[.]_p$ to denote the $p^{th}$ coordinate of a vector

\item
$M = \dim(X_t)$, $K=\dim(X_{t,s})$, $M_r = M-K = \dim(X_{t,r})$

\item
\bea
p^{*}(X_{t}) \defn  p(X_{t}|X_{t-1}^{i}, Y_t) \nn
\eea

\item
\bea
p^{**,i}(X_{t,r}) \defn p^*(X_t|X_{t,s}^i) = p(X_{t,r}|X_{t-1}^{i},X_{t,s}^i, Y_t) \nn
\eea

\item
\beq
E(X_t) \defn -\log p(Y_t|X_t) + \const \nn
\eeq

\item
By Assumption \ref{gausspxtr}, the STP of $X_{t,r}$ is
\bea
p(X_{t,r}|X_{t-1}^{i},X_{t,s}^i) \se \n(X_{t,r}; f_r^i, \Sigma_r), \ \mbox{where} \nn \\
\Sigma_r \se diag\{\Delta_{r,p}\}_{1}^{M_r} \nn \\
f_r^i \sdefn f_r(X_{t-1}^{i},X_{t,s}^i) \nn
\eea

\item
\bea
m_t^i \se m_t^i(X_{t-1}^i,X_{t,s}^i,Y_t) \defn \min_{X_{t,r}}  L^i(X_{t,r}), \  \nn \\
\Sigma_{IS}^i \sdefn [(\nabla^2 L^i)(m_t^i)]^{-1}, \ \ \mbox{where} \nn \\
L^i(X_{t,r}) \sdefn -\log[ p^{**,i}(X_{t,r})] + \const \nn \\
%\se E(X_{t,s}^i,X_{t,r}) +  \underbrace{ \sum_{p=1}^{M_r}  \frac{[\Dnum(X_{t,r}, f_r^i)]_p}{ \Delta_{r,p} } }_D
\se E(X_{t,s}^i,X_{t,r}) +  \underbrace{ \sum_{p=1}^{M_r}  \frac{( [X_{t,r}- f_r^i]_p )^2}{2 \Delta_{r,p} } }_{D(X_{t,r}, f_r^i)} \nn
\eea

\item
 $\Dnum$ denotes the vector of numerators of the $M_r$ terms of $D$, i.e.
\bea
[\Dnum]_p \defn \frac{ ( [X_{t,r}- f_r^i]_p )^2 }{ 2 }, \ \forall p=1, \dots M_r \nn
\eea

\item
For the model of (\ref{sysmod2}), define
\bea
\chat^i \defn C_{t-1}^i + B_s v_{t,s}^i \nn
\eea

\een




==> pfeismtass.tex <==


\begin{algorithm*}[t!]   %\begin{algorithmic} [1]
\caption{{\small \bf PF-EIS-MT-Assumption Verification. Going from $\pi_{t-1}^N$ to $\pi_t^N(X_t) = \sum_{i=1}^N \wi \delta(X_{t} - X_{t}^{i})$ }}
\label{pfeismtass}
Let $K_2$ denote the effective basis dimension for the MT step, and let $K< K_2$ denote the effective basis dimension for the EIS step, i.e. we importance sample from the STP on $X_{t,1:K}$, we use EIS on $X_{t,K+1:K_2}$ and we replace IS by MT on $X_{t,K_2+1:M}$. $K$ is chosen on the fly (depends on the particle and the observation).
\\
\\ {\bf Choosing $K_2$: } For a given $\gamma, \eps_2$, choose $K_2$ as the smallest $K$ that satisfies (\ref{chooseK}).
\\
\\ At $t$, for particle $i$, do ~~~~~~~ \% {\em \small Importance Sampling (and Mode Tracking) and Weighing steps for particle $i$ at time $t$ }
\ben
\item
Set  $K \longleftarrow 0$.
\\ Set $\fr \longleftarrow f_r(X_{t-1}^i,[ \ ])$.
\\ Set $EConvex \longleftarrow 1$ if  $\nabla^2 E(\fr) ) \ge 0 $, else set $EConvex \longleftarrow 0$
\\ Compute $\Delta^*=\Delta^*(\fr,[ \ ],Y_t,M-K)$ using (\ref{suff}).

\item {\em While $EConvex==1$ and $\max_{p=1, \dots M-K} \Delta_{p+K} > \Delta^*$ and $K < K_2$ do }
\ben
\item $K \longleftarrow K + 1$
\item {\em Importance Sample $X_{t,K}$ from its STP}, i.e.  $X_{t,K}^i \sim  p(X_{t,K}^i|X_{t-1}^i,X_{t,1:K-1}^i)$.
\item Set $X_{t,s}^i \longleftarrow X_{t,1:K}^i$ %,  $X_{t-1,r}^i \longleftarrow X_{t-1,K+1:M}^i$
\label{defxtsi}
\item Set $\fr \longleftarrow f_r(X_{t-1}^i,X_{t,s}^i)$
\label{deffri}
\item Set $EConvex \longleftarrow 1$ if  $\nabla^2 E(\fr) ) \ge 0 $, else set $EConvex \longleftarrow 0$.
\item {\em Compute $\Delta^*=\Delta^*(\fr,X_{t,s}^i,Y_t,M-K)$ using (\ref{suff}). }
\een
{\em End While }

\item {\em Efficient Importance Sample $X_{t,K+1:K_2}$: } Sample $X_{t,K+1:K_2}^i \sim \n(m_{t,r,s}^{i}, \ \Sigma_{IS}^{i})$. Here $m_{t,r,s}^{i}(X_{t-1}^i,X_{t,1:K}^i,Y_t) =  \arg \min_{X_{t,K+1:K_2}} L^i(X_{t,K+1:K_2})$, $\Sigma_{IS}^{i}\defn (\nabla^2 L^i(m_{t,r,s}^{i}))^{-1}$ where $L^i$ is defined in step \ref{isxtreismt} of Algorithm \ref{pfeismt}.
%where $L^i(X_{t,K+1:K_2}) = E(X_{t,1:K}^i,X_{t,K+1:K_2}, X_{t-1,K_2+1:M}^i) + \sum_{p=K+1}^{K_2} \frac{[X_{t,r,s} - f_r(X_{t-1}^i, X_{t,s}^i)]_p^2}{2\Delta_{p}}$.


\item {\em  Mode Track $X_{t,r,r}$: }  Set $X_{t,K_2+1:M}^i = m_{t,r,r}^{i}$. Here
$m_{t,r,r}^{i}(X_{t-1}^i,X_{t,1:K_2}^i,Y_t) =  \arg \min_{X_{t,K_2+1:M}} L^i(X_{t,K_2+1:M})$ where  $L^i$ is defined in step  \ref{mtxtreismt} of Algorithm \ref{pfeismt}.


\item {\em Weight: }  Compute $w_t^i = \frac{\tilde{w}_t^{i} }{ \sum_{j=1}^N \tilde{w}_t^{j}}$ where  $\tilde{w}_t^{i} = w_{t-1}^{i} \frac{p(Y_t|X_t^{i}) p(X_{t,K+1:M}^{i}|X_{t-1}^i, X_{t,1:K}^i)}{\n(X_{t,K+1:K_2}^{i}; \ m_{t,r,s}^{i}, \ \Sigma_{IS}^{i})}$.


%\item Compute $m_t^i = \arg \min L^i(X_{t,K+1:M})$, $L^i$ is defined in (\ref{defL}) with $\Delta_{r,p}=\Delta_{p+K}$ and $X_{t,s}^i$, $\fr$ defined in steps \ref{defxtsi}, \ref{deffri}.
%%and $X_{t,s}^i = X_{t,1:K}^i$,  $X_{t-1,r}^i = X_{t-1,K+1:M}^i$, $\fr = f_v(X_{t,s}^i,X_{t-1,r}^i)$.
%
%\item Compute $\Sigma_{IS}^i = ( \nabla^2 L^i (m_t^i) )^{-1}$.
%
%\item {\em If PF-EIS, then Efficient Importance Sample $X_{t,K+1:M}$, }  i.e. $X_{t,K+1:M}^i \sim \n( m_t^i, \Sigma_{IS}^i )$.
%%from Gaussian approx to $\pss$,
%
%\item {\em If PF-EIS-MT, then}
%\ben
%\item {\em Efficient Importance Sample $X_{t,K+1:K_2}$, } i.e. $X_{t,K+1:K_2}^i \sim \n( (m_t^i)_{1:K_2-K}, (\Sigma_{IS}^i)_{K-2-K \times K_2-K} )$.
%
%\item {\em Mode Track (MT) $X_{t,K_2 + 1:M}$, } i.e. set $X_{t,K_2 + 1:M}^i = (m_t^i)_{K_2+1:M}$
%\een
%
%\item {\em Weight: } Compute $w_t^i = \frac{\tilde{w}_t^{i} }{ \sum_{j=1}^N \tilde{w}_t^{j}}$ where  $\tilde{w}_t^{i} = w_{t-1}^{i} \frac{p(Y_t|X_t^{i}) p(X_{t,r}^{i}|X_{t-1}^i, X_{t,s}^i)}{\n(X_{t,K+1:M}^{i}; \ m_t^{i}, \ \Sigma_{IS}^{i})}$. % \& resample.
%
%%\item $t \leftarrow t+1$ \& go to step \ref{isxts}.
\een
\end{algorithm*}


%\begin{algorithm*}   %\begin{algorithmic} [1]
%\caption{{\small \bf PF-MT. Going from $\pi_{t-1}^N$ to $\pi_t^N(X_t) = \sum_{i=1}^N \wi \delta(X_{t} - X_{t}^{i})$, \ $X_{t}^{i} = [X_{t,s}^{i},X_{t,r}^{i}]$  }}
%\label{pfmt}
%\ben
%\item
%{\em Importance Sample $X_{t,s}$: } $\forall i$, sample $X_{t,s}^{i} \sim p(X_{t,s}^i|X_{t-1}^i)$.
%\label{isxtsmt}
%
%\item {\em  Mode Track $X_{t,r}$: } $\forall i$, set $X_{t,r}^i = m_t^{i}$. % Here $m_t^i(X_{t-1}^i,X_{t,s}^i,Y_t) =  \arg \min_{X_{t,r}} L^i(X_{t,r})$  where $L^i(X_{t,r}) \defn -\log[ p^{**,i}] = -\log[p(X_{t,r}|X_{t-1}^{i},X_{t,s}^i, Y_t)]$.
%%For model (\ref{sysmod2}), set $v_{t,r}^i = m_t^i$ and $C_t^i=\chat^i+B_rv_{t,r}^i$.)
%\label{mtxtrmt}
%
%\item {\em Weight \& Resample: } Compute $w_t^i = \frac{\tilde{w}_t^{i} }{ \sum_{j=1}^N \tilde{w}_t^{j}}$ where  $\tilde{w}_t^{i} = w_{t-1}^{i} p(Y_t|X_t^{i}) p(X_{t,r}^{i}|X_{t-1}^i, X_{t,s}^i)$ \& resample. $t \leftarrow t+1$, go to step \ref{isxtsmt}.
%\label{weightmt}
%\een
%\end{algorithm*} 

==> pfmt.tex <==



\begin{algorithm*}   %\begin{algorithmic} [1]
\caption{{\small \bf PF-MT (Approximate). Going from $\pi_{n-1}^N$ to $\pi_n^N(X_n) = \sum_{i=1}^N \wi \delta(X_{n} - X_{n}^{i})$, \ $X_{n}^{i} = [C_n^{i}, \rho_n^i, v_{n,s}^{i},v_{n,r}^{i}]$  }}
\label{pfmtapprox}
\ben
\item
{\em Importance Sample (IS) on effective basis: } $\forall i$, sample $v_{n,s}^{i} \sim \n(A_sv_{n-1,s}^{i}, \Sigma_s)$, sample $\rho_n^i \sim \n(A_\rho \rho_{n-1}^i, \Sigma_\rho)$ and compute $\chat^i$ using (\ref{defhatct}).
\item
{\em Mode Tracking (MT) in residual space: } $\forall i$, compute $C_n^{i}$ by starting with $\chat^i$ and running $k$ iterations of Gradient Descent to minimize $E(C_n) \defn -\log[p(Y_n|C_n)]$. In experiments, $k=1$ or $k=2$ suffice.
\label{modetrack}
 \item
{\em Weight \& Resample: } Compute $w_n^{i}$ using (\ref{compweightsapprox}) and resample \cite{tutorial}.
\label{weight}

\een
\end{algorithm*} 

==> pfmttv.tex <==
\begin{algorithm*}   %\begin{algorithmic} [1]
\caption{{\small \bf PF-MT-TV: PF-MT for a Time Varying Effective Basis. Going from $\pi_{n-1}^N$ to $\pi_n^N(X_n)$, \ $X_{n}^{i} = [C_n^{i}, \rho_n^i, v_{n,s}^{i},v_{n,r}^{i}]$  }}
\label{pfmttv}
\ben
\item
 Run  either Algorithm \ref{pfmt} or Algorithm \ref{pfmtapprox}.
 \label{pfmtstep}
\item
{\em Detect Basis Change:} Detect if basis change required. If yes, go to step \ref{changebasis}, else $n \longleftarrow n+1$ and go to step \ref{pfmtstep}.
\label{changedetect}

\item  {\em Change Basis:}
\ben
\item  Compute $K_{new} = L/\alpha_s$ where $L$ is the length of the most likely contour particle.
\item  $\forall i$, reallocate the knots uniformly and evaluate  the new basis $B_{K_{new}}(C_{n}^{(i)}) \defn B_{K_{new},i}$.
\item   $\forall i$, project $v_{n,s}^{i}$ into the new basis:  $v_{n,s}^i \longleftarrow  (B_{K_{new},i}^T B_{K_{new},i})^{-1} B_{K_{new},i}^T B_{i} v_{n,s}^i$.
\item   $\forall i$, set $B_{i} \longleftarrow B_{K_{new},i}$.
\item  $n \longleftarrow n+1$ and go to step \ref{pfmtstep}.
\een
\label{changebasis}
\een
\end{algorithm*}

%
%\item {\bf Change Basis:}
% Compute the new basis dimension $K_{new}$ as discussed in Section \ref{constfmax}. %and the new basis directions $B_{K_{new}}$ (assumes basis does not depend on $C_{n-1}$).
% For $i=1$ to $N$,
%\ben
%\item Compute the new basis $B_{new,i}$ and the old basis $B_{old,i}$ at uniformly spaced locations on the arclength of $C_n^{(i)}$.%=B_{K}(C_n^{(i)})$. % = B_{K_{new}}(C_{n}^{(i)})
%\item Project $v_{n,s}^{(i)}$ into new basis as: $v_{n,s}^{(i)} \longleftarrow (B_{new,i}^T B_{new,i})^{-1} B_{new,i}^T B_{old,i} v_{n,s}^{(i)}$.
%\item Set $K_n \longleftarrow K_{new}$, $B_{n,i} \longleftarrow B_{new,i}$.


==> practical.tex <==
%\section{Choice of Effective Basis}
%\label{choiceK}
%We discuss how to choose $K$ to  ensure that unimodality holds and to ensure that IS-MT assumption holds. We also discuss possible choices of effective basis.
%If it does not, one would sample $X_{t,1}^i$ from its STP and check if Theorem \ref{unimodthm} holds conditioned on $X_{t,1}^i$.
% that is most likely to satisfy unimodality  most of the time. %Some possible heuristics are:
%Note there is a tradeoff between choosing a larger $K$ and  particle efficiency on an average basis. If K larger, particle efficiency is lower under ``good situations" (when previous particle lies in the correct mode). But K=0 or very small will sometime result in all particles falling in the wrong mode resulting in near zero particle efficiency. %In our experiments we realized that anything more than $K=1$ resulted in loss of efficiency.  (and hence $K=\dim(X_{t,s})$)

\section{Practical Issues}
\label{heuristics}

\subsection{Choosing $X_{t,s}$ for Applying PF-EIS}
\label{chooseKunimod}
Theorem \ref{unimodthm} gives a unimodality condition that needs to be verified separately for each particle and each $Y_t$. An exact algorithm to to do this would be to check at each $t$, for each $i$, if Theorem \ref{unimodthm} holds with $K=0$. Keep increasing $K$ and doing this until find a $K$ for which Theorem \ref{unimodthm} holds conditioned on $X_{t,1:K}^i$. This can be done efficiently only if $\Delta^*$ can be computed analytically or using some efficient numerical techniques. That will be the focus of future research.
But, as discussed earlier, PF-EIS or PF-EIS-MT work even if unimodality holds for most particles at most times. We discuss some heuristics based on the result of Theorem \ref{unimodthm} to  choose $X_{t,s}$ a-priori or on-the-fly (but using an inexpensive heuristic).%(Theorem \ref{unimodthm})

\begin{heuristic}
Choose $X_{t,s}$ as the state(s) so that conditioned on $X_{t,s}$, $p^*$ is most likely to be unimodal.
\label{h1}
\end{heuristic}
%
\begin{heuristic}
If OL is multimodal with small probability (implies $p^*$ will multimodal with even smaller probability), then choosing a $K=0$ dim $X_{t,s}$ is usually the best. A simple heuristic is to choose $K>0$ if probability that OL is multimodal is more than 0.5.%very likely to be unimodal
\label{h2}
\end{heuristic}

Heuristic \ref{h1} was used in Example \ref{illumtrack} \cite{kaleicassp}.
We show how these heuristics apply to the temperature tracking problem of Example \ref{temptrack}. Assume that OL is multimodal as a function of temperature at only one node $p_0$ and is unimodal as a function of temperature at all other nodes. For the OL of Example \ref{example1}, this is the most likely scenario since it is highly unlikely that at a given time more than one sensor will fail. We want to choose $X_{t,s}=v_{t,s}$ that makes it most likely for $\pss(v_{t,r})$ to be unimodal. Given $X_{t-1}$ and $v_{t,s}$, $v_{t,r}$ is an affine function of $C_t$. Thus we can equivalently find conditions for unimodality of $\pss(C_{t})$, which is easier to do an approximate analysis of. If we can find an $X_{t,s}=v_{t,s}$ that ensures that $\pss(C_{t,p_0}) \defn p(C_{t,p_0}|Y_{t,p_0},X_{t-1}^i,v_{t,s}^i)$ is unimodal, then $\pss(C_t)$ will also usually be unimodal\footnote{This would be exactly true if $\pss(C_{t,p_0})$ were not just unimodal, but also log-concave (its $-\log$ is convex). This is because $\pss(C_t)$ is $\pss(C_{t,p_0})$ multiplied by two log-concave terms: $p(C_{t}|C_{t,p_0},X_{t-1}^i,v_{t,s}^i)$ (Gaussian) and $\prod_{p \neq p_0} p(Y_{t,p}|C_{t,p})$ (approximately Gaussian since no other sensor fails). $\pss(C_{t,p_0})$ will be log-concave if $\Delta_{C,p_0} = var[p(C_{t,p_0}|X_{t-1}^i,v_{t,s}^i)] < \inf_{\{ C_{t}: \nabla_{C_{t,p_0}}^2 E_{Y_t}(C_t) < 0 \}} \frac{1}{|\nabla_{C_{t,p_0}}^2 E_{Y_t}(C_t)|}$, i.e. it is more likely to be log-concave if $\Delta_{C,p_0}$ is smaller.}.
Now, $\pss(C_{t,p_0}) \propto p(Y_{t,p_0}|C_{t,p_0}) p(C_{t,p_0}|X_{t-1}^i,v_{t,s}^i)$. The $\Delta^*$ required for its unimodality (given in (\ref{suff})) can only be computed on the fly. A-priori, we can only choose the state $v_{t,s}$ so that $\Delta_{C,p_0} \defn var[p(C_{t,p_0}|X_{t-1}^i,v_{t,s}^i)]$ is the smallest (making it most likely that $\Delta_{C,p_0}< \Delta^*$). Now, $\Delta_{C,p_0} = B_{r,p_0} \Delta_{\nu,r} B_{r,p_0}^T$ where $B_{r,p_0}$ is the $p_0^{th}$ row of $(B_r)_{M \times M-K}$. Thus it will be smallest if $v_{t,s}$ is chosen to satisfy
\bea
v_{t,s} = v_{t,j_s}, \ j_s \defn \arg \min_{j_0=1,2,\dots M} \sum_{j \neq j_0} B_{j,p_0}^2 \Delta_{\nu,j}
\label{choosevts}
\eea
This is equivalent to choosing $v_{t,s}$ as the $v_{t,j}$ for which $B_{j,p_0} v_{t,j}$ is most strongly correlated to $C_{t,p_0}$ given $X_{t-1}$, i.e. $j_s = \arg \max_{j} B_{j,p_0}^2 \Delta_{\nu,j}$. The above ideas can be generalized to the following 2 heuristics.
\begin{heuristic}
Consider problems similar to Example \ref{temptrack}.
\ben
\item If it is given that OL is multimodal as a function of a $C_{t,p_0}$, and is unimodal as a function of all $C_{t,p}, p \neq p_0$, choose $v_{t,s}$ as the $v_{t,j}$ that minimizes  $\Delta_{C,p_0} = var[p(C_{t,p_0}|X_{t-1}^i,v_{t,s}^i)]$, i.e. choose $v_{t,s}$ using (\ref{choosevts}).%

\item If $p_0$ is a set of nodes, first fix $K$ (dimension of $v_{t,s}$). Then choose $v_{t,s}$ so that the maximum eigenvalue of $\Delta_{C,p_0} = B_{r,p_0} \Delta_{\nu,r} B_{r,p_0}^T$ (which now is a square matrix of size equal to number of nodes in $p_0$) is the smallest.
\een
\label{hsens1}
\end{heuristic}
\begin{heuristic}
Choose node(s) $p_0$ using one of the following:%for Heuristic \ref{hsens1}
\ben
\item It may be known a-priori that OL is most likely to be multimodal as a function of temperature at sensor node(s) $p_0$. We then apply Heuristic \ref{hsens1} to choose $v_{t,s}$ with this choice of $p_0$. For e.g. in case of Example \ref{example1}, this will be true if sensors at some node(s) are much more likely to fail (may be older) than those at other nodes. Alternatively, if some node(s) have a squared temperature sensor, i.e. $h_p(C_{t,p}) = C_{t,p}^2$ for $p=p_0$ (or $h(C_{t})$ is any other many-to-one function), they will often have a multimodal OL.
\label{aprior}

\item If OL is equally likely to be multimodal as a function of any $C_{t,p}$ (e.g. if all sensors have equal failure probability), then $p_0 = [1,2 \dots M]$ and so $\Delta_{C,p_0} = B_r \Delta_{\nu,r} B_r^T$, i.e. its eigenvalues are $\Delta_{\nu,r,p}$. Thus given $K$, we use as $v_{t,s}$, the $v_{t,j}$ with the top $K$ values of $\Delta_{\nu,j}$.%
\label{equal} %. Applying Heuristic \ref{hsens1},  = B_{r,p_0} \Delta_{\nu,r} B_{r,p_0}^T

\item Choose $v_{t,s}$ on-the-fly by using the current observation $Y_t$ to figure out the most likely multimodal nodes at $t$. For e.g., for Example \ref{example1}, at each $t$, the larger the value of $(Y_{t,p}^{(1)}-Y_{t,p}^{(2)})^2/\sigma_{obs,p}^2$, the more likely it is that OL is multimodal as a function of $C_{t,p}$. If this value is largest for $p=p_0$, then choose $v_{t,s}$ using (\ref{choosevts}) for this $p_0$. If no value is above a threshold, then use $K=0$ at that $t$. The complexity of this heuristic is only $M \log_2 M$ for $M$ nodes.%Use a simple heuristic to
%look at the observation pairs at a node to decide which pair is most likely to result in multimodal OL.
 \label{onfly}
\een
\label{hsens2}
\end{heuristic}
%If all sensor nodes have sensors with equal failure probabilities, choose as effective basis the eigen-coefficient with maximum STP variance, i.e. choose $j_s = \arg \max_j \Delta_{\nu,j}$.

We show an example now. Consider Example \ref{example1} with $\alpha^{(1)} = \alpha^{(2)} = [0.4,0.01,0.01]$, $\Sigma_\nu = diag([10,5,5])$, $B= [0.95, 0.21, 0.21]'; [-0.21,0.98,-0.05]'; [-0.22, 0, 0.98]'$ (using MATLAB notation). Thus, at least one sensor at node $p_0=1$ fails  with probability $0.4+0.4-0.16=0.64$, i.e. OL is multimodal as a function of $C_{t,1}$ with roughly this probability. Since the probability of OL multimodality is more than 0.5, by Heuristic \ref{h2}, we choose $K>0$. Also, by Heuristic \ref{hsens2}, we choose $p_0=1$ (OL is multimodal as a function of either $C_{t,2}$ or $C_{t,3}$ with very small probability). By Heuristic \ref{hsens1}, $v_{t,s}$ satisfying (\ref{choosevts}) for $p_0=1$ is $v_{t,1}$.%

When the state can be treated as a spatial signal, e.g. contour deformation, the above heuristics can be modified as follows.
\begin{heuristic}
If the state is spatially stationary and OL is equally likely to be multimodal as a function of any $C_{t,p}$, Heuristic \ref{hsens2}.\ref{equal} may be modified as follows. Replace the eigen-basis used to diagonalize $\Sigma_n$ by a Fourier basis, or any other  data-independent basis\footnote{More efficient when system model changes with time or when $M$ is time-varying as in \cite{cdc06}.}. If Fourier basis is used, Power Spectral Density (PSD) replaces eigenvalues. Thus by Heuristic \ref{hsens2}.\ref{equal}, we use the $K$ frequencies (of an $M$ length PSD) with highest PSD values as the effective basis. If these are the $K$ lowest frequencies, one can also equivalently spatially subsample the state to $K$ points to choose effective basis. This heuristic can be further refined using Heuristic \ref{hsens2}.\ref{aprior} or \ref{hsens2}.\ref{onfly}, for e.g. sample more finely in regions which are more likely to be multimodal.%
\label{hcont}
\end{heuristic}

In contour tracking, if in most cases, multiple OL modes are separated only by translation/scale, it suffices to use only these as $X_{t,s}$ \cite{cvpr05}. This happens when multimodality is due to non-overlapping clutter.
Heuristic \ref{hcont} was used in \cite{cdc06} for problems when OL modes are frequently separated by local deformation (e.g. due to overlapping clutter or partial occlusions) and it is impossible to decide which regions are more likely to have multiple modes\footnote{Since deformation is spatially stationary and also periodic (i.e. its covariance matrix is circulant), the PSD is actually equal to the eigenvalues.}. Similarly, if there are a very large number of sensor nodes and sensors,  all having the same failure probabilities, one can use temperature change at a subsampled set of node locations as the effective basis.
%
%
%For spatially Markov data, e.g. temperature change, DCT may be closer to its eigenvectors.  based on the form of the OL  for contour tracking
%spatially subsample the state to choose an effective basis. This is useful when it is not possible to infer anything about where the modes of OL are likely to lie. %If it is, then that can be used in a more intelligent way to use a smaller effective basis dimension for EIS.
% for e.g. contour deformation in case of contour tracking,
% or low contrast images  or due to overlapping clutter whose contour is separated from the true object by scale



\subsection{Choosing $X_{t,r,r}$ for Applying PF-EIS-MT/PF-MT}  % instead of (\ref{Sigrrbnd})
\label{chooseKismt}
We first choose an $X_{t,s}, X_{t,r}$ for the EIS step using the unimodality heuristics discussed above. Then we split $X_{t,r}$ into $X_{t,r,s}$ and $X_{t,r,r}$ so that $X_{t,r,r}$ satisfies the IS-MT assumption. Then  PF-EIS-MT can be implemented with the chosen $X_{t,s}, X_{t,r,s}, X_{t,r,r}$. Alternatively, one can implement PF-MT (faster) with $\tilde{X}_{t,s} =[X_{t,s}; X_{t,r,s}]$, $\tilde{X}_{t,r} = X_{t,r,r}$.
For a given value of $\eps, \eps_2$, two approaches can be used to choose $X_{t,r,r}$ based on the analysis of Sec. \ref{ismtanal}. The first uses (\ref{Sigrrbnd}) and the second does an approximate analysis of (\ref{SigISbnd}).%
\begin{heuristic}
 Begin with $M_{r,r} = M_r$ and keep reducing its value. For each value of $M_{r,r}$, choose the states with the $M_{r,r}$ smallest values of $\Delta_{\nu,r,p}$ (so that $\max_p \Delta_{\nu,r,r,p}$ is smallest) as $X_{t,r,r}$. With this choice, compute the bound of (\ref{Sigrrbnd}) and check if it is smaller than $\eps_2$. If it is smaller, then stop, else reduce $M_{r,r}$ by 1 and repeat the same steps.
\label{hSigrr}
\end{heuristic}
Alternatively, the same thing can be done but by using inequality (\ref{SigISbnd}). %Note that (\ref{SigISbnd}) also holds if expected value is taken on both sides. Let $\E[.]$ denote $\E_{X_t}[.]$. Using a first order approximation, $\E[\Sigma_{IS,r,r}^i] \approx ( \E[ \nabla_{X_{t,r,r}}^2 E_{Y_t} ] + \Delta_{\nu,r,r}^{-1} )^{-1}$.
%$\E_{X_{1:t,s}^i,X_{1:t,r,s}^i,Y_{1:t} }[.]$.
%For given $M_{r,r}$, choose the set of states for which the largest eigenvalue of this term is smallest as $X_{t,r,r}$. Thus,
\begin{heuristic}
Consider an observation model of the form $Y_t = h_a(X_{t,a}) h_b(X_{t,b}) + w_t$ (some examples are bearings-only tracking\cite{gordon} or Example \ref{illumtrack}). Let $X_{t,s} = X_{t,a}$. If $w_t$ is white Gaussian, $\nabla^2_{X_{t,r}} E_{Y_t} = \nabla^2_{X_{t,b}} E_{Y_t} = \sum_{k=1}^P [ h_{a,k}(X_{t,s}^i)^2  \nabla h_{b,k}(m_{t}^i)  \nabla h_{b,k}(m_{t}^i)^T - \nabla^2 h_{b,k}(m_{t}^i) (Y_{t,k} - h_{a,k}(X_{t,s}^i) h_{b,k}(m_{t}^i) ) ]/\sigma_{obs,k}^2$ where $P=\dim(Y_t)$. Choose $X_{t,r,r}$ on-the-fly by applying Heuristic \ref{hSigrr} but with $\Delta_{\nu,r,p}$ replaced by the $p^{th}$ eigenvalue of  $(\nabla^2 E_{Y_t} + \Delta_{\nu,r}^{-1} )^{-1}$. To choose $X_{t,r,r}$ a-priori, can replace $\nabla^2 E_{Y_t}$ by its expected value. If $w_t$ is not Gaussian, modify $E_{Y_t}$ and its Hessian appropriately.%
\label{hSigIS}
 \end{heuristic}
Heuristic \ref{hSigIS},  along with Heuristic \ref{h1}, explains the choice of $X_{t,r,r} = X_{t,r} =\lambda_t$ in Example \ref{illumtrack} \cite{kaleicassp}. %It can be shown that $\nabla^2_{X_{t,r}} E_{Y_t}$ has much larger values if $X_{t,r}=\lambda_t$ than if $X_{t,r}=u_t$.

%
%
%Then apply Heuristic \ref{hSigrr} but with $\Delta_{\nu,r,p}$ replaced by the $p^{th}$ eigenvalue of  $( \E[\nabla^2 E_{Y_t}] + \Delta_{\nu,r}^{-1} )^{-1}$. We do an average case analysis to choose $X_{t,r,r}$ a-priori. Alternatively, this can be done on the fly by using eigenvalues of $(\nabla^2 E_{Y_t} + \Delta_{\nu,r}^{-1} )^{-1}$.%
%the dominant term of $\E[\nabla_{X_{t,r}}^2 E_{Y_t}]$ is $\E[\pdif{h}{X_{t,r}}(X_t)^T \pdif{h}{X_{t,r}}(X_t)] \defn Q$. Choose those states which have largest diagonal entries\footnote{For a symmetric matrix, largest eigenvalue is $\ge$ all diagonal entries.} in $Q + \Delta_{\nu,r}^{-1}$ as $X_{t,r,r}$.%(larger diagonal entries of $\E[\pdif{h}{X_{t,r}}^T \pdif{h}{X_{t,r}}]$ and smaller entries of $\Delta_{\nu,r}$). A simple heuristic is to

%heuristic, along with Heuristic \ref{h1} was used in choosing the illumination states as $X_{t,r,r} =X_{t,r}$ in \cite{kaleicassp} (Example \ref{illumtrack}). If $X_{t,r,r} = \lambda_t$ then the $p^{th}$ diagonal entry of $Q$ would be $\sum_{i,j} ( P_{\lambda,p}(i,j) T_0( u_{t,3}(i-u_{t,1}), u_{t,3}(i-u_{t,2}) ) )^2 + \Delta_{\lambda,p}^{-1}$. If $X_{t,r,r} =  u_t$ were used, then the first diagonal entry of $Q$ will have the form $\sum_{i,j}  ( P_{\lambda}(i,j) \lambda_t u_{t,3} \pdif{T_0}{x}( u_{t,3}(i-u_{t,1}), u_{t,3}(i-u_{t,2}) ) )^2   + \Delta_{u,1}^{-1} $ and the other two entries will also have similar order. Now for most pixels of most images, the illumination component times the x gradient of template intensity  will be much smaller than the actual template intensity. Illumination is usually less than 1 or 2, magnitude of x gradient of template is usually less than 5 or 6, while the template intensity varies between 0 and 255 (if image is histogram equalized then it varies uniformly in this range). Thus $Q$ will be much smaller in the second case than in the first. Also the variance of motion over time is smaller than that for illumination.  Thus both terms in the second case will be much smaller than in the first case. Thus, the first case was chosen.% (any histogram equalized image (usually less than 4-5) (lies between 0 to 255) , and thus the sum taken over all pixels will also be much smaller illumination ($\Delta_{\lambda,p}$) is smaller than that of motion.








==> practicalismt.tex <==
\subsection{Choosing $X_{t,r,r}$ for Applying PF-EIS-MT/PF-MT}  % instead of (\ref{Sigrrbnd})
\label{chooseKismt}
We first choose an $X_{t,s}, X_{t,r}$ for the EIS step using the unimodality heuristics discussed above. Then we split $X_{t,r}$ into $X_{t,r,s}$ and $X_{t,r,r}$ so that $X_{t,r,r}$ satisfies the IS-MT assumption. Then  PF-EIS-MT can be implemented with the chosen $X_{t,s}, X_{t,r,s}, X_{t,r,r}$. Alternatively, one can implement PF-MT (faster) with $\tilde{X}_{t,s} =[X_{t,s}; X_{t,r,s}]$, $\tilde{X}_{t,r} = X_{t,r,r}$.
For a given value of $\eps, \eps_2$, two approaches can be used to choose $X_{t,r,r}$ based on the analysis of Sec. \ref{ismtanal}. The first uses (\ref{Sigrrbnd}) and the second does an approximate analysis of (\ref{SigISbnd}).%
\begin{heuristic}
 Begin with $M_{r,r} = M_r$ and keep reducing its value. For each value of $M_{r,r}$, choose the states with the $M_{r,r}$ smallest values of $\Delta_{\nu,r,p}$ (so that $\max_p \Delta_{\nu,r,r,p}$ is smallest) as $X_{t,r,r}$. With this choice, compute the bound of (\ref{Sigrrbnd}) and check if it is smaller than $\eps_2$. If it is smaller, then stop, else reduce $M_{r,r}$ by 1 and repeat the same steps.
\label{hSigrr}
\end{heuristic}
Alternatively, the same thing can be done but by using inequality (\ref{SigISbnd}). %Note that (\ref{SigISbnd}) also holds if expected value is taken on both sides. Let $\E[.]$ denote $\E_{X_t}[.]$. Using a first order approximation, $\E[\Sigma_{IS,r,r}^i] \approx ( \E[ \nabla_{X_{t,r,r}}^2 E_{Y_t} ] + \Delta_{\nu,r,r}^{-1} )^{-1}$.
%$\E_{X_{1:t,s}^i,X_{1:t,r,s}^i,Y_{1:t} }[.]$.
%For given $M_{r,r}$, choose the set of states for which the largest eigenvalue of this term is smallest as $X_{t,r,r}$. Thus,
\begin{heuristic}
Consider an observation model of the form $Y_t = h_a(X_{t,a}) h_b(X_{t,b}) + w_t$ (some examples are bearings-only tracking\cite{gordon} or Example \ref{illumtrack}). Let $X_{t,s} = X_{t,a}$. If $w_t$ is white Gaussian, $\nabla^2_{X_{t,r}} E_{Y_t} = \nabla^2_{X_{t,b}} E_{Y_t} = \sum_{k=1}^P [ h_{a,k}(X_{t,s}^i)^2  \nabla h_{b,k}(m_{t}^i)  \nabla h_{b,k}(m_{t}^i)^T - \nabla^2 h_{b,k}(m_{t}^i) (Y_{t,k} - h_{a,k}(X_{t,s}^i) h_{b,k}(m_{t}^i) ) ]/\sigma_{obs,k}^2$ where $P=\dim(Y_t)$. Choose $X_{t,r,r}$ on-the-fly by applying Heuristic \ref{hSigrr} but with $\Delta_{\nu,r,p}$ replaced by the $p^{th}$ eigenvalue of  $(\nabla^2 E_{Y_t} + \Delta_{\nu,r}^{-1} )^{-1}$. To choose $X_{t,r,r}$ a-priori, can replace $\nabla^2 E_{Y_t}$ by its expected value. If $w_t$ is not Gaussian, modify $E_{Y_t}$ and its Hessian appropriately.%
\label{hSigIS}
 \end{heuristic}
Heuristic \ref{hSigIS},  along with Heuristic \ref{h1}, explains the choice of $X_{t,r,r} = X_{t,r} =\lambda_t$ in Example \ref{illumtrack} \cite{kaleicassp}. %It can be shown that $\nabla^2_{X_{t,r}} E_{Y_t}$ has much larger values if $X_{t,r}=\lambda_t$ than if $X_{t,r}=u_t$.

%
%
%Then apply Heuristic \ref{hSigrr} but with $\Delta_{\nu,r,p}$ replaced by the $p^{th}$ eigenvalue of  $( \E[\nabla^2 E_{Y_t}] + \Delta_{\nu,r}^{-1} )^{-1}$. We do an average case analysis to choose $X_{t,r,r}$ a-priori. Alternatively, this can be done on the fly by using eigenvalues of $(\nabla^2 E_{Y_t} + \Delta_{\nu,r}^{-1} )^{-1}$.%
%the dominant term of $\E[\nabla_{X_{t,r}}^2 E_{Y_t}]$ is $\E[\pdif{h}{X_{t,r}}(X_t)^T \pdif{h}{X_{t,r}}(X_t)] \defn Q$. Choose those states which have largest diagonal entries\footnote{For a symmetric matrix, largest eigenvalue is $\ge$ all diagonal entries.} in $Q + \Delta_{\nu,r}^{-1}$ as $X_{t,r,r}$.%(larger diagonal entries of $\E[\pdif{h}{X_{t,r}}^T \pdif{h}{X_{t,r}}]$ and smaller entries of $\Delta_{\nu,r}$). A simple heuristic is to

%heuristic, along with Heuristic \ref{h1} was used in choosing the illumination states as $X_{t,r,r} =X_{t,r}$ in \cite{kaleicassp} (Example \ref{illumtrack}). If $X_{t,r,r} = \lambda_t$ then the $p^{th}$ diagonal entry of $Q$ would be $\sum_{i,j} ( P_{\lambda,p}(i,j) T_0( u_{t,3}(i-u_{t,1}), u_{t,3}(i-u_{t,2}) ) )^2 + \Delta_{\lambda,p}^{-1}$. If $X_{t,r,r} =  u_t$ were used, then the first diagonal entry of $Q$ will have the form $\sum_{i,j}  ( P_{\lambda}(i,j) \lambda_t u_{t,3} \pdif{T_0}{x}( u_{t,3}(i-u_{t,1}), u_{t,3}(i-u_{t,2}) ) )^2   + \Delta_{u,1}^{-1} $ and the other two entries will also have similar order. Now for most pixels of most images, the illumination component times the x gradient of template intensity  will be much smaller than the actual template intensity. Illumination is usually less than 1 or 2, magnitude of x gradient of template is usually less than 5 or 6, while the template intensity varies between 0 and 255 (if image is histogram equalized then it varies uniformly in this range). Thus $Q$ will be much smaller in the second case than in the first. Also the variance of motion over time is smaller than that for illumination.  Thus both terms in the second case will be much smaller than in the first case. Thus, the first case was chosen.% (any histogram equalized image (usually less than 4-5) (lies between 0 to 255) , and thus the sum taken over all pixels will also be much smaller illumination ($\Delta_{\lambda,p}$) is smaller than that of motion.





==> practicalunimod.tex <==
%\section{Choice of Effective Basis}
%\label{choiceK}
%We discuss how to choose $K$ to  ensure that unimodality holds and to ensure that IS-MT assumption holds. We also discuss possible choices of effective basis.
%If it does not, one would sample $X_{t,1}^i$ from its STP and check if Theorem \ref{unimodthm} holds conditioned on $X_{t,1}^i$.
% that is most likely to satisfy unimodality  most of the time. %Some possible heuristics are:
%Note there is a tradeoff between choosing a larger $K$ and  particle efficiency on an average basis. If K larger, particle efficiency is lower under ``good situations" (when previous particle lies in the correct mode). But K=0 or very small will sometime result in all particles falling in the wrong mode resulting in near zero particle efficiency. %In our experiments we realized that anything more than $K=1$ resulted in loss of efficiency.  (and hence $K=\dim(X_{t,s})$)

%\section{Practical Issues}
%\label{heuristics}

\subsection{Heuristics to Choose the Effective Basis}
\label{chooseKunimod}

Theorem \ref{unimodthm} gives a unimodality condition that needs to be verified separately for each particle and each $Y_t$. An exact algorithm to to do this would be to check at each $t$, for each $i$, if Theorem \ref{unimodthm} holds with $K=0$. Keep increasing $K$ and doing this until find a $K$ for which Theorem \ref{unimodthm} holds conditioned on $X_{t,1:K}^i$. This can be done efficiently only if $\Delta^*$ can be computed analytically or using some efficient numerical techniques. That will be the focus of future research.
But, as discussed earlier, PF-EIS works even if unimodality holds with high probability. We discuss some heuristics based on Theorem \ref{unimodthm} to  choose $X_{t,s}$ a-priori or on-the-fly (but using an inexpensive heuristic) to ensure this.%(Theorem \ref{unimodthm}) for most particles at most times

\begin{heuristic}
Choose $X_{t,s}$ as the state(s) so that conditioned on $X_{t,s}$, $p^*$ is most likely to be unimodal.
\label{h1}
\end{heuristic}
%
\begin{heuristic}
If OL is multimodal with small probability (implies $p^*$ will multimodal with even smaller probability), then choosing a $K=0$ dim $X_{t,s}$ is usually the best. A simple heuristic is to choose $K>0$ if probability that OL is multimodal is more than 0.5.%very likely to be unimodal
\label{h2}
\end{heuristic}

Heuristic \ref{h1} was used in Example \ref{illumtrack} \cite{kaleicassp}.
We show how these heuristics apply to the temperature tracking problem of Example \ref{temptrack}. Assume that OL is multimodal as a function of temperature at only one node $p_0$ and is unimodal as a function of temperature at all other nodes. For the OL of Example \ref{example1}, this is the most likely scenario since it is highly unlikely that at a given time more than one sensor will fail. We want to choose $X_{t,s}=v_{t,s}$ that makes it most likely for $\pss(v_{t,r})$ to be unimodal. Given $X_{t-1}$ and $v_{t,s}$, $v_{t,r}$ is an affine function of $C_t$. Thus we can equivalently find conditions for unimodality of $\pss(C_{t})$, which is easier to do an approximate analysis of. If we can find an $X_{t,s}=v_{t,s}$ that ensures that $\pss(C_{t,p_0}) \defn p(C_{t,p_0}|Y_{t,p_0},X_{t-1}^i,v_{t,s}^i)$ is unimodal, then $\pss(C_t)$ will also usually be unimodal\footnote{This would be exactly true if $\pss(C_{t,p_0})$ were not just unimodal, but also log-concave (its $-\log$ is convex). This is because $\pss(C_t)$ is $\pss(C_{t,p_0})$ multiplied by two log-concave terms: $p(C_{t}|C_{t,p_0},X_{t-1}^i,v_{t,s}^i)$ (Gaussian) and $\prod_{p \neq p_0} p(Y_{t,p}|C_{t,p})$ (approximately Gaussian since no other sensor fails). $\pss(C_{t,p_0})$ will be log-concave if $\Delta_{C,p_0} = var[p(C_{t,p_0}|X_{t-1}^i,v_{t,s}^i)] < \inf_{\{ C_{t}: \nabla_{C_{t,p_0}}^2 E_{Y_t}(C_t) < 0 \}} \frac{1}{|\nabla_{C_{t,p_0}}^2 E_{Y_t}(C_t)|}$, i.e. it is more likely to be log-concave if $\Delta_{C,p_0}$ is smaller.}.
Now, $\pss(C_{t,p_0}) \propto p(Y_{t,p_0}|C_{t,p_0}) p(C_{t,p_0}|X_{t-1}^i,v_{t,s}^i)$. The $\Delta^*$ required for its unimodality (given in (\ref{suff})) can only be computed on the fly. A-priori, we can only choose the state $v_{t,s}$ so that $\Delta_{C,p_0} \defn var[p(C_{t,p_0}|X_{t-1}^i,v_{t,s}^i)]$ is the smallest (making it most likely that $\Delta_{C,p_0}< \Delta^*$). Now, $\Delta_{C,p_0} = B_{r,p_0} \Delta_{\nu,r} B_{r,p_0}^T$ where $B_{r,p_0}$ is the $p_0^{th}$ row of $(B_r)_{M \times M-K}$. Thus it will be smallest if $v_{t,s}$ is chosen to satisfy
\bea
v_{t,s} = v_{t,j_s}, \ j_s \defn \arg \min_{j_0=1,2,\dots M} \sum_{j \neq j_0} B_{j,p_0}^2 \Delta_{\nu,j}
\label{choosevts}
\eea
This is equivalent to choosing $v_{t,s}$ as the $v_{t,j}$ for which $B_{j,p_0} v_{t,j}$ is most strongly correlated to $C_{t,p_0}$ given $X_{t-1}$, i.e. $j_s = \arg \max_{j} B_{j,p_0}^2 \Delta_{\nu,j}$. The above ideas can be generalized to the following 2 heuristics.
\begin{heuristic}
Consider problems similar to Example \ref{temptrack}.
\ben
\item If it is given that OL is multimodal as a function of a $C_{t,p_0}$, and is unimodal as a function of all $C_{t,p}, p \neq p_0$, choose $v_{t,s}$ as the $v_{t,j}$ that minimizes  $\Delta_{C,p_0} = var[p(C_{t,p_0}|X_{t-1}^i,v_{t,s}^i)]$, i.e. choose $v_{t,s}$ using (\ref{choosevts}).%

\item If $p_0$ is a set of nodes, first fix $K$ (dimension of $v_{t,s}$). Then choose $v_{t,s}$ so that the maximum eigenvalue of $\Delta_{C,p_0} = B_{r,p_0} \Delta_{\nu,r} B_{r,p_0}^T$ (which now is a square matrix of size equal to number of nodes in $p_0$) is the smallest.
\een
\label{hsens1}
\end{heuristic}
\begin{heuristic}
Choose node(s) $p_0$ using one of the following:%for Heuristic \ref{hsens1}
\ben
\item It may be known a-priori that OL is most likely to be multimodal as a function of temperature at sensor node(s) $p_0$. We then apply Heuristic \ref{hsens1} to choose $v_{t,s}$ with this choice of $p_0$. For e.g. in case of Example \ref{example1}, this will be true if sensors at some node(s) are much more likely to fail (may be older) than those at other nodes. Alternatively, if some node(s) have a squared temperature sensor, i.e. $h_p(C_{t,p}) = C_{t,p}^2$ for $p=p_0$ (or $h(C_{t})$ is any other many-to-one function), they will often have a multimodal OL.
\label{aprior}

\item If OL is equally likely to be multimodal as a function of any $C_{t,p}$ (e.g. if all sensors have equal failure probability), then $p_0 = [1,2 \dots M]$ and so $\Delta_{C,p_0} = B_r \Delta_{\nu,r} B_r^T$, i.e. its eigenvalues are $\Delta_{\nu,r,p}$. Thus given $K$, we use as $v_{t,s}$, the $v_{t,j}$ with the top $K$ values of $\Delta_{\nu,j}$.%
\label{equal} %. Applying Heuristic \ref{hsens1},  = B_{r,p_0} \Delta_{\nu,r} B_{r,p_0}^T

\item Choose $v_{t,s}$ on-the-fly by using the current observation $Y_t$ to figure out the most likely multimodal nodes at $t$. For e.g., for Example \ref{example1}, at each $t$, the larger the value of $(Y_{t,p}^{(1)}-Y_{t,p}^{(2)})^2/\sigma_{obs,p}^2$, the more likely it is that OL is multimodal as a function of $C_{t,p}$. If this value is largest for $p=p_0$, then choose $v_{t,s}$ using (\ref{choosevts}) for this $p_0$. If no value is above a threshold, then use $K=0$ at that $t$. The complexity of this heuristic is only $M \log_2 M$ for $M$ nodes.%Use a simple heuristic to
%look at the observation pairs at a node to decide which pair is most likely to result in multimodal OL.
 \label{onfly}
\een
\label{hsens2}
\end{heuristic}
%If all sensor nodes have sensors with equal failure probabilities, choose as effective basis the eigen-coefficient with maximum STP variance, i.e. choose $j_s = \arg \max_j \Delta_{\nu,j}$.

We show an example now. Consider Example \ref{example1} with $\alpha^{(1)} = \alpha^{(2)} = [0.4,0.01,0.01]$, $\Sigma_\nu = diag([10,5,5])$, $B= [0.95, 0.21, 0.21]'; [-0.21,0.98,-0.05]'; [-0.22, 0, 0.98]'$ (using MATLAB notation). Thus, at least one sensor at node $p_0=1$ fails  with probability $0.4+0.4-0.16=0.64$, i.e. OL is multimodal as a function of $C_{t,1}$ with roughly this probability. Since the probability of OL multimodality is more than 0.5, by Heuristic \ref{h2}, we choose $K>0$. Also, by Heuristic \ref{hsens2}, we choose $p_0=1$ (OL is multimodal as a function of either $C_{t,2}$ or $C_{t,3}$ with very small probability). By Heuristic \ref{hsens1}, $v_{t,s}$ satisfying (\ref{choosevts}) for $p_0=1$ is $v_{t,1}$.%

When the state can be treated as a spatial signal, e.g. contour deformation, the above heuristics can be modified as follows.
\begin{heuristic}
If the state is spatially stationary and OL is equally likely to be multimodal as a function of any $C_{t,p}$, Heuristic \ref{hsens2}.\ref{equal} may be modified as follows. Replace the eigen-basis used to diagonalize $\Sigma_n$ by a Fourier basis, or any other  data-independent basis\footnote{More efficient when system model changes with time or when $M$ is time-varying as in \cite{cdc06}.}. If Fourier basis is used, Power Spectral Density (PSD) replaces eigenvalues. Thus by Heuristic \ref{hsens2}.\ref{equal}, we use the $K$ frequencies (of an $M$ length PSD) with highest PSD values as the effective basis. If these are the $K$ lowest frequencies, one can also equivalently spatially subsample the state to $K$ points to choose effective basis. This heuristic can be further refined using Heuristic \ref{hsens2}.\ref{aprior} or \ref{hsens2}.\ref{onfly}, for e.g. sample more finely in regions which are more likely to be multimodal.%
\label{hcont}
\end{heuristic}

In contour tracking, if in most cases, multiple OL modes are separated only by translation/scale, it suffices to use only these as $X_{t,s}$ \cite{cvpr05}. This happens when multimodality is due to non-overlapping clutter.
Heuristic \ref{hcont} was used in \cite{cdc06} for problems when OL modes are frequently separated by local deformation (e.g. due to overlapping clutter or partial occlusions) and it is impossible to decide which regions are more likely to have multiple modes\footnote{Since deformation is spatially stationary and also periodic (i.e. its covariance matrix is circulant), the PSD is actually equal to the eigenvalues.}. Similarly, if there are a very large number of sensor nodes and sensors,  all having the same failure probabilities, one can use temperature change at a subsampled set of node locations as the effective basis.
%
%
%For spatially Markov data, e.g. temperature change, DCT may be closer to its eigenvectors.  based on the form of the OL  for contour tracking
%spatially subsample the state to choose an effective basis. This is useful when it is not possible to infer anything about where the modes of OL are likely to lie. %If it is, then that can be used in a more intelligent way to use a smaller effective basis dimension for EIS.
% for e.g. contour deformation in case of contour tracking,
% or low contrast images  or due to overlapping clutter whose contour is separated from the true object by scale





==> proof_ismt.tex <==
{\bf Proof: } %Theorem \ref{ismtthm}
From  (\ref{defsigis}) and (\ref{defL}), we have
\beq
(\Sigma_{IS}^i)^{-1} = (\nabla_{v_{t,r}}^2 L^i) (m_t^i) = (\nabla_{v_{t,r}}^2 E) (\chat^i+B_r m_t^i) + \Sigma_r^{-1} \ \ \
\eeq
By Theorem \ref{unimodthm}, $m_t^i$ is the unique minimizer of $L^i$. Also, as explained in the proof of Theorem \ref{unimodthm}, $m_t^i$ lies inside $\R_{K,LC}$ and inside $\R_{K,LC}$, $E$ is convex, i.e. $(\nabla_{v_{t,r}}^2 E) (\chat^i+B_r m_t^i) \ge 0$. Thus $(\Sigma_{IS}^i)^{-1} \ge \Sigma_r^{-1}$ or equivalently $\Sigma_{IS}^i \le \Sigma_r$. This implies that
\bea
\trace(\Sigma_{IS}^i) \le \trace(\Sigma_r)
\label{smaller}
\eea
Note that $m_{t}^i$ is a function of $v_{t-1,r}^i, C_{t-1}^i, v_{t,s}^i, Y_t$. %$\Sigma_{IS}^i$ is a function of $\Sigma_r$.
For any given values of $v_{t-1,r}^i, C_{t-1}^i, v_{t,s}^i, Y_t$, we have that
\bea
\ds
Pr(||v_{t,r}^{i} - m_t^{i}|| > \eps)   \sle  \sum_{p=1}^{M-K} Pr([v_{t,r}^{i} - m_t^{i}]_p^2> \frac{\eps^2}{M-K} ) \nn \\
\sle \sum_{p=1}^{M-K} \frac{(\Sigma_{IS}^i)_{p,p} }{\eps^2/(M-K)} = \frac{\trace(\Sigma_{IS}^i)}{\eps^2/(M-K)} \nn \\
\sle \frac{\trace(\Sigma_r)(M-K)}{\eps^2} \defn \frac{\Delta_{K,tot}(M-K)}{\eps^2} \nn % \frac{\sum_{p=1}^{M-K} \Delta_{p+K}(M-K)}{\eps^2} =
\label{convinprob}
\eea
The first inequality follows since $\{v_{t,r}^i: ||v_{t,r}^{i} - m_t^{i}||^2 > \eps^2 \} \subseteq \{v_{t,r}^i: \mbox{there exists at least one p for which $[v_{t,r}^{i} - m_t^{i}]_p^2 >  \eps^2/(M-K)$} \}$ and applying the union bound on the probability of this event.
The second inequality follows by applying Markov's inequality to $[v_{t,r}^{i} - m_t^{i}]_p)^2$.
The third inequality holds because of (\ref{smaller}).

%From (\ref{convinprob}),
Thus, for every $\eps>0$, we can find a $\delta_\eps = \eps^3/(M-K)$ s.t. if $\Delta_{K,tot} < \delta_\eps$, then $Pr(||v_{t,r}^{i} - m_t^{i}|| > \eps)  < \eps$. This holds for any  given values of $v_{t-1,r}^i, C_{t-1}^i, v_{t,s}^i, Y_t$. Thus the theorem follows.
\\



==> proof_unimod.tex <==
{\bf Proof: } %Theorem \ref{unimodthm}
We need a set of conditions that ensure that $L^i$ has a unique minimizer.%??
The second term in (\ref{defL}) is strongly convex everywhere. Consider the region $\R_{LC}$. Condition \ref{close} ensures that $\R_{LC}$ exists. By its definition, $E(C)$ as a function of $C$ is convex in  $\R_{LC}$. By condition \ref{twicediff}, this implies that the Hessian $\nabla_C^2 E \ge 0$ in $\R_{K,LC}$, which in turn implies that $\nabla_{v_{t,r}}^2 E = B_r^T [\nabla_C^2 E] B_r \ge 0$  in $\R_{K,LC}$. Thus in $\R_{K,LC}$, $L^i(v_{t,r})$ is strongly convex, i.e. it has a unique minimizer. We need to show that outside $\R_{K,LC}$, i.e. in $\R_{K,LC}^c$, $L^i$ has no minimizers. {\em A sufficient condition for this is that $\nabla_{v_{t,r}} L \neq 0$, $\forall v_{t,r} \in \R_{K,LC}^c$.}

%is bounded above zero\footnote{$\exists \eps > 0$, s.t. $\forall C \in \R_{LC}, C^T [\nabla_C^2 E](C) C > \eps$}.
%Thus, in $\R_{K,LC}$, $\nabla_{v_{t,r}}^2 E = B_r^T [\nabla_C^2 E] B_r$ is also $\ge 0$. Thus in $\R_{K,LC}$, $L^i$ is strongly convex, i.e. it has a unique minimizer.
%bounded above zero, i.e. $E$ is strongly convex as a function $v_{t,r}$. Thus in $\R_{K,LC}$, $L^i$ is strongly convex, i.e. it has a unique minimizer.


Let $T_2$ denotes the second term of (\ref{defL}). Now, $\nabla L = \nabla E + \nabla T_2$ can be zero only in regions of  $\R_{K,LC}^c$ where,  for all $p$,  $[\nabla E]_p$ and $[\nabla T_2]_p =\frac{[\nabla D]_p}{\Delta_{p+K}}$ either  have different signs or are both zero. Thus in $\R_{K,LC}^c$, $\nabla L$ can be zero only in $\reg = \cap_{p=1}^{M-K} (\A_{K,p} \cup \Z_{K,p})$.

 %In particular, in $\R_{K,LC}^c$, $[\nabla L]_p$ can be zero only inside $\A_{K,p}$.
 We need a condition on $\Delta_{p+K}$ that ensures that
\bea
[\nabla L]_p \neq 0, \ \mbox{for some $p$}, \ \forall v_{t,r} \in \reg
\label{req}
\eea

Now $T_2$ only has a minimizer inside $\R_{K,LC}$ and none outside it. Thus if we can find a condition on $\Delta_{p+K}$ that ensures that $[\nabla L]_p>0$ where $[\nabla T_2]_p>0$ and $[\nabla L]_p < 0$ where $[\nabla T_2]_p < 0$ for at least one $p$ for all points in $\reg$, we will be done.
Thus, at any point $v_{t,r} \in \reg$, we need $[\nabla L]_p . [\nabla T_2]_p > 0$ for at least one $p$.

Inside $\reg$, $v_{t,r}$ can either belong to $\cap_{p=1}^{M-K} \A_{K,p}$ or it can belong to $\Z_{K,p_1} \cap \dots \Z_{K,p_j} \cap [\cap_{p \neq p_1,p_2,\dots p_j} A_{K,p}]$ for some $j>0$.
First consider a $v_{t,r} \in \cap_{p=1}^{M-K} \A_{K,p}$.
For a given $p$, it is easy to see that $[\nabla L]_p . [\nabla T_2]_p > 0$  if $\Delta_{p+K} <  \frac{|[\nabla D]_p|}{|[\nabla E]_p|}$.
Thus for (\ref{req}) to hold, we need that for each $v_{t,r} \in \cap_{p=1}^{M-K} \A_{K,p}$, there is at least one $p$ for which $\Delta_{p+K} <  \frac{|[\nabla D]_p|}{|[\nabla E]_p|}$.
This is equivalent to requiring that
\bea
\max_{p=1,\dots (M-K)} [ \frac{|[\nabla D]_p|}{|[\nabla E]_p|} - \Delta_{K+p} ]  > 0, \ \forall v_{t,r} \in \cap_{p=1}^{M-K} \A_{K,p} \ \ \
\label{req2a}
\eea
Now consider $v_{t,r} \in \Z_{K,p_1} \cap \dots \Z_{K,p_j} \cap [\cap_{p \neq p_1,p_2,\dots p_j} \A_{K,p}] \defn \B$. Here $[\nabla L]_{p_k}=0$,  $\forall k=1,2,..j$. So in this case, for (\ref{req}) to hold, we need
\bea
\max_{p \neq p_1,p_2,..p_j}[\frac{|[\nabla D]_p|}{|[\nabla E]_p|} - \Delta_{p+K}] >0 \ \forall v_{t,r} \in \B
\label{req2b}
\eea
Now (\ref{req2a}) and (\ref{req2b}) can be combined and compactly written as: \\
$\max_{p}[\gamma_p(v_{t,r}) - \Delta_{p+K}] >0$ for all $v_{t,r} \in \reg$ or that \\
 $\inf_{v_{t,r} \in \reg} \max_{p}[\gamma_p(v_{t,r}) - \Delta_{p+K}] >0$ where $\gamma_p$ is defined (\ref{defgamma}). This is the same as (\ref{defcond}).

Condition (\ref{suff}) is sufficient for (\ref{defcond}) because $\max_p[g_1(p)-g_2(p)] > \max_p g_1(p)-\max_p g_2(p)$.
\\

% By setting $\gamma_{p_0}(v_{t,r}) = 0$ whenever $v_{t,r} \in \Z_{K,p_0}$, we have ensured that $\max_p \gamma_{p}(v_{t,r}) =\max_{p \neq p_0} \gamma_{p}(v_{t,r})$.
%Thus we get (\ref{defcond}).


%% This part is redundant
%There can be two ways of ensuring (\ref{req}). First is to find a condition on $\Delta_{p+K}$ that ensures that the sign of $[\nabla L]_p$ follows that of $[\nabla E]_p$ for at least one $p$ at all points in $\reg$, i.e. $[\nabla L]_p > 0$ where $[\nabla E]_p > 0$ and $[\nabla L]_p < 0$ where $[\nabla E]_p < 0$. The second way is to find a condition on $\Delta_{p+K}$ that ensures that the sign of $[\nabla L]_p$ follows that of $[\nabla T_2]_p$. The first option cannot be used because it will require that $\Delta_{p+K} >  \frac{|[\nabla D]_p|}{|[\nabla E]_p|}$ for some $p$ for all $v_{t,r} \in \reg$. Whenever OL is multimodal, all, except one, minimizers of $E$ will lie in $\R_{K,LC}^c$. The minimizers  will also lie on the boundary of $\reg$ since $\nabla E = 0$ at the minimizers. This will result in the requirement that $\Delta_{p+K} = \infty$ for some $p$ and hence this option cannot be used.% (at the boundary of)
%%\footnote{If $E$ has only one minimizer and condition \ref{close} holds, then $\A_{K,p}$ is an empty set for all p.
%%$\Delta_{p+K} < - \frac{[\nabla D]_p}{[\nabla E]_p}$ for some $p$ for all $v_{t,r} \in \reg$ or in other words $\max_p ( $\Delta_{p+K} < \inf_{v_{t,r} \in \reg} - \frac{[\nabla D]_p}{[\nabla E]_p} \defn \Delta_{K}^*$.
%%For unimodality of $L^i$, we need $\nabla_{v_{t,r}} L^i \neq 0$, $\forall v_{t,r} \in \R_{K,LC}^c$. As explained above, this requires (\ref{req}) to hold  for at least one $p$, i.e. $\Delta_{p+K}  < \Delta_{K}^*$ for at least one p. This is equivalent to requiring that $\max_{p=1,2,\dots M-K} [\Delta_{K,p+K}^* - \Delta_{p+K}] > 0$ (condition \ref{deltacond}).
%
%Thus we use the second option, i.e. sign of $[\nabla L]_p$ follows that of $[\nabla T_2]_p$ for at least one $p$ for all $v_{t,r} \in \reg$. %This is equivalent to requiring that (\ref{defcond}) holds. Condition (\ref{suff}) is sufficient for (\ref{defcond}) because $\max_p[g_1(p)-g_2(p)] > \max_p g_1(p)-\max_p g_2(p)$.
%
%(i.e.  $\frac{|[\nabla D]_p|}{|[\nabla E]_p|} - \Delta_{p+K} > 0$)

%Inside $\reg$, $v_{t,r}$ can either belong to $\cap_{p=1}^{M-K} \A_{K,p}$ or it can belong to $\Z_{K,p_1} \cap \Z_{K,p_2} \cap \dots \Z_{K,p_j} \cap [\cap_{p \neq p_1,p_2,\dots p_j} A_{K,p}]$. For $v_{t,r} \in \cap_p \A_{K,p}$, (\ref{req}) will hold if $\Delta_{p+K}< \frac{|[\nabla D]_p|}{|[\nabla E]_p|}$ for some $p$ at each $v_{t,r}$ or that $\max_p [\frac{|[\nabla D]_p|}{|[\nabla E]_p|} - \Delta_{p+K}] >0$ at each $v_{t,r}$. For $v_{t,r} \in \Z_{K,p_1} \cap \Z_{K,p_2} \cap \dots \Z_{K,p_j} \cap [\cap_{p \neq p_1,p_2,\dots p_j} A_{K,p}]$, $[\nabla L]_{p_k}=0$,  $\forall k=1,2,..j$. Thus we need  $\max_{p \neq p_1,p_2,..p_j}[\frac{|[\nabla D]_p|}{|[\nabla E]_p|} - \Delta_{p+K}] >0$ at each $v_{t,r}$.The above can be compactly written as: $\max_{p}[\gamma_p(v_{t,r}) - \Delta_{p+K}] >0$ for all $v_{t,r} \in \reg$ or that $\inf_{v_{t,r} \in \reg} \max_{p}[\gamma_p(v_{t,r}) - \Delta_{p+K}] >0$ where $\gamma_p$ is defined (\ref{defgamma}).
%% By setting $\gamma_{p_0}(v_{t,r}) = 0$ whenever $v_{t,r} \in \Z_{K,p_0}$, we have ensured that $\max_p \gamma_{p}(v_{t,r}) =\max_{p \neq p_0} \gamma_{p}(v_{t,r})$.
%%Thus we get (\ref{defcond}).
%%




==> rbpf.tex <==
\input{pfmtalgo}

\section{PF-MT: PF with Mode Tracker}
\label{pfmtsec}
LDSS problems very often have a small dimensional effective basis, $X_{t,s}$, in which most of the state change occurs and a large dimensional residual space,  $X_{t,r}$, in which the variance of the state change is small, i.e. $\trace(\Sigma_r)$ is small. Thus $\trace(\Sigma_{IS}^i) \le \trace(\Sigma_r)$  will also be small  \footnote{$\trace(\Sigma_{IS}^i) \le \trace(\Sigma_r)$ holds because of (\ref{defsigis}) and (\ref{defL}) and the fact that $E$ is convex at $m_t^i$ due to Theorem \ref{unimodthm}.}.
 When this is true, a valid approximation (stated rigorously in Theorem \ref{ismtthm} below) is to replace importance sampling of $X_{t,r}^i$ from $\n(m_t^i, \Sigma_{IS}^i)$ (step \ref{isxtr} in Algorithm \ref{pfeis}) by deterministically setting $X_{t,r}^i = m_t^i$.  We call this the Mode Tracking (MT) approximation to Importance Sampling (IS), since $m_t^i$ is the mode of $p^{**,i}$. Another valid approximation, when $\Sigma_r$ is small, is to set $\Sigma_{IS}^i = \Sigma_r$. This and the fact that $X_{t,r}^i = m_t^i$ makes the denominator of $\tilde{w}_t^i$ constant and hence it can be removed. The above modifications, called PF-MT, are summarized in Algorithm \ref{pfmt}.


\subsection{IS-MT Approximation}
We show below that when $\trace(\Sigma_r)$ is small, with high probability, there is little error in replacing a random sample from $\n(m_t^{i}, \Sigma_{IS}^i)$,  by  $m_t^{i}$, which is the mode of $p^{**,i}$.

\begin{theorem}[IS-MT]
Assume that Assumption \ref{gausspxtr} holds and that the conditions of Theorem \ref{unimodthm} are satisfied. Let $X_{t,r}^{i} \sim \n( m_t^{i}, \Sigma_{IS}^i)$ where $m_t^i$ and $\Sigma_{IS}^i$ are defined in (\ref{defsigis}).%, are functions of $\Sigma_r$ and of   $X_{t,s}^i$, $Y_t$ and $X_{t-1,r}^i=m_{t-1}^i$ (which is itself a function of $X_{1:t-1,s}^i$ and $Y_{1:t-1}$).
Then \\
$\forall \ \eps_1, \eps_2 > 0$,  $Pr(||X_{t,r}^{i} - m_t^{i}|| > \eps_1) < \eps_2$ whenever $\trace(\Sigma_r) < \delta_{\eps_1, \eps_2} = \eps_1^2 \eps_2/M$ and this holds for all values of $X_{1:t,s}^i, Y_{1:t}$.
In other words, $X_{t,r}^{i}$ converges to $m_t^i$ in probability as $\trace(\Sigma_r) \tends 0$, for almost all values of $X_{1:t,s}^i, Y_{1:t}$.%
\label{ismtthm}
\end{theorem}
Proof: See Appendix


The MT approximation of Importance Sampling (IS) introduces some error in the estimate of $X_{t,r}$ (error decreases with decreasing spread of $p^{**,i}$). But it reduces the PF dimension from $\dim(X_t)$ to $\dim(X_{t,s})$ (huge reduction for large dimensional problems), thus greatly improving the effective particle size. For carefully chosen dimension of $X_{t,s}$, this results in much smaller total error when the available number of particles, $N$, is small. This is observed experimentally, but proving it theoretically is an interesting open problem for future research.

Note also, that for best performance, one may choose a smaller dimensional $X_{t,r}$ for PF-MT than that for PF-EIS, i.e. split $X_{t,r}$ for PF-EIS into $X_{t,r,s}$ and $X_{t,r,r}$ and use the MT approximation only on $X_{t,r,r}$. This is discussed in Section \ref{pfeismt} and summarized in Algorithm \ref{pfeismtass}.
%(larger dimensional $X_{t,s}$)


%\subsection{Practical Modifications}
%PF-EIS-MT
%PF-D-EIS-MT (verifying assumption 1 and then implementing)
%connection with PMT, PF-D, PF-Original, PF-K-dim

\subsection{Connection with RB-PF}
%PF-MT can be understood as an approximation of the RB-PF, which is  explained in detail in \cite{gustaffson}. %Consider (7) of cc.
RB-PF \cite{chen_liu,gustaffson} is a PF algorithm which is applicable when  the state vector can be split as $X_t = [X_{t,nl},X_{t,l}]$ with the following property: $X_{t,nl}$ has any general nonlinear or non-Gaussian system and observation model; but conditioned on $X_{1:t,nl}$, $X_{t,l}$ has a linear Gaussian state space model. Thus RB-PF importance samples $X_{t,nl}$ using the original PF strategy \cite{gordon} but it applies the Kalman recursion to compute the conditional posterior of $X_{t,l}$, conditioned on each particle of $X_{1:t,nl}^i$ (which is a Gaussian in this case). The observation likelihood of each particle, $X_{1:t,nl}^i$, is computed by marginalizing over $X_{t,l}$.

PF-MT can be understood as an approximation to the RB-PF in the following sense: replace the ``nonlinear" part of the state space by $X_{t,s}$, i.e. $X_{t,nl} \equiv X_{t,s}$, and the ``linear" part by $X_{t,r}$, i.e. $X_{t,l} \equiv X_{t,r}$. In our case, the conditional posterior of $X_{t,r}$ (conditioned on  $X_{1:t,s}^i$) is assumed to be unimodal (not necessarily Gaussian), but very narrow. RB-PF requires it to be Gaussian (not necessarily narrow). PF-MT approximates the conditional posterior $X_{t,r}$, conditioned on  $X_{1:t,s}^i$ by a Dirac delta function at its mode (instead of a Gaussian in case of RB-PF).
The above can be stated  rigorously as follows.
\begin{remark}
PF-MT (Algorithm \ref{pfmt}) is  RB-PF (Algorithm 1 of \cite{gustaffson}) with the following approximation at each $t$:
\bea
&& p(Y_t|X_{t,s}^i, X_{t,r}) p (X_{t,r}|X_{t-1}^i, X_{t,s}^i)   \nn \\
& & \approx p(Y_t|X_{t,s}^i, X_{t,r}^i) p (X_{t,r}^i|X_{t-1}^i, X_{t,s}^i) \delta(X_{t,r}-X_{t,r}^i), \ \mbox{where}  \nn \\
&& X_{t,r}^i = m_t^i = \arg \max_{X_{t,r}} [ p(Y_t|X_{t,s}^i, X_{t,r}) p (X_{t,r}|X_{t-1}^i, X_{t,s}^i) ] \ \ \ \
\label{pfmtapprox}
\eea
i.e. when the STP of $X_{t,r}$ multiplied by the OL given $X_{t,s}^i$, is narrow enough s.t. it can be approximated by its maximum value times a Dirac delta function at the maximum, RB-PF and PF-MT are equivalent.
\label{pfmtrbpf}
\end{remark}
Proof: See Appendix

The proof of the above follows almost directly from Lemma \ref{rbpflemma} below and the notational substitutions: $X_{t}^{n} \equiv X_{1:t,s}$, $x_{t}^{l} \equiv X_{t,r}$, $Y_t \equiv Y_{1:t}$ in Algorithm 1 of \cite{gustaffson}.
 \begin{lemma}
Approximation (\ref{pfmtapprox}) implies that
\ben
\item $\forall \ t$,  $p(X_{t,r}|X_{1:t,s}^i,Y_{1:t}) = \delta(X_{t,r}-X_{t,r}^i)$ with $X_{t,r}^i$.% defined in (\ref{pfmtapprox}).
\label{postr}

\item $\forall \ t$, $p(Y_t|X_{1:t,s}^i,Y_{1:t-1}) = p(Y_t|X_{t}^i) p(X_{t,r}^i |X_{t-1}^i, X_{t,s}^i)$.%p(Y_t|X_{t,s}^i, X_{t,r}^i) p(X_{t,r}^i |X_{t-1,r}^i)$.
\label{obslik}

\item $\forall \ t$, $p(X_{t,s}|X_{1:t-1,s}^i,Y_{1:t-1}) = p(X_{t,s}|X_{t-1}^i)$.
%p(X_{t,s}|X_{t-1,s}^i,X_{t-1,r}^i)$ .
\label{stpxts}
\een
\label{rbpflemma}
\end{lemma}
Proof: See appendix.



% For systems where $X_{t,r}$ follows a linear Gaussian state space model conditioned on $X_{1:t,s}$, our algorithm can be understood as an approximation to Rao Blackwellized (or marginalized) PF \cite{chen_liu,gustaffson}. It replaces the Kalman filter in RB-PF by a posterior mode tracker. But it can be applied to other state space models as well, as long as conditioned on $X_{t,s}$, $X_{t,r}$ has a unimodal posterior with a narrow enough spread (a valid assumption for many LDSS problems).
%
%
%Using conditional variance identity \cite[Theorem 4.4.2]{stats},$\E_{Y_t,\chat^i}[Var(p^{**,i})] = \E_{Y_t,\chat^i}[Var[v_{t,r}|v_{t-1,r}^i,Y_t,\chat^i]] \le Var[v_{t,r}|v_{t-1,r}^i] = \Sigma_r = diag\{\Delta_p\}_{K+1}^{M}$. Since $\Sigma_{IS}^i$ approximates the variance of $p^{**,i}$, $\E_{Y_t,\chat^i}[\Sigma_{IS}^i] \approx \E_{Y_t,\chat^i}[Var(p^{**,i})] \le diag\{\Delta_p\}_{K+1}^{M}$.


%
%Assume that $m_t^i= \E[v_{t,r}|v_{t-1,r}^i,\chat^i,Y_t]$ and $\Sigma_{IS}^i = Var[v_{t,r}|v_{t-1,r}^i,\chat^i,Y_t]$. Then $v_{t,r}^{i}$  converges to $m_t^{i}$ in the max norm in probability as $\Delta_{K,tot} \defn \sum_{p=1}^{M-K} \Delta_{p+K} \tends 0$, i.e. for any $\eps>0$, $\exists \ \delta_\eps > 0$ s.t. $\forall \ \Delta_{K,tot} < \delta$, $Pr(||v_{t,r}^{i} - m_t^{i}||_\infty > \eps) < \eps$.
%$\n(v_{t,r}; m_t^{i}, \Sigma_{IS}^i) = p^{**,i}(v_{t,r}$ i.e.
 %,i.e. for any $\eps>0$, $Pr(||v_{t,r}^{i} - m_t^{i}||_\infty > \eps) < \frac{\sum_{p>K} \Delta_p}{\eps^2}.$
%Thus if $\Delta_{K,tot} \defn \sum_{p>K} \Delta_p < \eps^3$, then $Pr(||v_{t,r}^{i} - m_t^{i}||_\infty > \eps) < \eps$, i.e. $v_{t,r}^{i}$  converges to $m_t^{i}$ in probability as $\Delta_{K,tot} \tends 0$.%$\Delta_{p} \tends 0, \ \forall p>K$


%(\ref{smaller} holds because
% $M_1 < M_2$ implies that all eigenvalues of $(M_2-M_1)$ are positive.
%For any matrix $M$, $trace(M)=sum of eigenvalues of M$ (this is because $M=U Lam U'$ and trace(M)=trace(U'U Lam)=trace(Lam)=sum of eigenvalues$.
%Thus $trace(M_2-M_1)$ = sum of its eigenvalues which is positive. But $trace(M_2-M_1)=trace(M_2)-trace(M_1) >0$.

%\input{figscompare}


%In other words, RB-PF (Algorithm 1 of \cite{gustaffson}) with the above approximation implies the following 3 things. Note replace $X_{t}^{n} \equiv X_{1:t,s}$, $x_{t}^{l} \equiv X_{t,r}$ and $Y_t \equiv Y_{1:t}$ in Algorithm 1 of \cite{gustaffson}.
%\ben
%\item For each $t$,  $p(X_{t,r}|X_{1:t,s}^i,Y_{1:t}) = \delta(X_{t,r}-X_{t,r}^i)$ with $X_{t,r}^i$ defined in (\ref{pfmtapprox}). This replaces steps 4a and 4c of Algorithm 1 of \cite{gustaffson}.
%\label{postr}
%
%\item For each $t$, $p(Y_t|X_{1:t,s}^i,Y_{1:t-1}) = p(Y_t|X_{t,s}^i, X_{t,r}^i) p(X_{t,r}^i |X_{t-1,r}^i)$. This is used in step 2 of Algorithm 1 of \cite{gustaffson}.
%\label{obslik}
%
%\item For each $t$, $p(X_{t,s}|X_{1:t-1,s}^i,Y_{1:t-1}) =p(X_{t,s}|X_{t-1,s}^i,X_{t-1,r}^i)$ . This is used in step 4b of Algorithm 1 of \cite{gustaffson}.
%\label{stpxts}
%\een
%and this is the same as our PF-MT (Algorithm \ref{pfmt}).%which in turn lead to  PF-MT (Algorithm \ref{pfmt})
%\end{theorem}

% Consider (7) of  \cite{gustaffson} with $X_{t}^{n} \equiv X_{1:t,s}$ and $x_{t}^{l} \equiv X_{t,r}$. \cite{gustaffson} also runs the  original PF (IS from STP) for $X_{t,s}$, i.e. it approximates $p(X_{1:t,s}|Y_{1:t}) \approx \sum_{i} w_t^i \delta(X_{1:t,s} - X_{1:t,s}^i)$ where $w_t^i \propto w_{t-1}^i p(Y_t|X_{1:t,s}^i,Y_{1:t-1})$.  RB-PF computes $p(Y_t|X_{1:t,s}^i,Y_{1:t-1})$ exactly by marginalizing the OL over $p(X_{t,r}|X_{1:t,s}^i,Y_{1:t-1})$ (which is a Gaussian computed exactly using a Kalman filter).








